Relating Complexity-theoretic Parameters with SAT Solver Performance

Over the years complexity theorists have proposed many structural parameters to explain the surprising efficiency of conflict-driven clause-learning (CDCL) SAT solvers on a wide variety of large industrial Boolean instances. While some of these parameters have been studied empirically, until now there has not been a unified comparative study of their explanatory power on a comprehensive benchmark. We correct this state of affairs by conducting a large-scale empirical evaluation of CDCL SAT solver performance on nearly 7000 industrial and crafted formulas against several structural parameters such as backdoors, treewidth, backbones, and community structure. Our study led us to several results. First, we show that while such parameters only weakly correlate with CDCL solving time, certain combinations of them yield much better regression models. Second, we show how some parameters can be used as a "lens" to better understand the efficiency of different solving heuristics. Finally, we propose a new complexity-theoretic parameter, which we call learning-sensitive with restarts (LSR) backdoors, that extends the notion of learning-sensitive (LS) backdoors to incorporate restarts and discuss algorithms to compute them. We mathematically prove that for certain class of instances minimal LSR-backdoors are exponentially smaller than minimal-LS backdoors.

==> averagemetrics.tex <==
\centering
\begin{tabular}{llllll}
\hline
Benchmark &        LSR/V &       Weak/V &            Q &      Bones/V &         TW/V \\
\hline
Agile       &  0.28 (0.17) &  0.01 (0.01) &  0.82 (0.07) &  0.17 (0.11) &  0.16 (0.08) \\
Application &  0.56 (0.36) &  0.03 (0.05) &  0.75 (0.19) &  0.61 (0.39) &  0.31 (0.22) \\
Crafted     &  0.88 (0.20) &  0.08 (0.11) &  0.58 (0.24) &  0.39 (0.41) &  0.44 (0.29) \\
Random      &    nan (nan) &  0.11 (0.10) &  0.14 (0.10) &  0.47 (0.40) &  0.82 (0.12) \\
\hline
\end{tabular}

\caption{Mean (std. dev.) of several parameter values. }
\label{tab-meanstd}



==> benchmark_descriptions_table.tex <==
\begin{table}
  \begin{center}
    \begin{tabular}{| l | c | c |}
      \hline
      Benchmark & Obtained? & Description \\ \hline
      C02--C14 & Yes & The SAT competition benchmarks from 2002--2014 \\ \hline
      Race & Yes & The SAT Race 2008 benchmarks \\ \hline
      3SAT & Yes & Random 3SAT instances of various CVRs \\ \hline
      Auto & No & Automobile configurations from Damian Chrystler \\ \hline
      QWH & Yes & Quasigroups with holes \\ \hline
      GC & Yes & Graph coloring (from SATLib) \\ \hline
      MGC & Yes & Morphed Graph Coloring (from SATLib) \\ \hline
      LP & Yes & Logistics planning (from SATLib) \\ \hline
      CS & Yes & Circuit synthesis -- LTL, BMC, Verification, etc. \\ \hline
      FM & Yes & Real-world feature models \\ \hline
      Levi & Yes & Community-based Pseudo Industrial  \\ \hline
    \end{tabular}
  \end{center}
  \caption{Benchmarks used to support empirical efficacy of proposed structural metrics.}
\end{table}



==> comprehensive.tex <==
\section{A Comprehensive Evaluation of Structural Metrics}
\label{sec-comprehensive}

Numerous structural metrics such as backdoors \cite{williams}, community structure \cite{levi}, and treewidth \cite{mateescu} have been introduced in an attempt to explain the efficiency of CDCL SAT solvers on structured instances. However, it is less often the case that these metrics are empirically evaluated against each other, and even then the evaluation benchmark is not representative of instances found in practice. We attempt to remedy this issue by looking at multiple metrics found in practice and performing an evaluation over a wide range of benchmarks.

Our primary concern is whether solving time corresponds to a favorable metric value (e.g. a small backdoor) over a wide range of benchmarks.	\todo{add here}
Finally, given that we have data over a uniform set of benchmarks, we explore several hypotheses relating the metrics to each other. For example, we investigate the relationship between community structure and backdoors, hypothesizing that the backdoors of easier instances will cluster into a small set of communities.

\subsection{Experimental Setup}

==> datasummary.tex <==
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Benchmark &  Instances &   LSR &  Weak &  Cmty &  Bones &    TW \\
\hline
Application &       1238 &   420 &   306 &   984 &    218 &  1181 \\
Crafted     &        753 &   327 &   195 &   613 &    154 &   753 \\
Random      &        126 &   123 &    76 &   126 &     59 &   126 \\
Agile       &       4968 &  2828 &   464 &  4968 &    208 &  4968 \\ \hline
Total       &       7085 &  3698 &  1041 &  6691 &    639 &  7028 \\
\hline
\end{tabular}
\end{center}
\caption{ The number of instances for which we were able to successfully compute each parameter. ``Cmty'' refers to the community parameters; ``TW'' denotes the treewidth upper bound; ``Bones'' denotes backbone size. }
\label{tab_data_summary}



==> laser_figures.tex <==
	
	\todo{DependencyList is a mapping from vars to the decision vars needed to derive it (and all of its deriving clauses, recursively).}
	
	\begin{figure}[t]
		\renewcommand\algorithmicthen{}
		\renewcommand\algorithmicfunction{}
		\begin{algorithmic}[1]
			\Function{Laser\_a}{Vars finalDecs, DependencyList depList} 
			\State $B = finalDecs$ 	
			\For{$v \in AllVars \setminus finalDecs$} \Comment{Optimized with ``workpool''}
			\State $B = B \cup depList[v]$
			\EndFor
			\State \Return {$B$}
			
			\EndFunction
		\end{algorithmic}
		\caption{Current version.}
		\label{cas-preds}
	\end{figure}
	
	\begin{figure}[H]
		\renewcommand\algorithmicthen{}
		\renewcommand\algorithmicfunction{}
		\begin{algorithmic}[1]
			\Function{Laser\_b}{Vars finalDecs, DependencyList depList} 
			\State $S = Solver() $ 
			\For{$v$ in $AllVars$}
			\State $createSolverBool(v_b)$ \Comment{True if $v$ is in the LSR backdoor $B$.}
			\State $createSolverBool(v_i)$ \Comment{True if $parents(v)$ are all implied, or $v \in B$.}
			
			\EndFor
			
			\For{$v \in AllVars$}
			\State $S.assert(v_i)$
			\If $v \in finalDecs$
			\State $S.assert(v_B)$
			\Else
			\State $S.assert(\bigwedge_{p\in parents(v)} p_i \vee v_B )$
			\EndIf
			\EndFor
			\State $objectiveFunc = \sum_{v \in AllVars} b2i(v_B) $
			\State $model = S.minimize(objectiveFunc)$
			\State $B = \{v \mid model[v_B]\}$
			\State \Return {$B$}
			
			\EndFunction
		\end{algorithmic}
		\caption{Basically the idea is that for every non-final decision var, we have a choice of either including it, or all of its dependencies. \texttt{b2i(v)} is a macro for \texttt{If(v, 1, 0)}.}
		\label{cas-preds}
	\end{figure}
	
	%Note -- Graph abstraction based approach (maybe -- could be able to perform better heuristics with graph structure -- basically a dependency graph with nodes and clauses)
		

	\begin{figure}[H]
		\renewcommand\algorithmicthen{}
		\renewcommand\algorithmicfunction{}
		\begin{algorithmic}[1]
			\Function{\textbf{struct} State}{}
				\State{set$<$Clause$>$ learnts}
				\State{vector$<$Lit$>$ trail} 
			\EndFunction
			\State{}
			
			\Function{\textbf{def} isBackdoor}{Formula F, Vars V, bool withRestarts} 
			\LeftComment{Performs BFS over all decision sequences, pruning as necessary.}
			
			\State{Queue$<$State$>$ Q}
			\State{Set$<$State$>$ seenStates}
			\State{Q.push(EmptyState)}
			
			\While{$\neg$Q.empty()}
				\State State state = Q.pop()
				\State Solver solver = generateCleanMiniSAT$^{-}$(F)	
				\State \Comment{for now, learned unit clauses get put at beginning of trail}
				\State solver.updateLearnts(state.learnts)
				\State success = solver.solveWithTrail(state.trail)
				\If{}success
				\State \Return true
				\Else \Comment{Solver is in a failed state. Generate new decision branches.}
				\For{$v \in $ solver.unassignedVars $\cap$ V}
					\State Q.pushIfUnseen(new State(solver.learnts, solver.trail + ($\neg$v)))
					\State Q.pushIfUnseen(new State(solver.learnts, solver.trail + (v)))
					\If withRestarts and ``just learned clause''
					\State Q.pushIfUnseen(new State(solver.learnts, EmptyTrail))
					\EndIf
					
					
				\EndFor
				\EndIf
				
			\EndWhile
			
			
			\EndFunction
			\State{}
			\Function{\textbf{def} MinimumBackdoor}{Formula F, bool withRestarts} 
			\For{$k = 1 \ldots nVars()$}
			\For{every set $V$ of $k$ variables}
				\If{}isBackdoor(F, V, withRestarts)
				\State return V
				\EndIf
			\EndFor
			\EndFor
			\EndFunction
		\end{algorithmic}
		\caption{Solver$^-$: turns off periodic restarts and clause deletion. Takes as input a sequence of literals to be used for branch selection. If the sequence is exhausted and the solver has not determined SAT/UNSAT, returns unknown.}
		\label{cas-preds}
	\end{figure}
	
	Minimum LS Notes:
	\begin{itemize}
		\item if k == nVars, would compute the smallest possible number of decisions needed to decide F.
	\end{itemize}
\suppress{
	\todo{garbage:	
		For the first learnt clause $c_0$, $D_{c_0}$ can clearly be used to derive the clause from the initial state.
		For an arbitrary learnt clause $c^\prime$, we must reconstruct $R_{c^\prime}$ by only branching on variables $V_{c^\prime}$. Let $L_{full}$ be the full set of clauses derived by $S$ up to this point, and for any learnt clause $c$, let $L_c$ be the  that were used to derive any clause in $R_{c^\prime}$ \todo{include recursive clauses, dont know how to state}.
	}
	
	
	
	\todo{consider the set of clauses from S that recursively derive that of c', and ignore the rest}
	
	\todo{suppose there are n lc clauses used in R. Use S to get proof of r0, to derive r1, note that any learnts inbetween r0 and r1 cannot contribute to learning c' since they are not in R by our lc ordering ....if any intermediate exists theyll show up in the R for lc, but their vars will be accounted for}
	
	\todo{suppose by induction that for each lc in R, we can derive it from initial with Vlc, need to show we can derive all learnt clauses needed to derive c', use S somehow}
	
	\todo{finish...} 
	Starting from an initial solver state, our approach is to first derive all learnt clauses in $C$, and then use the decisions from $D$ to derive $c^\prime$. Note that the run of the solver $S$ up to the current point does not necessarily demonstrate that $V_{c^\prime}$ adheres to its desired property, since $S$ may have branched on other variables, or derived additional clauses not in $C$.
	
	Let $L$ be the set of learnt clauses in $C$, and $\sigma_L$ be a sequence over $L$ indicating the order in which $S$ learned the clauses. We derive the clauses in $L$ in the same order as witnessed by $S$. 
	
	
	Suppose we have already derived all clauses in $C$. By construction, each clause $c \in CS \cup RS$ can be derived by a SAT solver using only variables in $V_c$ %(as witnessed by the current run of the SAT solver up to the current conflict). 
	Note that for the $c^\prime$ under question, the current solver state cannot be directly used to complete the proof, as other branching decisions and learnt clauses may have been found by the solver that were not involved in the current conflict.
	Let $L_D$ be the literals used in the current conflict analysis corresponding to the variables in $D$.
	To derive 
	By assigning the variables in $D$ in the same order and polarity as the current state of the solver, unit propagation will the clauses in , unit propagation   \todo{finish}
}

==> ls_vs_lsr_sep.tex <==
\suppress{
Let $n$ be a positive integer and let $X = \set{x_1, x_2, \ldots, x_n}$ be a set of boolean variables.
For any boolean variable $x$, let $x^1$ denote the positive literal $x$ and $x^{0}$ denote the negative literal $\neg x$.
For any assignment $\alpha \in \set{0,1}^n$ let $C_\alpha = x_1^{1-\alpha_1} \vee x_2^{1-\alpha_2} \vee \ldots \vee x_n^{1-\alpha_n}$ denote the clause on $x$ variables which is uniquely falsified by the assignment $\alpha$.
The following CNF formula ${\cal F}$ was introduced for the purpose of separating \emph{strong backdoors} from \emph{learning sensitive backdoors}.
The formula is defined on the variables $x_1, x_2, \ldots, x_n$, and also three auxiliary sets of variables $\set{q_\alpha}_{\alpha \in \set{0,1}^n}, \set{a_\alpha}_{\alpha \in \set{0,1}^n}, \set{b_\alpha}_{\alpha \in \set{0,1}^n}$:
\begin{align*}
  {\cal F} = & \bigwedge_{\alpha \neq \vec 1} (C_\alpha \vee \neg q_\alpha) \wedge (q_\alpha \vee a_\alpha) \wedge (q_\alpha \vee b_\alpha) \wedge (q_\alpha \vee \neg a_\alpha \vee \neg b_\alpha) \\
  & \wedge \left(C_{\vec 1} \vee \bigvee_{\alpha \in \set{0,1}^n} \neg q_\alpha\right) \wedge (q_{\vec 1} \vee a_{\vec 1}) \wedge (q_{\vec 1} \vee b_{\vec 1}) \wedge (q_{\vec 1} \vee \neg a_{\vec 1} \vee \neg b_{\vec 1}).
\end{align*}
In this note we modify this formula to obtain a CNF formula providing an exponential separation between \emph{learning sensitive backdoors} and \emph{learning-sensitive backdoors with restarts}.
Throughout we implicitly assume that the clause learning algorithm is \emph{First UIP}.

\todo{eventually delete the formula above, and mention that the formula below is also from Dilkina}
Our formula will be defined by the following template.
Let ${\cal O}$ be an ordering of $\set{0,1}^n$; we write $<_{\cal O}$ to denote the relation induced by this ordering.
Given an ordering ${\cal O}$ we can define the formula \[{\cal F}_{\cal O} = \bigwedge_{\alpha \in \set{0,1}^n} (C_\alpha \vee \bigvee_{\alpha' \leq_{\cal O} \alpha} \neg q_{\alpha'}) \wedge (q_\alpha \vee a_\alpha) \wedge (q_\alpha \vee b_\alpha) \wedge (q_\alpha \vee \neg a_\alpha \vee \neg b_\alpha).\]

\begin{lemma}
  Let ${\cal O}$ be any ordering of $\set{0,1}^n$.
  The $X$-variables form a learning-sensitive backdoor with restarts for the formula ${\cal F}_{\cal O}$.
\end{lemma}
\begin{proof}
  Query the $x$ variables according to the ordering given by ${\cal O}$.
  As soon as we have a complete assignment to the $x$ variables, we will unit-propagate to a conflict and learn a $q_\alpha$ variable as a conflict clause; after that we restart.
  Once all such assignments are explored we can simply query the $X$ variables in any order (without restarts) to yield a contradiction, since every assignment to the $X$ variables will falsify the formula.
\end{proof}

Given two orderings ${\cal O}_1, {\cal O}_2$ let $d({\cal O}_1, {\cal O}_2)$ denote the Hamming distance of these two sequences (as sequences).
For instance the Hamming distance of the two sequences $(00, 01, 10, 11)$ and $(00, 10, 01, 11)$ is $2$.
Finally, consider any decision tree $T$ of depth $n$ where we have queried the $X$ variables in \emph{any} order in the tree $T$.
From this tree we obtain a natural ordering ${\cal O}(T)$ of $\set{0,1}^n$ by reading off the strings labelling the leaves in left-to-right order.
Note that the orderings of the form ${\cal O}(T)$ are \emph{exactly} the orderings which can be generated by DPLL algorithms (or, more generally, a CDCL algorithm without restarts).
}

\begin{lemma}\label{lem:main}
  Let ${\cal O}$ be any ordering of $\set{0,1}^n$, and let ${\cal T}_X$ denote the collection of all complete depth-$n$ decision trees on $X$ variables.
  Then any LS-backdoor of ${\cal F}_{\cal O}$ has size at least \[n + \min_{T \in {\cal T}_X} d({\cal O}, {\cal O}(T)).\]
\end{lemma}
\begin{proof}
  Let $B$ be a minimal learning-sensitive backdoor of ${\cal F}_{\cal O}$.
  Let $Q = \set{q_\alpha}_{\alpha \in \set{0,1}^n}$.
  Without loss of generality we can assume that $B \subseteq X \cup Q$, as a learning sensitive backdoor which queries $a_\alpha$ or $b_\alpha$ variables can be replaced with a backdoor querying $q_\alpha$ variables which is no larger.
  Furthermore, we can assume that $X \subseteq B$.
  To see this, observe first that $Q$ is \emph{not} a learning sensitive backdoor of ${\cal F}_{\cal O}$, since querying all assignments to the $Q$ variables will leave the algorithm in an inconclusive state.
  \todo{potential issue -- I think we only need n - 1 of the X variables, since if we already derived the necessary q's, we propagate the final x for free}
  It follows that $B$ must contain \emph{some} $X$ variable; to see that it contains \emph{all} $X$ variables, it is enough to observe that in order to hit a conflict (even after querying all $Q$ variables) we must assign a value to every $X$ variable by the structure of ${\cal F}_{\cal O}$.
  Thus $X \subseteq B \subseteq X \cup Q$ (and $|X|$ represents the $n$ term in the statement of the lemma).
    
  Furthermore, observe that we can always assume that if the algorithm queries a $q_\alpha$ variable as a decision variable, then it queries the variable negatively first.
  This is because querying $\neg q_\alpha$ will cause the CDCL algorithm to hit a conflict and learn the unit clause $q_\alpha$, so we may replace such ``positive'' queries \emph{in-situ} with negative queries without affecting the simulation of the backdoor queries.
  In turn, this implies that we may assume that all $q_\alpha$ variables occurring in the backdoor are queried at the beginning of the algorithm, leaving only queries to $X$ variables.
  Since all $q_\alpha$ variables in the backdoor $B$ are queried at the beginning of the algorithm without loss of generality, by the structure of ${\cal F}_{\cal O}$ we can see that once we start querying $X$ variables, we will only hit a conflict once we have assigned values to \emph{all} of the $X$ variables.
  This implies that the query order for the $X$ variables takes the form of a complete depth-$n$ decision tree $T \in {\cal T}_X$, using the notation in the statement of the lemma.

  With this, we can prove that every clause learned by the algorithm is a unit clause of the form $q_\alpha$ for some $\alpha \in \set{0,1}^n$.
  To see this, consider any time that we have hit a conflict in the process of simulating the variable queries of the backdoor $B$.
  If we have hit a conflict from querying $\neg q_\alpha$, as described above, we are done, so suppose otherwise.
  By assumption, the only variables that $B$ contains other than $Q$ variables are $X$ variables, thus, to hit a conflict we must have queried all of the $X$ variables by the structure of ${\cal F}_{\cal O}$.
  In such a case, since we have not queried $\neg q_\alpha$ for any $\alpha$, we must have unit-propagated $\neg q_\alpha$ for some $\alpha$ by the structure of ${\cal F}_{\cal O}$.
  This will hit a conflict and learn the unit clause $q_\alpha$, proving our claim.

  Recalling that $X \leq B \leq X \cup Q$, to prove the lemma it suffices to prove that \[|B \cap Q| \geq \min_{T \in {\cal T}_X} d({\cal O}, {\cal O}(T)) \] since $|X| = n$.
  Since $B$ is a backdoor, it must be that at every leaf of the tree $T$ the unit propagator will propagate the input to a conflict.
  Consider the ordering of the assignments ${\cal O}(T)$ induced by this tree $T$.
  At each leaf of this tree, which corresponds to an assignment $\alpha$ to the $X$ variables, there are two possibilities: either we learn the unit clause $q_\alpha$ or not.
  By the structure of ${\cal F}_{\cal O}$, we can only learn the unit clause $q_\alpha$ at the leaf if we have learned the unit clauses $q_{\alpha'}$ for each $\alpha' \leq_{{\cal O}} \alpha$.
  Thus, for any index in the orderings ${\cal O}(T)$ and ${\cal O}$, if the index has different strings in the respective orderings, it follows that we will not be able to learn the unit clause $q_\alpha$, and so we will have to query at least one extra variable from $Q$ in the backdoor $B$.
  This proves that \[|B \cap Q| \geq \min_{T \in {\cal T}_X} d({\cal O}, {\cal O}(T)) \] and therefore the lemma.
\end{proof}

By the previous lemma, to lower bound the size of the learning sensitive backdoor it suffices to find an ordering ${\cal O}$ of $\set{0,1}^n$ which is far in hamming distance from \emph{every} ordering of the form ${\cal O}(T)$ for some complete decision tree $T \in {\cal T}_X$ on the $X$ variables.

\begin{lemma}
  There exists an ordering ${\cal O}$ of $\set{0,1}^n$ such that for every decision tree $T \in {\cal T}_X$ we have \[ d({\cal O}, {\cal O}(T)) \geq 2^{n-1}.\]
\end{lemma}
\begin{proof}
  Let $N = 2^n - 1$ and write ${\cal O}(T) = \alpha_0, \alpha_1, \ldots, \alpha_N$.
  We use the following key property of orderings generated from decision trees:

  \spcnoindent
  {\bf Key Property.} For all $j = 0, 1, \ldots, N/2 - 1$, the strings $\alpha_{2j}, \alpha_{2j+1}$ differ at exactly one coordinate.

  \spcnoindent
  This property is easy to prove: every node in the decision tree $T$ which is the parent of a leaf is labeled with some variable $x_i$; it follows that both leaves below it differ exactly on the coordinate indexed by $x_i$.
  To use this property, recall that a \emph{Gray ordering} of $\set{0,1}^n$ is any ordering ${\cal O} = g_0, g_1, \ldots, g_{N-1}$ where for all $i = 0, 1, \ldots, N-2$ the strings $g_i$ and $g_{i+1}$ differ on exactly one coordinate.
  Observe that this immediately implies that $g_i$ and $g_{i+2}$ have Hamming distance exactly 2 for each $i$ --- this is because $d(g_i, g_{i+1}) = d(g_{i+1}, g_{i+2}) = 1$ and we could not have flipped the same coordinate twice to get from $g_i$ to $g_{i+1}$ to $g_{i+2}$.
  So, given any Gray ordering ${\cal O}$ of $\set{0,1}^n$, define the ordering ${\cal O}'$ by taking the ordering ${\cal O}$ and swapping the positions of the strings $g_{2j+1}$ and $g_{2j + 2}$ for all $j = 0, 1, \ldots, N/2 - 2$, and let \[ {\cal O}' = g_0', g_1', \ldots, g_{N-1}'\] after doing this swap.
  By what we have argued above, for any decision tree $T$ and all $j = 0, 1, \ldots, N/2 - 1$ at least one of the pairs of strings $\alpha_{2j}, g'_{2j}$ and $\alpha_{2j+1}, g'_{2j+1}$ must be mismatched, implying the lemma.
\end{proof}
\suppress{
\begin{corollary}
  There exists an ordering ${\cal O}$ such that any learning-sensitive backdoor for the formula ${\cal F}_{\cal O}$ has size at least $n + 2^{n-1}$.
\end{corollary}
}



==> lsr_all_decs_comparison.tex <==
\centering
\begin{tabular}{llll}
\hline
Benchmark &        Laser & All Decisions & Overlap Ratio \\
\hline
Agile       &  0.28 (0.17) &   0.35 (0.15) &   0.37 (0.13) \\
Application &  0.56 (0.36) &   0.57 (0.35) &   0.70 (0.26) \\
Crafted     &  0.88 (0.20) &   0.89 (0.19) &   0.89 (0.17) \\
Random      &    nan (nan) &     nan (nan) &     nan (nan) \\
\hline
\end{tabular}

\caption{Mean (std. dev.) of Laser produced backdoor sizes versus all decision variables. Overlap Ratio is the size of the set $(Laser \cap All Decisions) / (Laser \cup All Decisions)$.}
\label{lsr_vs_all_decs_table}



==> lsr_all_decs_table.tex <==
\begin{table}[t]
\centering
\begin{tabular}{llll}
{} &        LaSeR & AllDecisions & OverlapRatio \\
benchmark &              &              &              \\

agile     &  0.16 (0.11) &  0.38 (0.16) &  0.34 (0.11) \\
app       &  0.45 (0.33) &  0.56 (0.33) &  0.58 (0.29) \\
crafted   &  0.80 (0.24) &  0.85 (0.22) &  0.79 (0.23) \\
random    &    nan (nan) &    nan (nan) &    nan (nan) \\

\end{tabular}
\label{lsr_vs_all_decs_table}
\caption{\todo{clean}Comparison of LaSeR produced backdoor sizes versus all decision variables. Overlap Ratio is the size of the set $(LaSeR \cap AllDecisions) / (Laser \cup AllDecisions)$.}
\end{table}


==> paper_extensions.tex <==
\suppress{
	\begin{table}[t]
		\begin{center}
			\begin{tabular}{ |l|l||c|c|c| }
				\hline
				\textbf{Property} & \textbf{Benchmark} & \textbf{Luby} & \textbf{Always Restart} & \textbf{Never Restart} \\ \hline
				\multirow{4}{12em}{P1: Community-based Spatial Locality of Decisions} &
				agile & 0.672 & \textbf{0.701} & 0.693\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P2: Community-based Spatial Locality of Learnt Clauses} &
				agile & 0.725 & \textbf{0.739} & 0.697\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P3: LSR Size} &
				agile & 0.212 & \textbf{0.133} & 0.271\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P4: Avg. LSR of Learnt Clauses} &
				agile & 0.136 & \textbf{0.051} & 0.203\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P5: Avg. Number of Backbone Flips, Normalized for Backbone Size} &
				agile & 578.124 & 3005.809 & \textbf{36.486}\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P6: Number of Learnt Clauses Subsumed by Backbones, Normalized for Backbone Size} &
				agile & 14.452 & 164.800 & \textbf{2.106}\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
			\end{tabular}
		\end{center}
	\end{table}
	
\textit{P1: Spatial Locality of Decisions.} Given a community structure, we test whether the branching heuristic tends to disproportionately favor picking from certain communities. Note that this is effectively the same experiment as in \cite{hvc}, however here we are modifying the restart policy rather than the branching heuristic itself.

\textit{P2: Spatial Locality of Learnt Clauses.} Given a community structure, we test whether learnt clauses are disproportionately composed of variables from certain communities.

\textit{P3: LSR Size.} We test the LSR size, as computed by the approach discussed in Section \ref{lsralgsec}. A run of the solver that relies on fewer variables may be more favorable, and demonstrates a different type of locality than in P1 and P2.

\textit{P4: Avg. Learnt Clause LSR Size.} When computing the LSR-backdoor, each learnt clause is annotated with a set of variables $V$, which intuitively is the set of variables a fresh can branch upon and eventually derive the clause (as witnessed by the current run of the solver). We compute the average $V$ value of all learnt clauses. 

\textit{P5: Avg. Number of Backbone Flips.} Ideally, if the solver had \textit{a priori} knowledge of the backbone, it could set all variables to their correct polarity and simplify the formula accordingly. We consider how often the solver ``flips'' the polarity of a backbone literal, i.e., by adding it to the trail with a different polarity than previously. This may, in some sense, indicate that the solver is \textit{unsure} of the correct polarity of the backbone literal. 

\textit{P6: Number of Learnt Clauses Subsumed by the Backbone.} We consider how many learnt clauses are generated that contain a backbone literal with the correct polarity. In some sense, these clauses would be redundant if the solver had \textit{a priori} knowledge of the backbone, since they would be immediately satisfied.

	
We consider whether each of these components affects the size of the minimal backdoor. Further, we will also consider whether incorporating restarts, a pivotal feature of modern CDCL solvers, impacts the size of the backdoor. We note that, in addition to these features, modern solvers also incorporate clause minimization techniques to shrink learnt clauses \cite{Biere}, however we do not consider it in this work.

%\input{bd_comparison_table}

%Table \ref{bd-comparison-table} depicts our results. \todo{If we get a significant chunk of this table filled in, convert to a directed graph}

\begin{tabular}{llllll}
	\toprule
	{} &       simp\_lvr & simp\_all\_decsvr & simp\_lsr\_all\_decs\_unionvr & simp\_lsr\_all\_decs\_intervr & simp\_lsr\_all\_decs\_overlap\_ratio \\
	benchmark &                &                 &                           &                           &                                 \\
	\midrule
	agile     &  0.164 (0.108) &   0.375 (0.159) &             0.398 (0.167) &             0.141 (0.086) &                   0.344 (0.113) \\
	app       &  0.454 (0.335) &   0.564 (0.327) &             0.611 (0.319) &             0.412 (0.347) &                   0.581 (0.289) \\
	crafted   &  0.796 (0.235) &   0.853 (0.221) &             0.905 (0.172) &             0.744 (0.270) &                   0.793 (0.227) \\
	random    &      nan (nan) &       nan (nan) &                 nan (nan) &                 nan (nan) &                       nan (nan) \\
	\bottomrule
\end{tabular}

\section{LSR vs LS Examples}

\subsection{LS-Jumps-Restarts is exponentially smaller than strong \cite{bibid}} 

Assume we have a set $X$ of $k$ variables $x_1 \ldots x_k$. Given $\alpha: x_i \rightarrow {0, 1}$, let $C_\alpha$ be short for $\bigvee_{i=1}^{k} x_i^{1-\alpha_i}$ which is falsified by assigning $X$ according to the natural mapping of $\alpha$, e.g. $C_{001} = x_1 \vee x_2 \vee \neg x_3$. We will show that $X$ is an LSR-backtracking backdoor, but the smallest LS-backtracking backdoor is [TODO: exponentially?] bigger. At each line we learn through 1UIP the unit clause $\neg q_{\alpha}$.

The following is from \cite{Dilkina}, where $\alpha_1$ = $0^k$ and in general $\alpha_i$ is the lexicographic predecessor of $\alpha_{i+1}$.

$$
(C_{\alpha 1} \vee q_{\alpha 1}), 
(\neg q_{\alpha 1} \vee r_{\alpha 1}), 
(\neg q_{\alpha 1} \vee \neg r_{\alpha 1} \vee s_{\alpha 1}),
(\neg q_{\alpha 1} \vee \neg r_{\alpha 1} \vee \neg s_{\alpha 1})
$$
$$
(C_{\alpha 2} \vee q_{\alpha 1} \vee q_{\alpha 2}), 
(\neg q_{\alpha 2} \vee r_{\alpha 2}), 
(\neg q_{\alpha 2} \vee \neg r_{\alpha 2} \vee s_{\alpha 2}),
(\neg q_{\alpha 2} \vee \neg r_{\alpha 2} \vee \neg s_{\alpha 2})
$$
$$ \ldots$$
$$
(C_{\alpha 2^k} \vee q_{\alpha 1} \vee q_{\alpha 2} \vee \ldots \vee q_{\alpha 2^k} ), 
(\neg q_{\alpha 2^k} \vee r_{\alpha 2^k}), 
(\neg q_{\alpha 2^k} \vee \neg r_{\alpha 2^k} \vee s_{\alpha 2^k}),
(\neg q_{\alpha 2^k} \vee \neg r_{\alpha 2^k} \vee \neg s_{\alpha 2^k})
$$

\subsection{LS-Jumps+Restarts is [exponentially(?)] smaller than LS-Jumps-Restarts}
\todo{Not exponential -- view space of $\alpha$'s as a hypercube, and adversary can pick corner}

With the ordering of $\alpha_i$'s above, restarts do not help as a backtracking solver can learn every $\neg q_{\alpha j}$, $j < i$ before learning $\neg q_{\alpha i}$. By changing the sequence of $\alpha_i$'s to not be lexicographic, we can force a non-restarting backtracking solver to branch on variables other than in $X$.

Let $\alpha_1 = 0^k$ as before, and generally let $\alpha_{i+1}$ be the string lexicographically farthest from $\alpha_{i}$, that was not previously defined by any $\alpha_j$, $j < i$. \todo{finish; solver must start branching on non-X vars}

\subsection{Whiteboard Notes}
\begin{itemize}
	\item In order to derive any $q_{\alpha_i}$, must either pick $q_{\alpha_i}$ or derive every $q_{\alpha_j}, j < i$.
	\item If we've already derived some $q_{\alpha_i}$ it would propagate the x's instead, but I don't think this has consequence.
	\item Conjecture -- If we only ever branch on x's and q's, the only clauses we can possibly learn are $\neg q$'s.
	\item Suppose adversary starts with x sequence $x_1, ..., x_k$. Then we must learn every $q$ on the branch of $x_1$ before we can move to $x_1^{-1}$ branch. Need to count the number of assignments on the $x_1$ side that depend on q's of the other side.
\end{itemize}

\begin{conjecture}
	Take the formula from 7.1, with any ordering of the $\alpha$'s. Then, if the solver is only allowed to branch on $x$'s and $q$'s, regardless of the decision sequence, it can only learn unit clauses of the form $\neg q$. \todo{PROBLEM: assign all q's first??}
\end{conjecture}
\begin{proof}
	Suppose $c$ is the first learnt clause. There are three cases which can lead to this conflict. If we assign $q$ (positively), we immediately learn $\not q$. Suppose we falsify some clause with $C_{\alpha_i}$.
\end{proof}

\subsection{Whiteboard Notes 2.0}
Our goal is to show that the smallest LSR+backtracking backdoor for $F$ is exponentially smaller than the smallest LS+backtracking backdoor. We know $F$ is minimally unsatisfiable. First, let us partition $F$ into two sets of clauses. Let $\Delta_1$ be the $2^k$ clauses that contain some $C_{\alpha_i}$ disjunction, and $\Delta_2$ be the remaining clauses that allow us to learn each $\neg q_i$, i.e., the clauses in $L(\neg q_i)$ for all $i$. Let $F_{x=b} = \Delta_1[x=b] \cup \{ L(q_\alpha) \mid q_\alpha \in vars(\Delta_1[x=b]) \}$

\todo{proof sketch -- order the clauses according to number of qs, since each clause has 2 unseen vars, and the formula is min unsat, we must branch upon one of them to use the clause}

\begin{lemma}
For any $x \in X$ and any polarity $b$, $F_{x=b}$ is minimally unsatisfiable.
\end{lemma}
\begin{proof}
	Suppose for some $\alpha$ we remove some clause from $L(\neg q_alpha)$. Then we can assign $q_alpha$ (positively) without conflicting. By assigning $X$ according to $\alpha$, and $\neg q_\beta$, $\beta \ne \alpha$, we can satisfy all other clauses.
	If instead we remove any clause $C \in \Delta_1[x=b]$, then we can satisfy the remaining clauses by setting $\neg q_\alpha$ for every $\alpha$, and $X$ according to $\neg \alpha$.
\end{proof}



\subsection{LS+Jumps+Restarts is [exponentially(?)] smaller than LS+Jumps-Restarts}
\todo{BROKEN, but maybe not for sat case}
$X$ will denote our backdoor set of size $k$, where $k$ is even (\todo{may need one more var}). Different from before, $C_\alpha$ will correspond to a disjunction of the first $k/2$ variables in $X$, and $C_\beta$ is a disjunction of the second $k/2$ variables. Rather than the clauses used to conflict and learn $\neg q_\alpha$ as before, we have the following formula which will be used to derive binary clauses rather than unit clauses:
\todo{Fix 1uip according to williams discussion}
$$
L(l_\alpha \vee l_\beta) ::=
(\neg l_\alpha \vee r_\alpha),
(\neg l_\alpha \vee s_\alpha),
(\neg l_\beta \vee r_\beta),
(\neg l_\beta \vee s_\beta),
(\neg r_\alpha \vee \neg s_\alpha \vee \neg r_\beta \vee \neg s_\beta)
$$

We define a formula $\Omega(n)$ which is any formula over $n$ fresh variables with backdoor size $n$. As an example, the formula with all possible clauses of length $n$ over the $n$ variables will suffice. Finally, let $\Omega[l_1, l_2](n)$, where the literals $l_1, l_2$ are not in $\Omega(n)$, be the same as $\Omega(n)$, but every clause has the additional literals $l_1$ and $l_2$.

Potential example with LSR-backdoor set $X$ + any single $q$ or $r$:

\begin{equation}
\label{lsr_jump_eqn}
\begin{split}
&\bigwedge_{\alpha} 
(C_{\alpha} \vee q_{\alpha}),
\bigwedge_{\beta} 
(C_{\beta} \vee \neg r_{\beta}), \\
&\bigwedge \{ L(q_\alpha \Rightarrow r_\beta) \mid \alpha = \beta\} \\ 
&\bigwedge \{ L(r_\beta \Rightarrow q_\alpha) \mid \alpha = \beta + 1\} \\ 
&\bigwedge \{ \Omega[q_\alpha, \neg r_{\beta}] \mid \alpha \ne \beta \wedge \alpha \ne \beta + 1\}  \\
&(\neg q_{\alpha_0} \Rightarrow  r_{\beta_{2^k}}), 
(q_{\alpha_0} \Rightarrow \neg r_{\beta_{2^k}}), 
(\neg q_{\alpha_0} \Rightarrow \neg r_{\beta_{2^k}}),
\end{split}
\end{equation}

\todo{Might need to hide (4) under last X vals}

\begin{theorem}
	There exists a family of formulas such that the smallest LSR+backjumping backdoor is \todo{exponentially} smaller than the smallest LS+backjumping backdoor.
\end{theorem}
\begin{proof}
We first demonstrate that 
\end{proof}



\suppress{
\section{LSR vs LS old}
$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee p_1^\prime), (\neg x \vee p_2^\prime), (\neg p_1^\prime \vee \neg p_2^\prime \vee \neg q \vee q^\prime), (\neg q^\prime \vee a^\prime), (\neg q^\prime \vee \neg a^\prime \vee b^\prime), (\neg q^\prime \vee \neg a^\prime \vee \neg b^\prime) 
$$
$$
(x \vee q \vee q^\prime \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$


\section{LSR may be arbitrarily smaller than LS}
The following formula from the LS paper has a minimal LS backdoor \{x\}:
$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee q \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$
Essentially, if we set $x=0$, we learn $\neg q$ on the top half, which leads to a conflict on the bottom half when we set $x=1$.

Now consider a new formula which duplicates the first line: 
{\boldmath$$
(x \vee p_1^\prime), (x \vee p_2^\prime), (\neg p_1^\prime \vee \neg p_2^\prime \vee q^\prime), (\neg q^\prime \vee a^\prime), (\neg q^\prime \vee \neg a^\prime \vee b^\prime), (\neg q^\prime \vee \neg a^\prime \vee \neg b^\prime) 
$$
}$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee q \bm{\vee q^\prime} \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$
We can then set $x=0$ to learn $q$ as before, but then restart to learn $q^\prime$ as well. 

We can repeat this any number of times by introducing a new ``prime row'' (and q in the bottom clause).
This breaks my previous conjecture that $LS = LSR + \mathcal{O}(log(numRestarts))$. New conjecture: $LS = LSR + \mathcal{O}(numRestarts))$.


\section{Main Contributions}
\begin{itemize}
	\item LSR backdoor definition + algorithm
	\item Correlation experiments for several metrics over SAT comps + scaling.
	\item Relationship of cmty structure/bridges and backdoors
	\item Solving with a priori knowledge of metrics		
\end{itemize}

\section{Paper Threats}
\begin{itemize}
	\item Need to motivate LSR backdoors
	\begin{itemize}
		\item Small examples where minimum LS-backdoor is larger than LSR
		\item General relationship/bound of LSR to LS sizes.
	\end{itemize}
	\item General Threats to Validity
	\begin{itemize}
		\item We don't have optimal value (e.g. minimum backdoors). Answer: using current best algorithms + long timeouts.
		\item Consider multiple solvers (for now just maplesat times). Have most data for Glucose and Minisat. 
		\item Consider more than linear regression for correlation experiments (ridge regression, which handles multicollinearity better than LR, achieved similar $R^2$ values)
		\item LSR computation based upon solver run (circularity threat?.. cannot remember how we resolved this..)
		\item Solving times should probably be recomputed on StarExec/Azure (sharcnet has some unpredictability).
		\item Need to explain why correlations are lower than 2014 cmty structure paper.
	\end{itemize}
\end{itemize}
}
}

==> regression.tex <==
\begin{center}
\scalebox{0.7}{
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Feature Set} & \textbf{Application} & \textbf{Crafted} & \textbf{Random} & \textbf{Agile}\\ \hline

$V\oplus{}C\oplus{}C/V$ & 0.02 (1093) & 0.04 (706) & 0.08 (126) & 0.85 (4964)\\

$V\oplus{}C\oplus{}Cmtys\oplus{}Q$ & 0.04 (841) & 0.14 (566) & 0.25 (126) & 0.87 (4964)\\

$V\oplus{}C\oplus{}LSR\oplus{}LSR/V$ & 0.16 (345) & 0.40 (281) & N/A & 0.88 (3257)\\

$V\oplus{}C\oplus{}\#Min\_Weak\oplus{}Weak$ & 0.11 (238) & 0.14 (160) & 0.23 (76) & 0.56 (464)\\

$V\oplus{}C\oplus{}Bones\oplus{}Bones/V$ & 0.10 (167) & 0.35 (119) & 0.04 (59) & 0.43 (208)\\

$V\oplus{}C\oplus{}TW\oplus{}TW/V$ & 0.03 (1037) & 0.05 (706) & 0.28 (126) & 0.91 (4964)\\

$V\oplus{}C\oplus{}TW\oplus{}LSR\oplus{}Q\oplus{}Cmtys$ & 0.08 (345) & 0.53 (281) & N/A & 0.95 (3257)\\

$V\oplus{}C\oplus{}TW\oplus{}TW/V$ & 0.03 (1037) & 0.05 (706) & 0.28 (126) & 0.91 (4964)\\

\hline
$C/V\oplus{}Q\oplus{}Q/Cmtys\oplus{}LSR/V\oplus{}TW/V$ & \textbf{0.39 (345)} & 0.62 (281) & N/A & 0.94 (3257)\\

$C\oplus{}C/V\oplus{}Q\oplus{}LSR/V\oplus{}TW/V$ & 0.25 (345) & \textbf{0.65 (281)} & N/A & 0.93 (3257)\\

$V\oplus{}C\oplus{}C/V\oplus{}Cmtys\oplus{}Q$ & 0.10 (345) & 0.34 (281) & \textbf{N/A} & 0.91 (3257)\\

$V\oplus{}C\oplus{}Q\oplus{}LSR/V\oplus{}TW/V$ & 0.17 (345) & 0.58 (281) & N/A & \textbf{0.94 (3257)}\\

\hline
\end{tabular}
}
\end{center}
\caption{Adjusted R$^2$ values for the given features, compared to log of Maplecomsps' solving time. The number in parentheses indicates the number of instances that were considered in each case. The lower section of feature sets consider heterogeneous sets of features from different structural analyses.}
\label{tab-regressions}



==> related_work_table.tex <==
\begin{table}
\begin{center}
	\begin{tabular}{| l | c | c | c |}
		\hline
		Type & Benchmarks & Defined for Unsat? & Tool Available?  \\ \hline
		Strong \cite{Chaharmir2002} & 3SAT  & Yes & Yes (\cite{Li2011, Kilby2005}) \\ \hline
		Weak \cite{Chaharmir2002} & 3SAT, GC & No & Yes (\cite{Li2011, Kilby2005}) \\ \hline
		LS \cite{Dilkina2009a} & LP  & Yes & Yes (implemented) \\ \hline
		Tree \cite{Samer2008} & Auto, 3SAT  & Yes & No \\ \hline
		%Clause Deletion & Not Sure \todo{} & Yes & Not Sure \\  \hline
		LSR  & -- & Yes & Yes (implemented) \\
		\hline \hline
		Weak Keys \cite{Ruan2004} & MGC, LP, QWH & No & Yes (trivial) \\ \hline
		Backbones \cite{Chaharmir2002, Kilby2005} & 3SAT, GC & No & Yes (\cite{Marques-silva2012}) \\ \hline
		LSR Keys & -- & No & Yes (implemented) \\  \hline \hline
		% \footnote{\url{http://sat.inesc-id.pt/~mikolas/#Software}}
		Treewidth \cite{Mateescu2011, Liang2015} & C09, FM & Yes & No (Algorithm in \cite{Mateescu2011}) \\ \hline
		Q \cite{Newsham, Ans??tegui2012} & Most (all?) & Yes & Yes (Louvain, OL) \\ \hline
		Input-restricted \cite{Newsham, Ans??tegui2012} & CS & Yes & Yes (trivial) \\ \hline
	\end{tabular}
\end{center}
\caption{Subset of the proposed backdoors from the literature. Below the first double-line are concepts that are either related to backdoors. We also include treewidth and modularity of the community structure Q, as they have been proposed as an alternative metric for measuring the difficulty of SAT instances.}
\end{table}

==> related_work_table_condensed.tex <==

\begin{center}
	\begin{tabular}{| l | m{5.5em} | c | m{19em} |}
		\hline
		Type & Benchmarks & Unsat? & Tool Description \\ \hline
		%Strong \cite{Kilby2005,Li2011,Chaharmir2002} & 3SAT  & Yes & Not considered. \todo{explain or delete} \\ \hline
		Weak \cite{Kilby2005,Li2011,Chaharmir2002} & 3SAT, GC, SR & No & Perform Tabu-based  local search to minimize the number of decisions in the final model.  \\ \hline
		LS \cite{Dilkina2009a,Dilkina2014} & LP  & Yes & Run a clause-learning solver, recording all decisions, which constitutes a backdoor.  \\ \hline
		%Tree \cite{Samer2008} & Auto, 3SAT  & Yes & Not considered in experiments. \\ \hline
		%Deletion & Not Sure \todo{} & Yes \\  \hline
		%LSR  & -- & Yes & Yes (implemented) \\
		%\hline 
		%Weak Keys \cite{Ruan2004} & MGC, LP, QWH & No & Not considered in experiments. \\ \hline %Compute a weak backdoor as above. Compute the set of \textit{dependent} variables in the backdoor (see \cite{Ruan2004}). \\ \hline
		Backbones \cite{janota2015algorithms,Kilby2005,Chaharmir2002} & 3SAT, GC, Comps & No & Repeated SAT calls with UNSAT-core based optimizations.
		%Core-based heuristics which reduce the number of SAT calls necessary to check if each literal is in the backdoor.  
		\\ \hline
		%LSR Keys & -- & No ) \\  \hline \hline
		% \footnote{\url{http://sat.inesc-id.pt/~mikolas/#Software}}
		Treewidth \cite{Liang2015,Mateescu2011} & C09, FM & Yes & Heuristically compute residual graph $G$. The max-clique of $G$ is an upper-bound. \\ \hline
		Modularity \cite{Ansotegui2012,newsham2014impact} & Comps & Yes & The \textit{Louvain method} \cite{blondel2008fast} -- greedily join communities to improve modularity. \\ \hline
		%Input-restricted \cite{Newsham, Ans??tegui2012} & CS & Yes \\ \hline
	\end{tabular}
\end{center}
\caption{Previously studied benchmarks for each considered parameter, as well as description of tools used to compute them. The ``Unsat?'' column indicates if the parameter is defined on unsatisfiable instances. Abbrevations: 3SAT -- random 3-SAT; GC -- graph coloring; LP -- logistics planning; SR -- SAT Race 2008;
	%Auto -- automobile configuration; MGC -- morphed graph coloring; QWH -- quasigroup with holes; Comps -- SAT competitions; 
	C09 -- SAT competition 2009; Comps -- 2009-2014 SAT competitions; FM -- feature models. }
\label{tab-relatedwork}


==> satmin_averagemetrics.tex <==
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Benchmark &        LSR/V &       Weak/V &            Q &      Bones/V &         TW/V \\
\hline
Agile       &  0.18 (0.13) &  0.01 (0.01) &  0.82 (0.07) &  0.17 (0.11) &  0.16 (0.08) \\
Application &  0.35 (0.34) &  0.03 (0.05) &  0.75 (0.19) &  0.64 (0.38) &  0.32 (0.22) \\
Crafted     &  0.58 (0.35) &  0.08 (0.11) &  0.58 (0.24) &  0.39 (0.41) &  0.44 (0.29) \\
Random      &  0.64 (0.32) &  0.11 (0.10) &  0.14 (0.10) &  0.47 (0.40) &  0.82 (0.12) \\
\hline
\end{tabular}
\end{center}
\caption{ Mean (std. dev.) of several parameter values. }
\label{tab-meanstd}



==> satmin_lsr_all_decs_comparison.tex <==
\centering
\begin{tabular}{llll}
\hline
Benchmark &        Laser & All Decisions & Overlap Ratio \\
\hline
Agile       &  0.18 (0.13) &   0.36 (0.17) &   0.43 (0.14) \\
Application &  0.34 (0.33) &   0.57 (0.35) &   0.70 (0.26) \\
Crafted     &  0.58 (0.35) &   0.89 (0.19) &   0.89 (0.17) \\
Random      &  0.64 (0.32) &    0.91 (nan) &    0.92 (nan) \\
\hline
\end{tabular}

\caption{Mean (std. dev.) of Laser produced backdoor sizes versus all decision variables. Overlap Ratio is the size of the set $(Laser \cap All Decisions) / (Laser \cup All Decisions)$.}
\label{lsr_vs_all_decs_table}



==> satmin_regression.tex <==
\begin{center}
\scalebox{0.93}{
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Feature Set} & \textbf{Application} & \textbf{Crafted} & \textbf{Random} & \textbf{Agile}\\ \hline

$V\oplus{}C\oplus{}C/V$ & 0.03 (1237) & 0.04 (753) & 0.04 (126) & 0.84 (4968)\\

$V\oplus{}C\oplus{}Cmtys\oplus{}Q$ & 0.06 (982) & 0.22 (613) & 0.17 (126) & 0.86 (4968)\\

$V\oplus{}C\oplus{}LSR\oplus{}LSR/V$ & 0.14 (420) & 0.26 (327) & 0.26 (123) & 0.87 (2828)\\

$V\oplus{}C\oplus{}\#Min\_Weak\oplus{}Weak$ & 0.04 (299) & 0.11 (195) & 0.08 (76) & 0.54 (464)\\

$V\oplus{}C\oplus{}Bones\oplus{}Bones/V$ & 0.18 (218) & 0.39 (154) & 0.04 (59) & 0.39 (208)\\

$V\oplus{}C\oplus{}TW\oplus{}TW/V$ & 0.05 (1180) & 0.07 (753) & 0.11 (126) & 0.91 (4968)\\

\hline
$Q\oplus{}C/V\oplus{}LSR/V\oplus{}Q/Cmtys\oplus{}C$ &\textbf{0.29 (420)} & 0.34 (327) & 0.13 (123) & 0.90 (2828)\\

$TW/V\oplus{}Q\oplus{}Cmtys\oplus{}TW\oplus{}LSR/V$ & 0.12 (420) & \textbf{0.57 (327)} & 0.08 (123) & 0.92 (2828)\\

$Q/Cmtys\oplus{}LSR/V\oplus{}C\oplus{}LSR\oplus{}Q$ & 0.22 (420) & 0.35 (327) & \textbf{0.45 (123)} & 0.89 (2828)\\

$Cmtys\oplus{}TW/V\oplus{}C/V\oplus{}TW\oplus{}Q$ & 0.18 (420) & 0.29 (327) & 0.04 (123) & \textbf{0.93 (2828)}\\

\hline
\end{tabular}
}
\end{center}
\caption{ Adjusted R$^2$ values for the given features, compared to log of MapleCOMSPS' solving time. The number in parentheses indicates the number of instances that were considered in each case. The lower section considers heterogeneous sets of features across different parameter types.}
\label{tab-regressions}



==> scrap.tex <==
\suppress{
We consider whether each of these components affects the size of the minimal backdoor. Further, we will also consider whether incorporating restarts, a pivotal feature of modern CDCL solvers, impacts the size of the backdoor. We note that, in addition to these features, modern solvers also incorporate clause minimization techniques to shrink learnt clauses \cite{Biere}, however we do not consider it in this work.

%\input{bd_comparison_table}

%Table \ref{bd-comparison-table} depicts our results. \todo{If we get a significant chunk of this table filled in, convert to a directed graph}



\section{LSR vs LS Examples}

\subsection{LS-Jumps-Restarts is exponentially smaller than strong \cite{bibid}} 

Assume we have a set $X$ of $k$ variables $x_1 \ldots x_k$. Given $\alpha: x_i \rightarrow {0, 1}$, let $C_\alpha$ be short for $\bigvee_{i=1}^{k} x_i^{1-\alpha_i}$ which is falsified by assigning $X$ according to the natural mapping of $\alpha$, e.g. $C_{001} = x_1 \vee x_2 \vee \neg x_3$. We will show that $X$ is an LSR-backtracking backdoor, but the smallest LS-backtracking backdoor is [TODO: exponentially?] bigger. At each line we learn through 1UIP the unit clause $\neg q_{\alpha}$.

The following is from \cite{Dilkina}, where $\alpha_1$ = $0^k$ and in general $\alpha_i$ is the lexicographic predecessor of $\alpha_{i+1}$.

$$
(C_{\alpha 1} \vee q_{\alpha 1}), 
(\neg q_{\alpha 1} \vee r_{\alpha 1}), 
(\neg q_{\alpha 1} \vee \neg r_{\alpha 1} \vee s_{\alpha 1}),
(\neg q_{\alpha 1} \vee \neg r_{\alpha 1} \vee \neg s_{\alpha 1})
$$
$$
(C_{\alpha 2} \vee q_{\alpha 1} \vee q_{\alpha 2}), 
(\neg q_{\alpha 2} \vee r_{\alpha 2}), 
(\neg q_{\alpha 2} \vee \neg r_{\alpha 2} \vee s_{\alpha 2}),
(\neg q_{\alpha 2} \vee \neg r_{\alpha 2} \vee \neg s_{\alpha 2})
$$
$$ \ldots$$
$$
(C_{\alpha 2^k} \vee q_{\alpha 1} \vee q_{\alpha 2} \vee \ldots \vee q_{\alpha 2^k} ), 
(\neg q_{\alpha 2^k} \vee r_{\alpha 2^k}), 
(\neg q_{\alpha 2^k} \vee \neg r_{\alpha 2^k} \vee s_{\alpha 2^k}),
(\neg q_{\alpha 2^k} \vee \neg r_{\alpha 2^k} \vee \neg s_{\alpha 2^k})
$$

\subsection{LS-Jumps+Restarts is [exponentially(?)] smaller than LS-Jumps-Restarts}
\todo{Not exponential -- view space of $\alpha$'s as a hypercube, and adversary can pick corner}

With the ordering of $\alpha_i$'s above, restarts do not help as a backtracking solver can learn every $\neg q_{\alpha j}$, $j < i$ before learning $\neg q_{\alpha i}$. By changing the sequence of $\alpha_i$'s to not be lexicographic, we can force a non-restarting backtracking solver to branch on variables other than in $X$.

Let $\alpha_1 = 0^k$ as before, and generally let $\alpha_{i+1}$ be the string lexicographically farthest from $\alpha_{i}$, that was not previously defined by any $\alpha_j$, $j < i$. \todo{finish; solver must start branching on non-X vars}

\subsection{Whiteboard Notes}
\begin{itemize}
	\item In order to derive any $q_{\alpha_i}$, must either pick $q_{\alpha_i}$ or derive every $q_{\alpha_j}, j < i$.
	\item If we've already derived some $q_{\alpha_i}$ it would propagate the x's instead, but I don't think this has consequence.
	\item Conjecture -- If we only ever branch on x's and q's, the only clauses we can possibly learn are $\neg q$'s.
	\item Suppose adversary starts with x sequence $x_1, ..., x_k$. Then we must learn every $q$ on the branch of $x_1$ before we can move to $x_1^{-1}$ branch. Need to count the number of assignments on the $x_1$ side that depend on q's of the other side.
\end{itemize}

\begin{conjecture}
	Take the formula from 7.1, with any ordering of the $\alpha$'s. Then, if the solver is only allowed to branch on $x$'s and $q$'s, regardless of the decision sequence, it can only learn unit clauses of the form $\neg q$. \todo{PROBLEM: assign all q's first??}
\end{conjecture}
\begin{proof}
	Suppose $c$ is the first learnt clause. There are three cases which can lead to this conflict. If we assign $q$ (positively), we immediately learn $\not q$. Suppose we falsify some clause with $C_{\alpha_i}$.
\end{proof}

\subsection{Whiteboard Notes 2.0}
Our goal is to show that the smallest LSR+backtracking backdoor for $F$ is exponentially smaller than the smallest LS+backtracking backdoor. We know $F$ is minimally unsatisfiable. First, let us partition $F$ into two sets of clauses. Let $\Delta_1$ be the $2^k$ clauses that contain some $C_{\alpha_i}$ disjunction, and $\Delta_2$ be the remaining clauses that allow us to learn each $\neg q_i$, i.e., the clauses in $L(\neg q_i)$ for all $i$. Let $F_{x=b} = \Delta_1[x=b] \cup \{ L(q_\alpha) \mid q_\alpha \in vars(\Delta_1[x=b]) \}$

\todo{proof sketch -- order the clauses according to number of qs, since each clause has 2 unseen vars, and the formula is min unsat, we must branch upon one of them to use the clause}

\begin{lemma}
For any $x \in X$ and any polarity $b$, $F_{x=b}$ is minimally unsatisfiable.
\end{lemma}
\begin{proof}
	Suppose for some $\alpha$ we remove some clause from $L(\neg q_alpha)$. Then we can assign $q_alpha$ (positively) without conflicting. By assigning $X$ according to $\alpha$, and $\neg q_\beta$, $\beta \ne \alpha$, we can satisfy all other clauses.
	If instead we remove any clause $C \in \Delta_1[x=b]$, then we can satisfy the remaining clauses by setting $\neg q_\alpha$ for every $\alpha$, and $X$ according to $\neg \alpha$.
\end{proof}



\subsection{LS+Jumps+Restarts is [exponentially(?)] smaller than LS+Jumps-Restarts}
\todo{BROKEN, but maybe not for sat case}
$X$ will denote our backdoor set of size $k$, where $k$ is even (\todo{may need one more var}). Different from before, $C_\alpha$ will correspond to a disjunction of the first $k/2$ variables in $X$, and $C_\beta$ is a disjunction of the second $k/2$ variables. Rather than the clauses used to conflict and learn $\neg q_\alpha$ as before, we have the following formula which will be used to derive binary clauses rather than unit clauses:
\todo{Fix 1uip according to williams discussion}
$$
L(l_\alpha \vee l_\beta) ::=
(\neg l_\alpha \vee r_\alpha),
(\neg l_\alpha \vee s_\alpha),
(\neg l_\beta \vee r_\beta),
(\neg l_\beta \vee s_\beta),
(\neg r_\alpha \vee \neg s_\alpha \vee \neg r_\beta \vee \neg s_\beta)
$$

We define a formula $\Omega(n)$ which is any formula over $n$ fresh variables with backdoor size $n$. As an example, the formula with all possible clauses of length $n$ over the $n$ variables will suffice. Finally, let $\Omega[l_1, l_2](n)$, where the literals $l_1, l_2$ are not in $\Omega(n)$, be the same as $\Omega(n)$, but every clause has the additional literals $l_1$ and $l_2$.

Potential example with LSR-backdoor set $X$ + any single $q$ or $r$:

\begin{equation}
\label{lsr_jump_eqn}
\begin{split}
&\bigwedge_{\alpha} 
(C_{\alpha} \vee q_{\alpha}),
\bigwedge_{\beta} 
(C_{\beta} \vee \neg r_{\beta}), \\
&\bigwedge \{ L(q_\alpha \Rightarrow r_\beta) \mid \alpha = \beta\} \\ 
&\bigwedge \{ L(r_\beta \Rightarrow q_\alpha) \mid \alpha = \beta + 1\} \\ 
&\bigwedge \{ \Omega[q_\alpha, \neg r_{\beta}] \mid \alpha \ne \beta \wedge \alpha \ne \beta + 1\}  \\
&(\neg q_{\alpha_0} \Rightarrow  r_{\beta_{2^k}}), 
(q_{\alpha_0} \Rightarrow \neg r_{\beta_{2^k}}), 
(\neg q_{\alpha_0} \Rightarrow \neg r_{\beta_{2^k}}),
\end{split}
\end{equation}

\todo{Might need to hide (4) under last X vals}

\begin{theorem}
	There exists a family of formulas such that the smallest LSR+backjumping backdoor is \todo{exponentially} smaller than the smallest LS+backjumping backdoor.
\end{theorem}
\begin{proof}
We first demonstrate that 
\end{proof}



\suppress{
\section{LSR vs LS old}
$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee p_1^\prime), (\neg x \vee p_2^\prime), (\neg p_1^\prime \vee \neg p_2^\prime \vee \neg q \vee q^\prime), (\neg q^\prime \vee a^\prime), (\neg q^\prime \vee \neg a^\prime \vee b^\prime), (\neg q^\prime \vee \neg a^\prime \vee \neg b^\prime) 
$$
$$
(x \vee q \vee q^\prime \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$


\section{LSR may be arbitrarily smaller than LS}
The following formula from the LS paper has a minimal LS backdoor \{x\}:
$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee q \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$
Essentially, if we set $x=0$, we learn $\neg q$ on the top half, which leads to a conflict on the bottom half when we set $x=1$.

Now consider a new formula which duplicates the first line: 
{\boldmath$$
(x \vee p_1^\prime), (x \vee p_2^\prime), (\neg p_1^\prime \vee \neg p_2^\prime \vee q^\prime), (\neg q^\prime \vee a^\prime), (\neg q^\prime \vee \neg a^\prime \vee b^\prime), (\neg q^\prime \vee \neg a^\prime \vee \neg b^\prime) 
$$
}$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee q \bm{\vee q^\prime} \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$
We can then set $x=0$ to learn $q$ as before, but then restart to learn $q^\prime$ as well. 

We can repeat this any number of times by introducing a new ``prime row'' (and q in the bottom clause).
This breaks my previous conjecture that $LS = LSR + \mathcal{O}(log(numRestarts))$. New conjecture: $LS = LSR + \mathcal{O}(numRestarts))$.


\section{Main Contributions}
\begin{itemize}
	\item LSR backdoor definition + algorithm
	\item Correlation experiments for several metrics over SAT comps + scaling.
	\item Relationship of cmty structure/bridges and backdoors
	\item Solving with a priori knowledge of metrics		
\end{itemize}

\section{Paper Threats}
\begin{itemize}
	\item Need to motivate LSR backdoors
	\begin{itemize}
		\item Small examples where minimum LS-backdoor is larger than LSR
		\item General relationship/bound of LSR to LS sizes.
	\end{itemize}
	\item General Threats to Validity
	\begin{itemize}
		\item We don't have optimal value (e.g. minimum backdoors). Answer: using current best algorithms + long timeouts.
		\item Consider multiple solvers (for now just maplesat times). Have most data for Glucose and Minisat. 
		\item Consider more than linear regression for correlation experiments (ridge regression, which handles multicollinearity better than LR, achieved similar $R^2$ values)
		\item LSR computation based upon solver run (circularity threat?.. cannot remember how we resolved this..)
		\item Solving times should probably be recomputed on StarExec/Azure (sharcnet has some unpredictability).
		\item Need to explain why correlations are lower than 2014 cmty structure paper.
	\end{itemize}
\end{itemize}
}
}

==> structure_logging.tex <==
\centering
\begin{center}
	\begin{tabular}{ |l|c|c|c| }
		\hline
		\textbf{Property} & \textbf{Luby} & \textbf{Always Restart} & \textbf{Never Restart} \\ \hline
		LSR Size& 0.16 (0.11) & \textbf{0.13 (0.08)} & 0.25 (0.17)\\
		Avg. Clause LSR& 0.11 (0.08) & \textbf{0.05 (0.05)} & 0.19 (0.14)\\
		Num Conflicts& 133246 (206441) & \textbf{50470 (84606)} & 256046 (347899)\\
		Solving Time (s)& 8.59 (14.26) & \textbf{6.09 (11.01)} & 18.09 (24.86)\\
		\hline
	\end{tabular}
\end{center}

\caption{Comparison of LSR measures and solving time for various restart policies on the Agile benchmark. LSR sizes are normalized by the number of variables.}
\label{tab_lens}



==> structure_logging_table.tex <==
\begin{table}[t]
	\begin{center}
		\begin{tabular}{ |l|l||c|c|c| }
			\hline
			\textbf{Property} & \textbf{Benchmark} & \textbf{Luby} & \textbf{Always Restart} & \textbf{Never Restart} \\ \hline
			\multirow{4}{12em}{P1: LSR Size} &
			agile & nan & nan & nan\\
			& app & nan & nan & nan\\
			& crafted & nan & nan & nan\\
			& random & nan & nan & nan \\ \hline
			\multirow{4}{12em}{Solving Time} &
			agile & nan & nan & nan\\
			& app & nan & nan & nan\\
			& crafted & nan & nan & nan\\
			& random & nan & nan & nan \\ \hline
		\end{tabular}
		\caption{\todo{fill in}}
	\end{center}
\end{table}

==> summary.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrrrrr}
\toprule
{} &  Instances &   SAT &  LSR &  Weak &  Cmty &  Bones &    TW \\
\midrule
Agile       &       4968 &   315 &    0 &   464 &  4968 &    208 &  4968 \\
Application &       1144 &   438 &    0 &   281 &   891 &    193 &  1088 \\
Crafted     &        753 &   236 &    0 &   195 &   613 &    154 &   753 \\
Random      &        126 &    76 &    0 &    76 &   126 &     59 &   126 \\
Total       &       6991 &  1065 &    0 &  1016 &  6598 &    614 &  6935 \\
\bottomrule
\end{tabular}

\caption{The number of instances in each benchmark, as well as the number of instances we were able to successfully compute each parameter/time (timeouts included). ``Cmty'' refers to the community parameters; ``TW'' denotes the treewidth upper bound; ``Bones'' denotes backbone size. Note that the number of satisfiable instances upper bounds the number of instances for which we can obtain weak backdoors and backbones.}
\end{table}



==> tables/averagemetrics.tex <==
\centering
\begin{tabular}{llllll}
\hline
Benchmark &        LSR/V &       Weak/V &            Q &      Bones/V &         TW/V \\
\hline
Agile       &  0.28 (0.17) &  0.01 (0.01) &  0.82 (0.07) &  0.17 (0.11) &  0.16 (0.08) \\
Application &  0.56 (0.36) &  0.03 (0.05) &  0.75 (0.19) &  0.61 (0.39) &  0.31 (0.22) \\
Crafted     &  0.88 (0.20) &  0.08 (0.11) &  0.58 (0.24) &  0.39 (0.41) &  0.44 (0.29) \\
Random      &    nan (nan) &  0.11 (0.10) &  0.14 (0.10) &  0.47 (0.40) &  0.82 (0.12) \\
\hline
\end{tabular}

\caption{Mean (std. dev.) of several parameter values. }
\label{tab-meanstd}



==> tables/background.tex <==
\section{Background}
\label{sec:background}
\textbf{CDCL SAT Solvers.}  We assume basic familiarity with the
satisfiability problem, CDCL solvers and the standard notation used by
solver developers and complexity theorists. For an overview we refer
to \cite{biere2009handbook}. We assume that Boolean formulas are given
in conjunctive normal form (CNF). For a formula $F$, we denote its variables
as \textit{vars(F)}. A \textit{model} refers to a complete satisfying
assignment to a formula.  The \textit{trail} refers to the sequence of
variable assignments, in the order they have been assigned, at any
given point in time during the run of a solver. Learnt clauses are
derived by analyzing the \textit{conflict analysis graph} (CAG), which
represents which decisions and propagations that led to a conflict. We
assume the first unique implication point (1st-UIP) clause learning
scheme throughout this paper, which is the most common in practice
\cite{moskewicz2001chaff}. The learnt clause (aka conflict clause)
defines a cut in the CAG; we denote the subgraph on the side of the
cut which contains the conflict node as the \textit{conflict side},
and the other side as the \textit{reason side}.  For a set of clauses
$\Delta$ and a literal $l$, $\Delta \vdash_1 l$ denotes that unit
propagation can derive $l$ from $\Delta$.

\textbf{Backdoors and Backbones.}  Backdoors are defined with respect
to \textit{subsolvers}, which are algorithms that can solve certain
class of SAT instances in polynomial-time. Example subsolvers
include the unit propagation (UP) algorithm
\cite{Dilkina2014,Williams2003}, which is also what we focus on as
it is a standard
subroutine implemented in CDCL SAT solvers.  Given a partial
assignment $\alpha: B \rightarrow \{0,1\}$, the simplification of $F$
with respect to $\alpha$, denoted $F[\alpha]$, removes all clauses
that are satisfied by $\alpha$, and removes any literals that are
falsified by $\alpha$ in the remaining clauses.  A \textit{strong
  backdoor} of a formula $F$ is a set of variables $B$ such that for
every assignment $\alpha$ to $B$, $F[\alpha]$ can be determined to be
satisfiable or unsatisfiable by the UP subsolver \cite{Williams2003}.
A set of variables $B$ is a \textit{weak backdoor} with respect to a
subsolver $S$ if there exists an assignment $\alpha$ to $B$ such that
the UP subsolver determines the formula to be satisfiable.  Backdoors
were further extended to allow clause-learning to occur while
exploring the search space of the backdoor:

\begin{definition}[Learning-sensitive (LS) backdoor \cite{Dilkina2009}]
	A set of variables $B \subseteq vars(F)$ is an LS-backdoor of
        a formula $F$ with respect to a subsolver $S$ if there exists
        a search-tree exploration order such that a CDCL SAT solver
        without restarts, branching only on $B$ and learning clauses
        at the leaves of the tree with subsolver $S$, either finds a
        model for $F$ or proves that $F$ is unsatisfiable.
\end{definition}

%The \textit{backbone} of a SAT instance is the set of variables such
%that all models of the instance contain the same polarity of the
%	variable \cite{monasson1999determining}. 
The backbone of a SAT instance is the maximal set of variables such that all variables in the set have the same polarity in every model \cite{monasson1999determining}.
Note that weak backdoors and
backbones are typically only defined over satisfiable
instances. Further, while the backbone of an instance is unique, many
backdoors may exist; we typically try to find the smallest backdoors
possible.

\textbf{Learning-sensitive with Restarts (LSR) Backdoors.}
\label{bg_lsr}
We introduce the concept of an LSR-backdoor here.  Section
\ref{sec_lsr_algorithms} formalizes our approach.

\begin{definition}[Learning-sensitive with restarts (LSR) backdoor]
	A set of variables $B \subseteq vars(F)$ is an LSR-backdoor of
        the formula $F$ with respect to a subsolver $S$ if there
        exists a search-tree exploration order such that a CDCL SAT
        solver (with restarts), branching only on $B$ and learning
        clauses at the leaves of the tree with subsolver $S$, either
        finds a model for $F$ or proves that $F$ is unsatisfiable.
\end{definition}

By allowing restarts, the solver may learn clauses from different
parts of the search-tree of $B$, which would otherwise not be
accessible without restarts. 
%From an empirical perspective, allowing
%restarts has several advantages. First, restarts are a pivotal aspect
%of CDCL performance, and since we compute LSR-backdoors from a run of
%a CDCL solver, performance is much faster with restarts
%enabled. 
%Further, restarts allow us to reduce the size of the
%computed backdoor using algorithms for \textit{clause absorption} from
%\cite{atserias2011clause}, as discussed in Section
%\ref{sec_lsr_algorithms}.
In Section
\ref{sec_lsr_algorithms}, we demonstrate an approach to computing upper bounds on minimal LSR-backdoor sizes using algorithms for \textit{clause absorption} from
\cite{atserias2011clause}, which intrinsically relies upon restarts.

\textbf{Graph Parameters.}  We refer to treewidth~\cite{robertson1984graph} and
community structure~\cite{Ansotegui2012} as graph parameters. All graphs parameters
are computed over the \textit{variable incidence graph (VIG)} of a CNF
formula $F$ \cite{Ansotegui2012}. There exists a vertex for every
variable in $F$, and edges between vertices if their corresponding
variables appear in clauses together (weighted according to clause
size).  Intuitively, the community structure of a graph is a partition
of the vertices into communities such that there are more
intra-community edges than inter-community
edges. The \textit{modularity} or \textit{Q} value intuitively denotes
how easily separable the communities of the graph are. The \textit{Q}
value ranges from $[-1/2, 1)$, where values near $1$ means the communities are
highly 
separable and the graph intuitively has a \textit{better} community
structure.  \textit{Treewidth} intuitively measures how much a graph
resembles a tree. Actual trees have treewidth 1. Further details can
be found in \cite{robertson1984graph}.



==> tables/benchmark_descriptions_table.tex <==
\begin{table}
  \begin{center}
    \begin{tabular}{| l | c | c |}
      \hline
      Benchmark & Obtained? & Description \\ \hline
      C02--C14 & Yes & The SAT competition benchmarks from 2002--2014 \\ \hline
      Race & Yes & The SAT Race 2008 benchmarks \\ \hline
      3SAT & Yes & Random 3SAT instances of various CVRs \\ \hline
      Auto & No & Automobile configurations from Damian Chrystler \\ \hline
      QWH & Yes & Quasigroups with holes \\ \hline
      GC & Yes & Graph coloring (from SATLib) \\ \hline
      MGC & Yes & Morphed Graph Coloring (from SATLib) \\ \hline
      LP & Yes & Logistics planning (from SATLib) \\ \hline
      CS & Yes & Circuit synthesis -- LTL, BMC, Verification, etc. \\ \hline
      FM & Yes & Real-world feature models \\ \hline
      Levi & Yes & Community-based Pseudo Industrial  \\ \hline
    \end{tabular}
  \end{center}
  \caption{Benchmarks used to support empirical efficacy of proposed structural metrics.}
\end{table}



==> tables/comprehensive.tex <==
\section{A Comprehensive Evaluation of Structural Metrics}
\label{sec-comprehensive}

Numerous structural metrics such as backdoors \cite{williams}, community structure \cite{levi}, and treewidth \cite{mateescu} have been introduced in an attempt to explain the efficiency of CDCL SAT solvers on structured instances. However, it is less often the case that these metrics are empirically evaluated against each other, and even then the evaluation benchmark is not representative of instances found in practice. We attempt to remedy this issue by looking at multiple metrics found in practice and performing an evaluation over a wide range of benchmarks.

Our primary concern is whether solving time corresponds to a favorable metric value (e.g. a small backdoor) over a wide range of benchmarks.	\todo{add here}
Finally, given that we have data over a uniform set of benchmarks, we explore several hypotheses relating the metrics to each other. For example, we investigate the relationship between community structure and backdoors, hypothesizing that the backdoors of easier instances will cluster into a small set of communities.

\subsection{Experimental Setup}

==> tables/conclusions.tex <==
\section{Future Work and Conclusions}

We presented a large-scale study of several structural parameters of
SAT instances. We showed that combinations of these features can lead
to improved regression models, and that in general, industrial
instances tend to have much more favorable parameter values than
crafted or random. Further, we gave examples of how such parameters
may be used as a ``lens'' to evaluate different solver heuristics. We
hope these studies can be used by complexity theorists as a guide for
which parameters to focus on in future analyses of CDCL. Finally, we
introduced LSR-backdoors, which characterize a sufficient subset of
the variables that CDCL can branch on to solve the formula.  In doing
so, we presented an algorithm to compute LSR-backdoors that exploits
the notion of clause absorption, and further showed that certain
formulas have exponentially smaller minimal LSR-backdoors than
LS-backdoors under the assumption that the CDCL solver only backtracks
(not backjumps) and uses the 1st-UIP learning scheme. From a theoretical point
of view, it remains open whether there is a separation between LS and
LSR-backdoors when backjumping is allowed.  On the empirical side, we
plan to investigate approaches to computing many small LSR-backdoors
to formulas. The intuition is that CDCL solvers may be more efficient
on Application instances because they have lots of LSR-backdoors and
the solver may ``latch'' on to a backdoor relatively easily, while
these solvers are less efficient for crafted instances because they
have too few backdoors.  Further, we plan to refine our results by
analyzing individual sub-categories of the benchmarks studied,
with a particular focus on scaling to crafted instances.


==> tables/introduction.tex <==
\section{Introduction}
Modern conflict-driven clause-learning (CDCL) satisfiability (SAT)
solvers routinely solve real-world Boolean instances with millions of
variables and clauses, despite the Boolean satisfiability problem
being NP-complete and widely regarded as intractable in
general.
%add citations from stephen cook's paper and the SAT competition
This has perplexed both theoreticians and solver developers alike over
the last two decades. A commonly proposed explanation is that these
solvers somehow exploit the underlying structure inherent in
industrial instances. Previous work has attempted to identify a
variety of structural parameters, such as
backdoors~\cite{Williams2003,szeider2003fixed,Dilkina2014}, community
structure modularity \cite{Ansotegui2012,newsham2014impact}, and
treewidth~\cite{Mateescu2011}. Additionally, researchers have
undertaken limited studies to correlate the size/quality measures of
these parameters with CDCL SAT solver runtime. For example, Newsham et
al.~\cite{newsham2014impact} showed that there is moderate correlation
between the runtime of CDCL SAT solvers and modularity of community
structure of industrial instances. Others have shown that certain
classes of crafted and industrial instances often have favorable
parameter values, such as small backdoor sizes
\cite{Dilkina2014,Kilby2005,Li2011,Williams2003}.

%There are several reason for trying to understand why SAT solvers work
%as well as they do on industrial instances, and what if any structure
%they exploit: first and foremost is the scientific motivation. A
%common refrain about heuristics in computer science is that we rarely
%fully understand why and under what circumstances they work
%well. 

There are several reason for trying to understand why SAT solvers work as well as they do on industrial instances, and what, if any, structure they exploit. First and foremost is the scientific motivation: a common refrain about heuristics in computer science is that we rarely fully understand why and under what circumstances they work well.
Second, a deeper understanding of the relationship between the
power of SAT heuristics and the structure of instances over which they
work well can lead us to develop better SAT solvers. Finally, we hope
that this work will eventually lead to new parameterized
complexity results relevant to classes of industrial instances.

Before we get into the details of our empirical study, we briefly
discuss several principles that guided us in this work: first, we
wanted our study to be comprehensive both in terms of the parameters
as well as the large size and variety of benchmarks considered.  This
approach enabled us to compare the explanatory strengths of different
parameters in a way that previous studies could not. Also, the large
scale and variety of benchmarks allowed us to draw more general
conclusions than otherwise. Second, we were clear from the outset that
we would be agnostic to the type of correlations (strong or moderate,
positive or negative) obtained, as poor correlations are crucial in
ruling out parameters that are not explanatory. Third, parameter
values should enable us to distinguish between industrial and crafted
instances.

Although many studies of these parameters have been performed in
isolation, a comprehensive comparison has not been performed between
them. A primary reason for this is that most of these parameters are
difficult to compute -- often NP-hard -- and many take longer to
compute than solving the original formula. Further, certain parameters
such as \textit{weak} backdoor size are only applicable to satisfiable
instances \cite{Williams2003}. Hence, such parameters have often been
evaluated on incomparable benchmark sets, making a proper comparison
between them difficult. We correct this issue in our study by focusing
on instances found in previous SAT competitions, specifically from the
Application, Crafted, and Agile tracks \cite{satcomps}. These
instances are used to evaluate state-of-the-art SAT solvers on a
yearly basis. Application instances are derived from a wide variety of
sources and can be considered a small sample of the types of SAT
instances found in practice, such as from verification
domains. Crafted instances mostly contain encodings of
combinatorial/mathematical properties, such as the pigeon-hole
principle or pebbling formulas. While many of these instances are much
smaller than industrial instances, they are often very hard for CDCL
solvers. The Agile track evaluates solvers on bit-blasted
quantifier-free bit-vector instances generated from the whitebox fuzz
tester SAGE~\cite{godefroid2008automated}. In total, we consider
approximately 1200 application instances, 800 crafted instances, and
5000 Agile instances.

\vspace{0.2cm}
\noindent{\bf Contributions.} We make the following four key
contributions in this paper:
%\footnote{Due to space limitations, we only include proof sketches for Sections \ref{sec_lsr_algorithms} and \ref{sec_lsr_theory}. In the interest of not including an overly long appendix, we refer to an extended technical report at the anonymous link in \cite{extended_paper_link}.}

\begin{enumerate}
\item We perform a large scale evaluation of several structural
  parameters on approximately 7000 SAT instances obtained from a wide variety
  of benchmark suites, and relate them to CDCL solver performance. We
  show moderate correlations to solving time for certain combinations
  of features, and very high correlations for the Agile benchmark. We
  further show that application and Agile instances have significantly
  better structural parameter values compared to crafted instances. To
  the best of our knowledge, this is first such comprehensive
  study. (Refer Section~\ref{sec_sat_analysis})
  
\item We introduce a new structural parameter, which we call learning-sensitive with restarts (LSR) backdoors, and describe a novel
  algorithm for computing upper bounds on minimum LSR-backdoor sizes, using the concept of
  clause absorption from \cite{atserias2011clause}. The LSR-backdoor
  concept naturally extends the idea of learning-sensitive (LS)
  backdoors introduced by Dilkina et al.~\cite{Dilkina2009a} by taking
  into account restarts, a key feature of CDCL SAT solvers. (Refer
  Background Section~\ref{sec:background} and
  Section~\ref{sec_lsr_algorithms})

\item We show how these structural parameters can be used as a lens to
  compare various solving heuristics, with a current focus on restart
  policies.  For example, we show that the ``Always Restart'' policy
  not only produces the smallest backdoors (with respect to the algorithm we use from Section \ref{sec_lsr_algorithms}), but also has the fastest
  runtime for a class of instances. We hope that our work can be used
  as a guide by theorists and SAT solver developers to rule out the
  study of certain types of parameters (and rule in new types of
  parameters) for understanding the efficiency of CDCL SAT
  solvers. (Refer Section~\ref{sec_sat_analysis})

\item We mathematically prove that minimal LSR-backdoors can be
  exponentially smaller than LS-backdoors for certain formulas. (Refer
  Section~\ref{sec_lsr_theory})
\end{enumerate}


==> tables/laser_algorithms.tex <==
\section{Computing LSR-Backdoors}
\label{sec_lsr_algorithms}

Dilkina et al.~\cite{Dilkina2009,Dilkina2014} incorporated clause
learning into the concept of strong backdoors 
%and thus introduced the concept of 
by introducing LS-backdoors, and additionally described an approach for
empirically computing upper bounds on minimal LS-backdoors.
We refer the reader to our [anonymized] extended technical report for complete proofs \cite{extended_paper_link}.


We propose a new concept called learning-sensitive with restarts (LSR)
backdoors and an approach that takes advantage of allowing restarts
which can often greatly reduce the number of decisions necessary to
construct such a backdoor especially if many ``unnecessary'' clauses
are derived during solving. Our key insight is that, as stated in
\cite{ansotegui2015using,oh2015between}, most learnt clauses are 
ultimately not used to determine SAT or UNSAT, and therefore we only need
to consider variables required to derive such ``useful'' clauses. Our
result shows that, for an unsatisfiable formula, the set of variables
within the set of learnt clauses in the UNSAT proof constitutes an
LSR-backdoor. The result for satisfiable formulas shows that the set
of decision variables in the final trail of the solver, along with the
variables in certain learnt clauses, constitute an
LSR-backdoor. Before describing result, we first recall the properties
of \textit{absorption}, \textit{1-empowerment}, and
\textit{1-provability}, which were initially used to demonstrate that
CDCL can simulate general resolution within some polynomial-size
bound:

\begin{definition}[Absorption \cite{atserias2011clause}]
  Let $\Delta$ be a set of clauses, let $C$ be a non-empty clause and
  let $x^\alpha$ be a literal in $C$. Then $\Delta$ absorbs $C$ at
  $x^\alpha$ if every non-conflicting state of the solver that
  falsifies $C \setminus \{x^\alpha\}$ assigns $x$ to $\alpha$. If
  $\Delta$ absorbs $C$ at every literal, then $\Delta$ absorbs $C$.
\end{definition}
	
The intuition behind absorbed clauses is that adding an already
absorbed clause $C$ to $\Delta$ is in some sense redundant, since any
unit propagation that could have been realized with $C$ is already
realized by clauses in $\Delta$.
	
\begin{definition}[1-Empowerment \cite{pipatsrisawat2008new}]
  Let $\alpha \Rightarrow l$ be a clause where $l$ is some literal in
  the clause and $\alpha$ is a conjunction of literals. The clause is
  1-empowering with respect to a set of clauses $\Delta$ if:
  \begin{enumerate}
  \item $\Delta \models (\alpha \Rightarrow l)$: the clause is implied
    by $\Delta$.
  \item $\Delta \wedge \alpha$ does not result in a conflict
    detectable by unit propagation.
  \item $\Delta \wedge \alpha \not \vdash_{1} l$: unit propagation
    cannot derive $l$ after asserting the literals in $\alpha$.
  \end{enumerate} 
\end{definition}
	
\begin{definition}[1-Provability \cite{pipatsrisawat2009power}]
  Given a set of clauses $\Delta$, a clause $C$ is 1-provable with
  respect to $\Delta$ \textit{iff} $\Delta \wedge \neg C \vdash_{1}
  false$.
\end{definition}
		
An important note is that every learnt clause is both 1-empowering and
1-provable, and therefore not absorbed, at the moment it is derived by
a CDCL solver (i.e., before being added to $\Delta$)
\cite{pipatsrisawat2008new,pipatsrisawat2009power}.
%% \footnote{This result requires that the clause learning algorithm
%%   only produces \textit{asserting clauses}, which is the case for
%%   the 1st-UIP algorithm~\cite{moskewicz2001chaff}.}
	
	
\begin{lemma}
  \label{absorb-lemma}		 
  Let $\Delta$ be a set of clauses and suppose that C is a
  1-empowering and 1-provable clause with respect to $\Delta$. Then
  there exists a sequence $\sigma$ of decisions and restarts
  containing only variables from C such that $\Delta$ and the set of
  learned clauses obtained from applying $\sigma$ absorbs C.
\end{lemma}
\begin{proof} 
  The proof follows directly from the construction of such a decision
  sequence in the proof of Proposition 2 of
  \cite{pipatsrisawat2009power}.
\end{proof}	

%\input{lsr_proof_notation_figure}

Our result additionally makes use of the following notation.  Let $F$
be a formula and $S$ be a CDCL solver. We denote the full set of
learnt clauses derived during solving as $S_L$. For every
conflicting state, let $C^\prime$ denote the clause that will be
learned through conflict analysis.  We let $R_{C^\prime}$ be the set
of clauses on the conflict side of the implication graph used to
derive $C^\prime$ where $R_{C^\prime}^* = R_{C^\prime} \cup \bigcup_{C
  \in R_{C^\prime}} R_C^*$ recursively defines the set of clauses
needed to derive $C^\prime$ (where $R_{original\_clause}^* =
\emptyset$). For every learnt clause we define $D_{C^\prime}^* =
vars(C^\prime) \cup \bigcup_{C \in R_{C^\prime}^*} D_C^*$, where
$D_{original\_clause}^* = \emptyset$, as the set of variables in the
clause itself as well as any learnt clause used in the derivation of
the clause (recursively). Intuitively, $D_{C^\prime}^*$ is a
sufficient set of \textit{dependency variables}, such that a fresh SAT
solver can absorb $C^\prime$ by only branching on variables in the
set. For a set of clauses $\Delta$, we let $R_\Delta^* = \bigcup_{C\in
  \Delta} R_C^*$ and $D_\Delta^* = \bigcup_{C \in \Delta} D_C^*$.
%For reference, we include an example of the above notation in Appendix \ref{app_lsr_notation}.
% We
% defer full proofs of the lemmas below to the Appendix
% \ref{sec_appendix_proofs}. 

	
\begin{lemma}
Let $S$ be a CDCL solver used to determine the satisfiability of some
formula $F$. Let $\Delta \subseteq S_L$ be a set of clauses learned while solving $F$. Then a fresh solver $S^\prime$ can absorb
all clauses in $\Delta$ by only branching on the variables in
$D_{\Delta}^*$.
\label{lem_absorb_clauses}
\end{lemma}

\begin{sketch}
  Let $seq(R_\Delta^*)=\langle C_1, C_2, \ldots C_n \rangle$ be the
  sequence over $R_\Delta^*$ in the order that the original solver $S$
  derived the clauses, and suppose we have already absorbed the first
  $k-1$ clauses by only branching upon $D_{\{C_1, \ldots, C_{k-1}
    \}}^*$. Then, in particular, the clauses in $R_{C_k}$ have been
  absorbed, so $C_k$ must be 1-provable. If $C_k$ is not 1-empowering,
  then it is absorbed and we are done. If $C_k$ is 1-empowering, we
  can invoke Lemma \ref{lem_absorb_clauses} to absorb $C_k$ by only
  branching on variables in $C_k$, and $vars(C_k) \subseteq
  D_\Delta^*$ by construction.
\end{sketch}

\begin{theorem}[LSR Computation, SAT case]
  \label{thm_lsr_sat}
  Let $S$ be a CDCL solver, $F$ be a satisfiable formula, and $T$ be
  the final trail of the solver immediately before returning SAT,
  which is composed of a sequence of decision variables $T_D$ and
  propagated variables $T_P$. For each $p\in T_P$, let the clause used
  to unit propagate $p$ be $l_p$ and the full set of such clauses be
  $L_P$.  Then $B = T_D \cup D_{L_p}^*$ constitutes an LSR-backdoor
  for $F$.
\end{theorem}
\begin{sketch}
  Using Lemma \ref{lem_absorb_clauses}, we first absorb all clauses in
  $L_P$ by branching on $D_{L_P}^*$.  We can then restart the solver
  to clear the trail, and branch on the variables in $T_D$, using the
  same order and polarity as the final trail of $S$. Since we have
  absorbed each $l_p$, every $p$ will be propagated.
\end{sketch}
	
%% As an optimization for the SAT case, note that in Theorem
%% \ref{thm_lsr_sat} we always include the dependency variables
%% $D_{l_p}^*$ needed to propagate $p$. We could instead just branch on
%% $p$ without deriving $l_p$, which may reduce backdoor size if
%% $D_{l_p}^*$ is large. More specifically, we choose the backdoor set $B
%% = min(\{X \mid T_D \subseteq X \wedge \forall_{p \in T_P}(D_{l_p}^*
%% \subseteq X \vee p \in X)\})$, which we compute through a reduction to
%% MaxSAT. We use this optimization for our data in Section
%% \ref{sec_sat_analysis}. We also note that algorithms used to minimize
%% weak backdoors, such as in \cite{Li2011}, can also be used for
%% satisfiable LSR-backdoors. We plan to incorporate their minimization
%% techniques in future work.
	
\begin{theorem}[LSR Computation, UNSAT case]
  \label{thm_lsr_unsat}
  Let $S$ be a CDCL solver, $F$ be an unsatisfiable formula, and
  $\Delta \subseteq S_L$ be the set of learnt clauses used to derive
  the final conflict.  Then $D_{\Delta}^*$ constitutes an LSR-backdoor
  for $F$.
\end{theorem}
\begin{proof}
  The result follows similarly to the satisfiable
  case. We learn all clauses relevant to the proof using
  Lemma \ref{lem_absorb_clauses}, which then allows unit
  propagation to derive UNSAT.
\end{proof}

We make some observations about our approach. First, our approach can
be easily lifted to any learning scheme other than the 1st-UIP scheme
that is currently the most widely used one.  Second, the set of
variables that constitute an LSR-backdoor may be disjoint from
the set of decisions made by the solver.  Third, the above approach
depends on the ability to restart, and therefore cannot be used to
compute LS-backdoors. In particular, the construction of the decision
sequence for Lemma \ref{absorb-lemma}, as described in
\cite{pipatsrisawat2009power}, requires restarting after every
conflict.  As an additional remark of practical importance, modern
CDCL solvers often perform clause minimization to shrink a newly
learnt clause before adding it to the clause database
\cite{sorensson2009minimizing}, which can have a significant impact on
performance. Intuitively, this procedure reduces the clause by finding
dependencies among its literals.  In order to allow clause
minimization in our experiments, for each clause $C$ we include all
clauses used by the minimizer in our set $R_{C}$.

For our empirical results, we modified an off-the-shelf solver
MapleSat \cite{liang2016learning}, by annotating each learnt clause $C^\prime$
with $D_{C^\prime}^*$. Note that we do not need to explicitly record
the set $R_{C^\prime}^*$ at any time.  As in the LS-backdoor
experiments in \cite{Dilkina2009}, different LSR-backdoors can be
obtained by randomizing the branching heuristic and polarity
selection. However, given the size and number of instances considered
here, we only perform one run per instance.

To ensure that our output is indeed an LSR-backdoor, we implemented a
verifier that works in three phases. First, we compute an LSR-backdoor
$B$ as above. Second, we re-run the solver, and record every learnt
clause $C$ such that $D_C^* \subseteq B$. We then run a final solver
with a modified branching heuristic, that iterates through the
sequence of learnt clauses from phase 2, absorbing each as described
in Lemma \ref{lem_absorb_clauses} (first checking that the clause is
either absorbed or 1-provable upon being reached in the sequence). We
ensure that the solver is in a final state by the end of the sequence.


==> tables/laser_figures.tex <==
	
	\todo{DependencyList is a mapping from vars to the decision vars needed to derive it (and all of its deriving clauses, recursively).}
	
	\begin{figure}[t]
		\renewcommand\algorithmicthen{}
		\renewcommand\algorithmicfunction{}
		\begin{algorithmic}[1]
			\Function{Laser\_a}{Vars finalDecs, DependencyList depList} 
			\State $B = finalDecs$ 	
			\For{$v \in AllVars \setminus finalDecs$} \Comment{Optimized with ``workpool''}
			\State $B = B \cup depList[v]$
			\EndFor
			\State \Return {$B$}
			
			\EndFunction
		\end{algorithmic}
		\caption{Current version.}
		\label{cas-preds}
	\end{figure}
	
	\begin{figure}[H]
		\renewcommand\algorithmicthen{}
		\renewcommand\algorithmicfunction{}
		\begin{algorithmic}[1]
			\Function{Laser\_b}{Vars finalDecs, DependencyList depList} 
			\State $S = Solver() $ 
			\For{$v$ in $AllVars$}
			\State $createSolverBool(v_b)$ \Comment{True if $v$ is in the LSR backdoor $B$.}
			\State $createSolverBool(v_i)$ \Comment{True if $parents(v)$ are all implied, or $v \in B$.}
			
			\EndFor
			
			\For{$v \in AllVars$}
			\State $S.assert(v_i)$
			\If $v \in finalDecs$
			\State $S.assert(v_B)$
			\Else
			\State $S.assert(\bigwedge_{p\in parents(v)} p_i \vee v_B )$
			\EndIf
			\EndFor
			\State $objectiveFunc = \sum_{v \in AllVars} b2i(v_B) $
			\State $model = S.minimize(objectiveFunc)$
			\State $B = \{v \mid model[v_B]\}$
			\State \Return {$B$}
			
			\EndFunction
		\end{algorithmic}
		\caption{Basically the idea is that for every non-final decision var, we have a choice of either including it, or all of its dependencies. \texttt{b2i(v)} is a macro for \texttt{If(v, 1, 0)}.}
		\label{cas-preds}
	\end{figure}
	
	%Note -- Graph abstraction based approach (maybe -- could be able to perform better heuristics with graph structure -- basically a dependency graph with nodes and clauses)
		

	\begin{figure}[H]
		\renewcommand\algorithmicthen{}
		\renewcommand\algorithmicfunction{}
		\begin{algorithmic}[1]
			\Function{\textbf{struct} State}{}
				\State{set$<$Clause$>$ learnts}
				\State{vector$<$Lit$>$ trail} 
			\EndFunction
			\State{}
			
			\Function{\textbf{def} isBackdoor}{Formula F, Vars V, bool withRestarts} 
			\LeftComment{Performs BFS over all decision sequences, pruning as necessary.}
			
			\State{Queue$<$State$>$ Q}
			\State{Set$<$State$>$ seenStates}
			\State{Q.push(EmptyState)}
			
			\While{$\neg$Q.empty()}
				\State State state = Q.pop()
				\State Solver solver = generateCleanMiniSAT$^{-}$(F)	
				\State \Comment{for now, learned unit clauses get put at beginning of trail}
				\State solver.updateLearnts(state.learnts)
				\State success = solver.solveWithTrail(state.trail)
				\If{}success
				\State \Return true
				\Else \Comment{Solver is in a failed state. Generate new decision branches.}
				\For{$v \in $ solver.unassignedVars $\cap$ V}
					\State Q.pushIfUnseen(new State(solver.learnts, solver.trail + ($\neg$v)))
					\State Q.pushIfUnseen(new State(solver.learnts, solver.trail + (v)))
					\If withRestarts and ``just learned clause''
					\State Q.pushIfUnseen(new State(solver.learnts, EmptyTrail))
					\EndIf
					
					
				\EndFor
				\EndIf
				
			\EndWhile
			
			
			\EndFunction
			\State{}
			\Function{\textbf{def} MinimumBackdoor}{Formula F, bool withRestarts} 
			\For{$k = 1 \ldots nVars()$}
			\For{every set $V$ of $k$ variables}
				\If{}isBackdoor(F, V, withRestarts)
				\State return V
				\EndIf
			\EndFor
			\EndFor
			\EndFunction
		\end{algorithmic}
		\caption{Solver$^-$: turns off periodic restarts and clause deletion. Takes as input a sequence of literals to be used for branch selection. If the sequence is exhausted and the solver has not determined SAT/UNSAT, returns unknown.}
		\label{cas-preds}
	\end{figure}
	
	Minimum LS Notes:
	\begin{itemize}
		\item if k == nVars, would compute the smallest possible number of decisions needed to decide F.
	\end{itemize}
\suppress{
	\todo{garbage:	
		For the first learnt clause $c_0$, $D_{c_0}$ can clearly be used to derive the clause from the initial state.
		For an arbitrary learnt clause $c^\prime$, we must reconstruct $R_{c^\prime}$ by only branching on variables $V_{c^\prime}$. Let $L_{full}$ be the full set of clauses derived by $S$ up to this point, and for any learnt clause $c$, let $L_c$ be the  that were used to derive any clause in $R_{c^\prime}$ \todo{include recursive clauses, dont know how to state}.
	}
	
	
	
	\todo{consider the set of clauses from S that recursively derive that of c', and ignore the rest}
	
	\todo{suppose there are n lc clauses used in R. Use S to get proof of r0, to derive r1, note that any learnts inbetween r0 and r1 cannot contribute to learning c' since they are not in R by our lc ordering ....if any intermediate exists theyll show up in the R for lc, but their vars will be accounted for}
	
	\todo{suppose by induction that for each lc in R, we can derive it from initial with Vlc, need to show we can derive all learnt clauses needed to derive c', use S somehow}
	
	\todo{finish...} 
	Starting from an initial solver state, our approach is to first derive all learnt clauses in $C$, and then use the decisions from $D$ to derive $c^\prime$. Note that the run of the solver $S$ up to the current point does not necessarily demonstrate that $V_{c^\prime}$ adheres to its desired property, since $S$ may have branched on other variables, or derived additional clauses not in $C$.
	
	Let $L$ be the set of learnt clauses in $C$, and $\sigma_L$ be a sequence over $L$ indicating the order in which $S$ learned the clauses. We derive the clauses in $L$ in the same order as witnessed by $S$. 
	
	
	Suppose we have already derived all clauses in $C$. By construction, each clause $c \in CS \cup RS$ can be derived by a SAT solver using only variables in $V_c$ %(as witnessed by the current run of the SAT solver up to the current conflict). 
	Note that for the $c^\prime$ under question, the current solver state cannot be directly used to complete the proof, as other branching decisions and learnt clauses may have been found by the solver that were not involved in the current conflict.
	Let $L_D$ be the literals used in the current conflict analysis corresponding to the variables in $D$.
	To derive 
	By assigning the variables in $D$ in the same order and polarity as the current state of the solver, unit propagation will the clauses in , unit propagation   \todo{finish}
}

==> tables/ls_vs_lsr_sep.tex <==
\suppress{
Let $n$ be a positive integer and let $X = \set{x_1, x_2, \ldots, x_n}$ be a set of boolean variables.
For any boolean variable $x$, let $x^1$ denote the positive literal $x$ and $x^{0}$ denote the negative literal $\neg x$.
For any assignment $\alpha \in \set{0,1}^n$ let $C_\alpha = x_1^{1-\alpha_1} \vee x_2^{1-\alpha_2} \vee \ldots \vee x_n^{1-\alpha_n}$ denote the clause on $x$ variables which is uniquely falsified by the assignment $\alpha$.
The following CNF formula ${\cal F}$ was introduced for the purpose of separating \emph{strong backdoors} from \emph{learning sensitive backdoors}.
The formula is defined on the variables $x_1, x_2, \ldots, x_n$, and also three auxiliary sets of variables $\set{q_\alpha}_{\alpha \in \set{0,1}^n}, \set{a_\alpha}_{\alpha \in \set{0,1}^n}, \set{b_\alpha}_{\alpha \in \set{0,1}^n}$:
\begin{align*}
  {\cal F} = & \bigwedge_{\alpha \neq \vec 1} (C_\alpha \vee \neg q_\alpha) \wedge (q_\alpha \vee a_\alpha) \wedge (q_\alpha \vee b_\alpha) \wedge (q_\alpha \vee \neg a_\alpha \vee \neg b_\alpha) \\
  & \wedge \left(C_{\vec 1} \vee \bigvee_{\alpha \in \set{0,1}^n} \neg q_\alpha\right) \wedge (q_{\vec 1} \vee a_{\vec 1}) \wedge (q_{\vec 1} \vee b_{\vec 1}) \wedge (q_{\vec 1} \vee \neg a_{\vec 1} \vee \neg b_{\vec 1}).
\end{align*}
In this note we modify this formula to obtain a CNF formula providing an exponential separation between \emph{learning sensitive backdoors} and \emph{learning-sensitive backdoors with restarts}.
Throughout we implicitly assume that the clause learning algorithm is \emph{First UIP}.

\todo{eventually delete the formula above, and mention that the formula below is also from Dilkina}
Our formula will be defined by the following template.
Let ${\cal O}$ be an ordering of $\set{0,1}^n$; we write $<_{\cal O}$ to denote the relation induced by this ordering.
Given an ordering ${\cal O}$ we can define the formula \[{\cal F}_{\cal O} = \bigwedge_{\alpha \in \set{0,1}^n} (C_\alpha \vee \bigvee_{\alpha' \leq_{\cal O} \alpha} \neg q_{\alpha'}) \wedge (q_\alpha \vee a_\alpha) \wedge (q_\alpha \vee b_\alpha) \wedge (q_\alpha \vee \neg a_\alpha \vee \neg b_\alpha).\]

\begin{lemma}
  Let ${\cal O}$ be any ordering of $\set{0,1}^n$.
  The $X$-variables form a learning-sensitive backdoor with restarts for the formula ${\cal F}_{\cal O}$.
\end{lemma}
\begin{proof}
  Query the $x$ variables according to the ordering given by ${\cal O}$.
  As soon as we have a complete assignment to the $x$ variables, we will unit-propagate to a conflict and learn a $q_\alpha$ variable as a conflict clause; after that we restart.
  Once all such assignments are explored we can simply query the $X$ variables in any order (without restarts) to yield a contradiction, since every assignment to the $X$ variables will falsify the formula.
\end{proof}

Given two orderings ${\cal O}_1, {\cal O}_2$ let $d({\cal O}_1, {\cal O}_2)$ denote the Hamming distance of these two sequences (as sequences).
For instance the Hamming distance of the two sequences $(00, 01, 10, 11)$ and $(00, 10, 01, 11)$ is $2$.
Finally, consider any decision tree $T$ of depth $n$ where we have queried the $X$ variables in \emph{any} order in the tree $T$.
From this tree we obtain a natural ordering ${\cal O}(T)$ of $\set{0,1}^n$ by reading off the strings labelling the leaves in left-to-right order.
Note that the orderings of the form ${\cal O}(T)$ are \emph{exactly} the orderings which can be generated by DPLL algorithms (or, more generally, a CDCL algorithm without restarts).
}

\begin{lemma}\label{lem:main}
  Let ${\cal O}$ be any ordering of $\set{0,1}^n$, and let ${\cal T}_X$ denote the collection of all complete depth-$n$ decision trees on $X$ variables.
  Then any LS-backdoor of ${\cal F}_{\cal O}$ has size at least \[n + \min_{T \in {\cal T}_X} d({\cal O}, {\cal O}(T)).\]
\end{lemma}
\begin{proof}
  Let $B$ be a minimal learning-sensitive backdoor of ${\cal F}_{\cal O}$.
  Let $Q = \set{q_\alpha}_{\alpha \in \set{0,1}^n}$.
  Without loss of generality we can assume that $B \subseteq X \cup Q$, as a learning sensitive backdoor which queries $a_\alpha$ or $b_\alpha$ variables can be replaced with a backdoor querying $q_\alpha$ variables which is no larger.
  Furthermore, we can assume that $X \subseteq B$.
  To see this, observe first that $Q$ is \emph{not} a learning sensitive backdoor of ${\cal F}_{\cal O}$, since querying all assignments to the $Q$ variables will leave the algorithm in an inconclusive state.
  \todo{potential issue -- I think we only need n - 1 of the X variables, since if we already derived the necessary q's, we propagate the final x for free}
  It follows that $B$ must contain \emph{some} $X$ variable; to see that it contains \emph{all} $X$ variables, it is enough to observe that in order to hit a conflict (even after querying all $Q$ variables) we must assign a value to every $X$ variable by the structure of ${\cal F}_{\cal O}$.
  Thus $X \subseteq B \subseteq X \cup Q$ (and $|X|$ represents the $n$ term in the statement of the lemma).
    
  Furthermore, observe that we can always assume that if the algorithm queries a $q_\alpha$ variable as a decision variable, then it queries the variable negatively first.
  This is because querying $\neg q_\alpha$ will cause the CDCL algorithm to hit a conflict and learn the unit clause $q_\alpha$, so we may replace such ``positive'' queries \emph{in-situ} with negative queries without affecting the simulation of the backdoor queries.
  In turn, this implies that we may assume that all $q_\alpha$ variables occurring in the backdoor are queried at the beginning of the algorithm, leaving only queries to $X$ variables.
  Since all $q_\alpha$ variables in the backdoor $B$ are queried at the beginning of the algorithm without loss of generality, by the structure of ${\cal F}_{\cal O}$ we can see that once we start querying $X$ variables, we will only hit a conflict once we have assigned values to \emph{all} of the $X$ variables.
  This implies that the query order for the $X$ variables takes the form of a complete depth-$n$ decision tree $T \in {\cal T}_X$, using the notation in the statement of the lemma.

  With this, we can prove that every clause learned by the algorithm is a unit clause of the form $q_\alpha$ for some $\alpha \in \set{0,1}^n$.
  To see this, consider any time that we have hit a conflict in the process of simulating the variable queries of the backdoor $B$.
  If we have hit a conflict from querying $\neg q_\alpha$, as described above, we are done, so suppose otherwise.
  By assumption, the only variables that $B$ contains other than $Q$ variables are $X$ variables, thus, to hit a conflict we must have queried all of the $X$ variables by the structure of ${\cal F}_{\cal O}$.
  In such a case, since we have not queried $\neg q_\alpha$ for any $\alpha$, we must have unit-propagated $\neg q_\alpha$ for some $\alpha$ by the structure of ${\cal F}_{\cal O}$.
  This will hit a conflict and learn the unit clause $q_\alpha$, proving our claim.

  Recalling that $X \leq B \leq X \cup Q$, to prove the lemma it suffices to prove that \[|B \cap Q| \geq \min_{T \in {\cal T}_X} d({\cal O}, {\cal O}(T)) \] since $|X| = n$.
  Since $B$ is a backdoor, it must be that at every leaf of the tree $T$ the unit propagator will propagate the input to a conflict.
  Consider the ordering of the assignments ${\cal O}(T)$ induced by this tree $T$.
  At each leaf of this tree, which corresponds to an assignment $\alpha$ to the $X$ variables, there are two possibilities: either we learn the unit clause $q_\alpha$ or not.
  By the structure of ${\cal F}_{\cal O}$, we can only learn the unit clause $q_\alpha$ at the leaf if we have learned the unit clauses $q_{\alpha'}$ for each $\alpha' \leq_{{\cal O}} \alpha$.
  Thus, for any index in the orderings ${\cal O}(T)$ and ${\cal O}$, if the index has different strings in the respective orderings, it follows that we will not be able to learn the unit clause $q_\alpha$, and so we will have to query at least one extra variable from $Q$ in the backdoor $B$.
  This proves that \[|B \cap Q| \geq \min_{T \in {\cal T}_X} d({\cal O}, {\cal O}(T)) \] and therefore the lemma.
\end{proof}

By the previous lemma, to lower bound the size of the learning sensitive backdoor it suffices to find an ordering ${\cal O}$ of $\set{0,1}^n$ which is far in hamming distance from \emph{every} ordering of the form ${\cal O}(T)$ for some complete decision tree $T \in {\cal T}_X$ on the $X$ variables.

\begin{lemma}
  There exists an ordering ${\cal O}$ of $\set{0,1}^n$ such that for every decision tree $T \in {\cal T}_X$ we have \[ d({\cal O}, {\cal O}(T)) \geq 2^{n-1}.\]
\end{lemma}
\begin{proof}
  Let $N = 2^n - 1$ and write ${\cal O}(T) = \alpha_0, \alpha_1, \ldots, \alpha_N$.
  We use the following key property of orderings generated from decision trees:

  \spcnoindent
  {\bf Key Property.} For all $j = 0, 1, \ldots, N/2 - 1$, the strings $\alpha_{2j}, \alpha_{2j+1}$ differ at exactly one coordinate.

  \spcnoindent
  This property is easy to prove: every node in the decision tree $T$ which is the parent of a leaf is labeled with some variable $x_i$; it follows that both leaves below it differ exactly on the coordinate indexed by $x_i$.
  To use this property, recall that a \emph{Gray ordering} of $\set{0,1}^n$ is any ordering ${\cal O} = g_0, g_1, \ldots, g_{N-1}$ where for all $i = 0, 1, \ldots, N-2$ the strings $g_i$ and $g_{i+1}$ differ on exactly one coordinate.
  Observe that this immediately implies that $g_i$ and $g_{i+2}$ have Hamming distance exactly 2 for each $i$ --- this is because $d(g_i, g_{i+1}) = d(g_{i+1}, g_{i+2}) = 1$ and we could not have flipped the same coordinate twice to get from $g_i$ to $g_{i+1}$ to $g_{i+2}$.
  So, given any Gray ordering ${\cal O}$ of $\set{0,1}^n$, define the ordering ${\cal O}'$ by taking the ordering ${\cal O}$ and swapping the positions of the strings $g_{2j+1}$ and $g_{2j + 2}$ for all $j = 0, 1, \ldots, N/2 - 2$, and let \[ {\cal O}' = g_0', g_1', \ldots, g_{N-1}'\] after doing this swap.
  By what we have argued above, for any decision tree $T$ and all $j = 0, 1, \ldots, N/2 - 1$ at least one of the pairs of strings $\alpha_{2j}, g'_{2j}$ and $\alpha_{2j+1}, g'_{2j+1}$ must be mismatched, implying the lemma.
\end{proof}
\suppress{
\begin{corollary}
  There exists an ordering ${\cal O}$ such that any learning-sensitive backdoor for the formula ${\cal F}_{\cal O}$ has size at least $n + 2^{n-1}$.
\end{corollary}
}



==> tables/ls_vs_lsr_sep_v2.tex <==


Let $n$ be a positive integer and let $X = \set{x_1, x_2, \ldots, x_n}$ be a set of boolean variables.
For any boolean variable $x$, let $x^1$ denote the positive literal $x$ and $x^{0}$ denote the negative literal $\neg x$.
For any assignment $\alpha \in \set{0,1}^n$ let $C_\alpha = x_1^{1-\alpha_1} \vee x_2^{1-\alpha_2} \vee \ldots \vee x_n^{1-\alpha_n}$ denote the clause on $x$ variables which is uniquely falsified by the assignment $\alpha$.
\suppress{
The following CNF formula ${\cal F}$ was introduced for the purpose of separating \emph{strong backdoors} from \emph{learning sensitive backdoors}.


The formula is defined on the variables $x_1, x_2, \ldots, x_n$, and also three auxiliary sets of variables $\set{q_\alpha}_{\alpha \in \set{0,1}^n}, \set{a_\alpha}_{\alpha \in \set{0,1}^n}, \set{b_\alpha}_{\alpha \in \set{0,1}^n}$:
\begin{align*}
  {\cal F} = & \bigwedge_{\alpha \neq \vec 1} (C_\alpha \vee \neg q_\alpha) \wedge (q_\alpha \vee a_\alpha) \wedge (q_\alpha \vee b_\alpha) \wedge (q_\alpha \vee \neg a_\alpha \vee \neg b_\alpha) \\
  & \wedge \left(C_{\vec 1} \vee \bigvee_{\alpha \in \set{0,1}^n} \neg q_\alpha\right) \wedge (q_{\vec 1} \vee a_{\vec 1}) \wedge (q_{\vec 1} \vee b_{\vec 1}) \wedge (q_{\vec 1} \vee \neg a_{\vec 1} \vee \neg b_{\vec 1}).
\end{align*}
In this note we modify this formula to obtain a CNF formula providing an exponential separation between \emph{learning sensitive backdoors} and \emph{learning-sensitive backdoors with restarts}.
}
Throughout we implicitly assume that the clause learning algorithm is \emph{1st-UIP}.

Our formula will be defined by the following template.
Let ${\cal O}$ be an ordering of $\set{0,1}^n$; we write $<_{\cal O}$ to denote the relation induced by this ordering.
Given an ordering ${\cal O}$ we can define the formula \[{\cal F}_{\cal O} = \bigwedge_{\alpha \in \set{0,1}^n} (C_\alpha \vee \bigvee_{\alpha' \leq_{\cal O} \alpha} \neg q_{\alpha'}) \wedge (q_\alpha \vee a_\alpha) \wedge (q_\alpha \vee b_\alpha) \wedge (q_\alpha \vee \neg a_\alpha \vee \neg b_\alpha).\]

\begin{customlemma}{3}
  Let ${\cal O}$ be any ordering of $\set{0,1}^n$.
  The $X$-variables form a learning-sensitive backdoor with restarts for the formula ${\cal F}_{\cal O}$.
\end{customlemma}
\begin{proof}
  Query the $x$ variables according to the ordering given by ${\cal O}$.
  As soon as we have a complete assignment to the $x$ variables, we will unit-propagate to a conflict and learn a $q_\alpha$ variable as a conflict clause; after that we restart.
  Once all such assignments are explored we can simply query the $X$ variables in any order (without restarts) to yield a contradiction, since every assignment to the $X$ variables will falsify the formula.
\end{proof}

% Given two orderings ${\cal O}_1, {\cal O}_2$ let $d({\cal O}_1, {\cal O}_2)$ denote the Hamming distance of these two sequences (as sequences).
% For instance the Hamming distance of the two sequences $(00, 01, 10, 11)$ and $(00, 10, 01, 11)$ is $2$.
Consider any decision tree $T$ of depth $n$ where we have queried the $X$ variables in \emph{any} order in the tree $T$.
From this tree we obtain a natural ordering ${\cal O}(T)$ of $\set{0,1}^n$ by reading off the strings labelling the leaves in left-to-right order.
Note that the orderings of the form ${\cal O}(T)$ are \emph{exactly} the orderings which can be generated by DPLL algorithms (or, more generally, a CDCL algorithm without restarts).
For any such complete decision tree $T$ and any ordering ${\cal O}$ of $\set{0,1}^n$, define \[ d({\cal O}, {\cal O}(T)) = |\set{\alpha' \in \set{0,1}^n \st \exists \alpha \in \set{0,1}^n : \alpha' <_{\cal O} \alpha, \alpha <_{{\cal O}(T)} \alpha'}|.\]
That is, $d({\cal O}, {\cal O}(T))$ is the number of strings $\alpha'$ which are ``out of order'' in ${\cal O}(T)$ with respect to ${\cal O}$.

\begin{customlemma}{4}\label{lem:main}
  Let ${\cal O}$ be any ordering of $\set{0,1}^n$, and let ${\cal T}_X$ denote the collection of all complete depth-$n$ decision trees on $X$ variables.
  Then any learning-sensitive backdoor of ${\cal F}_{\cal O}$ has size at least \[\min_{T \in {\cal T}_X} d({\cal O}, {\cal O}(T)).\]
\end{customlemma}
\begin{proof}
  Let $B$ be a minimal learning-sensitive backdoor of ${\cal F}_{\cal O}$.
  Let $Q = \set{q_\alpha}_{\alpha \in \set{0,1}^n}$.
  First we show that without loss of generality the following holds:
  \begin{enumerate}
  \item $B \subseteq X \cup Q$.
  \item All queries to $Q$-variables occur before any query to an $X$-variable.
  \end{enumerate}
  We begin with an observation: any query to a variable $q_\alpha$ can be assumed to be of the form $q_\alpha = F$.
  To see this, notice that querying $q_\alpha = F$ will immediately unit propagate to a conflict, and 1UIP-learning will immediately yield the unit clause $q_\alpha$.
  Thus we can always replace queries of the form $q_\alpha = T$ \emph{in-situ} with queries $q_\alpha = F$ without affecting the rest of the algorithm's execution.

  Let us first show that $B \subseteq X \cup Q$.
  Suppose that there is a variable $a_\alpha \in B$ (the case where $b_\alpha \in B$ is symmetric).
  We show that $a_\alpha$ can be replaced with $q_\alpha$.
  Consider the first time that $a_\alpha$ is queried as a decision variable.
  By the structure of ${\cal F}_{\cal O}$, we can assume that $q_\alpha$ has not been assigned before querying $a_\alpha$ as a decision variable (as we have shown above, if this is the case then $q_\alpha = T$, which eliminates the two clauses containing $a_\alpha$).
  If $a_\alpha = F$, then $q_\alpha = T$ is unit-propagated, and all clauses containing $a_\alpha$ or $b_\alpha$ will be removed.
  It follows that any conflict following this assignment must occur in a clause containing $C_{\alpha'}$ for some $\alpha'$, and thus replacing $a_\alpha$ with $q_\alpha$ will not affect the queries to the backdoor in this case.
  So, instead, suppose that $a_\alpha = T$.
  Clearly, in order for this assignment to have been necessary, the variable $q_\alpha$ must be assigned after assigning $a_\alpha$ (either by unit propagation or a decision).
  Observe that if $q_\alpha$ is set to true after assigning $a_\alpha = T$, then the two clauses containing $a_\alpha$ are removed and so assigning $q_\alpha = T$ to begin with would not have affected the execution of the algorithm on the backdoor.
  Similarly, setting $q_\alpha = F$ will unit propagate to a conflict in this case and we would learn the unit clause $q_\alpha = T$ as above, again showing that we could have replaced $a_\alpha$ with $q_\alpha$ without affecting the backdoor.
  Thus $a_\alpha$ can be replaced with $q_\alpha$ without loss of generality.

  Next we show that all decision queries to $Q$-variables can be made before queries to $X$-variables without loss of generality.
  As argued above, we can assume that when $q_\alpha$ is queried as a decision variable it is queried negatively (as this will lead immediately to learning the unit clause $q_\alpha$).
  Consider any conflict which occurs in the process of querying the variables of the backdoor that does not happen because of querying $\neg q_\alpha$.
  Since $B \subseteq X \cup Q$, by the structure of ${\cal F}_{\cal O}$ any such conflict must occur after assigning all $X$-variables to some string $\alpha \in \set{0,1}^n$.
  Corresponding to this total assignment $\alpha$ to the $X$-variables is the unique clause $C_\alpha$ which is falsified by this assignment, so consider the clause in ${\cal F}_{\cal O}$ of the form \[ C_\alpha \vee \bigvee_{\alpha' \leq_{\cal O} \alpha} \neg q_{\alpha'}.\]
  After assigning a subset of the $Q$-variables of $B$ and assigning all $X$-variables to $\alpha$ a conflict can occur in two ways:
  \begin{enumerate}
  \item $q_{\alpha'} = 1$ for all $\alpha' \leq_{\cal O} \alpha$ and the clause above is the conflict clause, or
  \item there exists a single $q_{\alpha^*}$ which is unassigned after assigning all of these variables; the above clause leads to assigning $q_{\alpha^*} = F$ and thus learning the unit clause $q_{\alpha^*}$, as argued above.
  \end{enumerate}
  In either case, moving all $q_\alpha$ queries to the beginning of the algorithm will not affect these conflicts: this is clear in case (1); in case (2) the only possibility is that $q_{\alpha^*}$ was queried at the beginning and so the conflict will change to a case (1) conflict.

  We are now ready to finish the proof of the lemma.
  We encode the execution of the CDCL algorithm as a decision tree, wherein we first query all $Q$-variables and then query all $X$-variables.
  Note that we must assign all $X$-variables to hit a conflict by the structure of ${\cal F}_{\cal O}$, and so we let $T$ denote the complete depth-$n$ decision tree querying the $X$-variables obtained from the CDCL execution tree.
  Recalling that $B \subseteq X \cup Q$, to prove the lemma it suffices to prove that \[|B \cap Q| \geq d({\cal O}, {\cal O}(T)).\]
  
  Since $B$ is a backdoor, it must be that at every leaf of the tree $T$ the unit propagator will propagate the input to a conflict.
  Consider the ordering of the assignments ${\cal O}(T)$ induced by this tree $T$.
  At each leaf of this tree, which corresponds to an assignment $\alpha$ to the $X$ variables, consider the clause \[ C_\alpha \vee \bigvee_{\alpha' \leq_{\cal O} \alpha} \neg q_{\alpha'}.\]
  There are two possibilities: either we learn a unit clause $q_{\alpha^*}$ for some $\alpha^* \leq_{\cal O} \alpha$ or we do not.
  If we have not then we must have already learned the unit clauses $q_{\alpha'}$ for all $\alpha' \leq_{\cal O} \alpha$.
  Otherwise, we must have learned the unit clauses $q_{\alpha'}$ for each $\alpha' \leq_{{\cal O}} \alpha$ satisfying $\alpha' \neq \alpha^*$.
  This implies that \[ B \cap Q \supseteq \bigcup_{\alpha \in \set{0,1}^n} \set{\alpha' \st \alpha' >_{{\cal O}(T)} \alpha, \alpha' \leq_{\cal O} \alpha},\] as for each $\alpha \in \set{0,1}^n$ we must query, at least, all variables $\alpha'$ which occur after $\alpha$ in ${\cal O}(T)$ but before $\alpha$ in ${\cal O}$.
  This proves the lemma.
\end{proof}

By the previous lemma, to lower bound the size of the learning sensitive backdoor it suffices to find an ordering ${\cal O}$ of $\set{0,1}^n$ for which any ordering ${\cal O}(T)$ produced by a decision tree has many ``inversions'' with respect to ${\cal O}$.

\begin{customlemma}{5}
  There exists an ordering ${\cal O}$ of $\set{0,1}^n$ such that for every decision tree $T \in {\cal T}_X$ we have \[ d({\cal O}, {\cal O}(T)) \geq 2^{n-2}.\]
\end{customlemma}
\begin{proof}
  Let $T \in {\cal T}_X$ be any decision tree.
  Let $N = 2^n$ and write ${\cal O}(T) = \alpha_1, \alpha_1, \ldots, \alpha_N$.
  We use the following key property of orderings generated from decision trees:

  \spcnoindent
  {\bf Key Property.} For any decision tree $T$ there is a coordinate $i \in [n]$ and $b \in \set{0,1}$ such that \[ \alpha_j[i] = b, \alpha_k[i] = 1-b\] for all $j = 1, 2, \ldots, N/2$ and $k = N/2 + 1, N/2 + 2, \ldots, N$.

  \spcnoindent
  This property is easy to prove: simply let $i$ be the index of the variable labelled on the root of the decision tree $T$.
  If the decision tree queries the bit $b$ in the left subtree then the first half of the strings in the ordering will have the $i$th bit of the string set to $b$, and the second half of strings set to $1-b$.

  To use this property, let $\beta_1, \beta_2, \ldots, \beta_N$ be the lexicographic ordering of $\set{0,1}^n$, and for any string $\beta_i$ define $\overline{\beta_i}$ to be the string obtained by flipping each bit in $\beta_i$.
  Then let ${\cal O}$ be the ordering \[ \beta_1, \overline \beta_1, \beta_2, \overline \beta_2, \ldots, \beta_{N/2}, \overline \beta_{N/2}.\]
  It follows that for each $i \in [n]$ and each $b \in \set{0,1}$, half of the strings $\alpha \in \set{0,1}^n$ with $\alpha[i] = b$ will be in the first half of the ordering ${\cal O}$ and half of the strings with $\alpha[i] = b$ are in the second half of the ordering ${\cal O}$.
  The lemma follows by applying the Key Property.
\end{proof}

\begin{corollary}
  There exists an ordering ${\cal O}$ such that any learning-sensitive backdoor for the formula ${\cal F}_{\cal O}$ has size at least $2^{n-2}$.
\end{corollary}

\begin{customthm}{3}
	For every $n > 3$, there is a formula $F_n$ on $N = O(2^n)$ variables such that the minimal LSR-backdoor has $O(\log N)$ variables, but every LS-backdoor has $\Omega(N)$ variables.
\end{customthm}




==> tables/lsr_all_decs_comparison.tex <==
\centering
\begin{tabular}{llll}
\hline
Benchmark &        Laser & All Decisions & Overlap Ratio \\
\hline
Agile       &  0.28 (0.17) &   0.35 (0.15) &   0.37 (0.13) \\
Application &  0.56 (0.36) &   0.57 (0.35) &   0.70 (0.26) \\
Crafted     &  0.88 (0.20) &   0.89 (0.19) &   0.89 (0.17) \\
Random      &    nan (nan) &     nan (nan) &     nan (nan) \\
\hline
\end{tabular}

\caption{Mean (std. dev.) of Laser produced backdoor sizes versus all decision variables. Overlap Ratio is the size of the set $(Laser \cap All Decisions) / (Laser \cup All Decisions)$.}
\label{lsr_vs_all_decs_table}



==> tables/lsr_all_decs_table.tex <==
\begin{table}[t]
\centering
\begin{tabular}{llll}
{} &        LaSeR & AllDecisions & OverlapRatio \\
benchmark &              &              &              \\

agile     &  0.16 (0.11) &  0.38 (0.16) &  0.34 (0.11) \\
app       &  0.45 (0.33) &  0.56 (0.33) &  0.58 (0.29) \\
crafted   &  0.80 (0.24) &  0.85 (0.22) &  0.79 (0.23) \\
random    &    nan (nan) &    nan (nan) &    nan (nan) \\

\end{tabular}
\label{lsr_vs_all_decs_table}
\caption{\todo{clean}Comparison of LaSeR produced backdoor sizes versus all decision variables. Overlap Ratio is the size of the set $(LaSeR \cap AllDecisions) / (Laser \cup AllDecisions)$.}
\end{table}


==> tables/lsr_proof_notation_figure.tex <==
\begin{figure}
	\begin{minipage}{0.6\linewidth}
	\begin{center}
	\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
	thick,main node/.style={circle,draw=none},decision node/.style={circle,draw}] 

	\node[main node] at (0,3) (d1) {$d_1$};
	\node[main node] at (0,2) (d2) {$d_2$};
	\node[main node] at (0,1) (d3) {$d_3$};
	\node[main node] at (0,0) (d4) {$d_4$};
	
	\node[main node] at (2, 2.5) (l1) {$l_1$};
	\node[main node] at (2, 1.5) (l2) {$l_2$};
	\node[main node] at (2, 0.5) (l3) {$l_3$};
	\node[main node] at (2, 3.2) (cprime) {$C^\prime$};
	
	\node[main node] at (4, 2) (l4) {$l_4$};
	\node[main node] at (4, 1) (l5) {$l_5$};
	
	\node[main node] at (6, 1.5) (bot) {$\bot$};

	\draw[] (d1) -- (l1) node [midway, above] {$L_1$};
	\draw[] (d2) -- (l1);
	\draw[] (d2) -- (l2);
	\draw[] (d3) -- (l2) node [near start, above] {$L_2$};
	\draw[] (d4) -- (l3);

	\draw[] (l1) -- (l4) node [midway, above] {$L_3$};
	\draw[] (l2) -- (l4);
	\draw[] (l2) -- (l5);
	\draw[] (l3) -- (l5);
	
	\draw[] (l4) -- (bot) node [near start, above] {$L_4$};
	\draw[] (l5) -- (bot) node [near start, above] {$L_5$};

	\node[rectangle,inner sep=0.6mm,rounded corners, dashed,draw, fit=(l1) (l2) (l3)](lc) {};
	\end{tikzpicture}
	\end{center}
	\end{minipage}%
	\begin{minipage}{0.34\linewidth}
	\begin{align*}
	C^\prime &= (\neg l_1 \vee \neg l_2 \vee \neg l_3) \\
	R_{L_3}^* &= \{L_6, L_7\}\\
	R_{L_4}^* &= \{\}\\
	R_{L_5}^* &= \{L_6\}\\
	\\
	R_{C^\prime} &= \{L_3, L_4, L_5\}\\
	R_{C^\prime}^* &= \{L_3, L_4, L_5, L_6, L_7\}\\
	D_{C^\prime}^* &= \{var(l_1), var(l_2), var(l_3)\} \cup \\
	& \hphantom{asd} vars(\{L_3, L_4, L_5, L_6, L_7\})
	\end{align*}
	\end{minipage}
	\caption{Example conflict analysis graph depicting the set of relevant clauses and variables to some learnt clause $C^\prime$. Nodes are literals. Edges labeled with some $L_i$ are previously learnt clauses; all other edges depicting propagations are from the original formula $F$. The clauses $L_6, L_7$ used to derive $L_3$ and $L_5$ are not shown, but would be in the respective conflict analysis graphs of $L_3$ and $L_5$. The clauses $L_1$ and $L_2$ are not included in $R_{C^\prime}$ since they occur on the reason side of the graph. }
	\label{notation-figure}
	\end{figure}


==> tables/lsr_vs_ls_theory.tex <==
\section{Separating LS and LSR-Backdoors}
\label{sec_lsr_theory}
In this section we prove that for certain kinds of formulas the
minimal LSR-backdoors are exponentially smaller than the minimal
LS-backdoors under the assumption that the learning scheme is 1st-UIP
and that the CDCL solver is only allowed to backtrack (and not
backjump). In \cite{Dilkina2009a}, the authors demonstrate that
LS-backdoors may be exponentially smaller than strong backdoors with
1st-UIP learning scheme but without restarts.% (Note that when we
% refer to these separation results we always are referring to minimal
% backdoors. However, we may drop the term ``minimal'' since it is
% obvious from context.)

Let $n$ be a positive integer and let $X = \set{x_1, x_2, \ldots, x_n}$ be a set of Boolean
variables.  For any Boolean variable $x$, let $x^1$ denote the
positive literal $x$ and $x^{0}$ denote the negative literal $\neg x$.
For any assignment $\alpha \in \set{0,1}^n$ let $C_\alpha =
x_1^{1-\alpha_1} \vee x_2^{1-\alpha_2} \vee \ldots \vee
x_n^{1-\alpha_n}$ denote the clause on $x$ variables which is uniquely
falsified by the assignment $\alpha$.

Our family of formulas will be defined using the following template.  Let
${\cal O}$ be any total ordering of $\set{0,1}^n$; we write $<_{\cal O}$ to
denote the relation induced by this ordering.  The formula is defined
on the variables $x_1, x_2, \ldots, x_n$, and also three auxiliary
sets of variables $\set{q_\alpha}_{\alpha \in \set{0,1}^n},
\set{a_\alpha}_{\alpha \in \set{0,1}^n}, \set{b_\alpha}_{\alpha \in
  \set{0,1}^n}$.  Given an ordering ${\cal O}$ we define the
formula
\[{\cal F}_{\cal O} = \bigwedge_{\alpha \in \set{0,1}^n} (C_\alpha \vee \bigvee_{\alpha' \leq_{\cal O} \alpha} \neg q_{\alpha'}) \wedge (q_\alpha \vee a_\alpha) \wedge (q_\alpha \vee b_\alpha) \wedge (q_\alpha \vee \neg a_\alpha \vee \neg b_\alpha).\]
This family was introduced by Dilkina et al. \cite{Dilkina2009a}, where the formula using the lexicographic ordering
provides an exponential separation between the sizes of LS-backdoors and strong backdoors. 
Their key insight was that if a CDCL solver without restarts queried
the $x_1,\ldots,x_n$ variables in the lexicographic ordering of
assignments, it would learn crucial conflict clauses that would enable
the solver to establish the unsatisfiability of the instance without
having to query any additional variables. (By the term ``querying a
variable'' we mean that the solver assigns value to it and then performs any unit propagations.)
Since strong backdoors cannot benefit from clause learning they will necessarily have to query additional variables to hit any conflict.

We show that the same family of formulas (but for a different ordering ${\cal O}$) can be used to separate LS-backdoor size from LSR-backdoor size.
Observe that for \emph{any} ordering ${\cal O}$ the variables $x_1, x_2, \ldots, x_n$ form an LSR-backdoor for ${\cal F}_{\cal O}$.
\begin{lemma}\label{lem:lsr-backdoor}
  Let ${\cal O}$ be any ordering of $\set{0,1}^n$.
  The $X$-variables form an LSR-backdoor for the formula ${\cal F}_{\cal O}$.
\end{lemma}
\begin{proof}
  For each assignment $\alpha \in \set{0,1}^n$ (ordered by ${\cal O}$), assign $\alpha$ to the $x$ variables by decision queries.
  By the structure of ${\cal F}_{\cal O}$, as soon as we have a complete assignment to the $x$ variables, we will unit-propagate to a conflict and learn a $q_\alpha$ variable as a conflict clause; after that we restart.
  Once all of these assignments are explored we will have learned the unit clause $q_\alpha$ for \emph{every} assignment $\alpha$, and so we can just query the $X$ variables in any order (without restarts) to yield a contradiction, since every assignment to the $X$ variables will falsify the formula.
\end{proof}

Note that the formula ${\cal F}_{\cal O}$ depends on $N = O(2^n)$ variables, and so the size of this LSR-backdoor is $O(\log N)$.
Furthermore, observe that the $X$-variables will also form an LS-backdoor if we can query the assignments $\alpha \in \set{0,1}^n$ according to ${\cal O}$ without needing to restart --- for example, if ${\cal O}$ is the lexicographic ordering.
This suggests the following definition, which captures the orderings ${\cal O}$ of $\set{0,1}^n$ that can be explored by a CDCL algorithm without restarts:
\begin{definition}
  Let ${\cal T}_X$ be the collection of all depth-$n$ decision trees on $X$-variables, where we label each leaf $\ell$ of a tree $T \in {\cal T}_X$ with the assignment $\alpha \in \set{0,1}^n$ obtained by taking the assignments to the $X$-variables on the path from the root of $T$ to $\ell$.
  For any $T \in {\cal T}_X$, let ${\cal O}(T)$ be the ordering of $\set{0,1}^n$ obtained by reading the assignments labelling the leaves of $T$ from left to right.
\end{definition}
To get some intuition for our lower-bound argument, consider an ordering ${\cal O}(T)$ for some decision tree $T \in {\cal T}_X$.
By using the argument in Lemma \ref{lem:lsr-backdoor} the formula ${\cal F}_{{\cal O}(T)}$ will have a small LS-backdoor, obtained by querying the $X$-variables according to the decision tree $T$.
Now, take any two assignments $\alpha_i, \alpha_j \in {\cal O}(T)$ and let ${\cal O}(T)'$ be the ordering obtained from ${\cal O}(T)$ by swapping the indices of $\alpha_i$ and $\alpha_j$.
If we try and execute the same CDCL algorithm without restarts (corresponding to the ordering ${\cal O}(T)$) on the new formula ${\cal F}_{{\cal O}(T)'}$, the algorithm will reach an inconclusive state once it reaches the clause corresponding to $\alpha_j$ in ${\cal O}(T)'$ since at that point the assignment to the $X$-variables will be $\alpha_i$.
Thus, it will have to query at least one more $q$ variable (for instance, $q_{\alpha_j}$), which increases the size of the backdoor by one.
We can generalize the above argument to multiple ``swaps'' --- the CDCL algorithm without restarts querying the variables according to ${\cal O}(T)$ would then have to query one extra variable for every $q_\alpha$ which is ``out-of-order'' with respect to ${\cal O}(T)$.

This discussion leads us to the following complexity measure: for any ordering ${\cal O} \in \set{0,1}^n$ (not necessarily obtained from a decision tree $T \in {\cal T}_X$) and any ordering of the form ${\cal O}(T)$, let \[ d({\cal O}, {\cal O}(T)) = |\set{\alpha' \in \set{0,1}^n \st \exists \alpha \in \set{0,1}^n : \alpha' <_{\cal O} \alpha, \alpha <_{{\cal O}(T)} \alpha'}|.\]
Informally, $d({\cal O}, {\cal O}(T))$ counts the number of elements of ${\cal O}$ which are ``out-of-order'' with respect to ${\cal O}(T)$ as we have discussed above.
We are able to show that the above argument is fully general:

% We show that for a particular ordering ${\cal O}$, the formula ${\cal F}_{\cal O}$ such that its minimal
% LSR-backdoor only needs the solver querying the $x_1, \ldots, x_n$
% variables whereas the minimal LS-backdoor requires querying exponentially more
% variables. The crucial difference between our formula and that of
% Dilkina et al. is that the ordering used to define our formula ${\cal
%   F}_{\cal O}$ is not lexicographic. 
% %Instead, the ordering has this
% %property that adjacent elements in the order are very far apart from
% %each other. \mynote{the previous sentence is not quite right, but I need to think of a better wording} 
% The intuition here is that, with a properly chosen ordering, a backtracking CDCL solver
% without restarts will not only have to query the $x_i$ variables but
% exponentially many more variables in order to infer unsatisfiability of every
% element in the ordering (i.e., every assignment to the $x_i$
% variables). By contrast, the restart feature of the solver allows it
% infer unsatisfiability of every ordering of $x_i$ variables without
% having to query any additional variables in the formula.

%% Note that if we assign any $\neg q_\alpha$, the three clauses over
%% $q_\alpha$, $a_\alpha$, and $b_\alpha$ immediately allow us to
%% learn the unit clause $q_\alpha$, using 1st-UIP.


% Given two orderings ${\cal O}_1, {\cal O}_2$ let $d({\cal O}_1, {\cal
%   O}_2)$ denote the Hamming distance of these two sequences (as
% sequences).  For instance the Hamming distance of the two sequences
% $(00, 01, 10, 11)$ and $(00, 10, 01, 11)$ is $2$.  Finally, consider
% any decision tree $T$ of depth $n$ where we have queried the $X$
% variables in \emph{any} order in the tree $T$.  From this tree we
% obtain a natural ordering ${\cal O}(T)$ of $\set{0,1}^n$ by reading
% off the strings labelling the leaves in left-to-right order.  Note
% that the orderings of the form ${\cal O}(T)$ are \emph{exactly} the
% orderings which can be generated by DPLL algorithms (or, more
% generally, a CDCL algorithm without restarts).

\begin{lemma}\label{lem:main}
  Let ${\cal O}$ be any ordering of $\set{0,1}^n$, and let ${\cal T}_X$ denote the collection of all complete depth-$n$ decision trees on $X$ variables.
  Then any learning-sensitive backdoor of ${\cal F}_{\cal O}$ has size at least \[\min_{T \in {\cal T}_X} d({\cal O}, {\cal O}(T)).\]
  % Let ${\cal O}$ be any ordering of $\set{0,1}^n$, and let ${\cal
  %   T}_X$ denote the collection of all complete depth-$n$ decision
  % trees on $X$ variables.  Then any  LS-backdoor of
  % ${\cal F}_{\cal O}$ has size at least \[n + \min_{T \in {\cal T}_X}
  % d({\cal O}, {\cal O}(T)).\]
\end{lemma}

This reduces our problem to finding an ordering ${\cal O}$ for which \emph{every} ordering of the form ${\cal O}(T)$ has many elements which are ``out-of-order'' with respect to ${\cal O}$ (again, intuitively for every mis-ordered element in the LS-backdoor we will have to query at least one more $q$-variable.)
\begin{lemma}
  For any $n > 4$ there exists an ordering ${\cal O}$ of $\set{0,1}^n$ such that for every decision tree $T \in {\cal T}_X$ we have \[ d({\cal O}, {\cal O}(T)) \geq 2^{n-2}.\]
\end{lemma}
\begin{sketch}
  We define the ordering, and leave the full proof of correctness to the companion technical report~\cite{extended_paper_link}.
  Let $\beta_1, \beta_2, \ldots, \beta_N$ be the lexicographic ordering of $\set{0,1}^n$, and for any string $\beta_i$ define $\overline{\beta_i}$ to be the string obtained by flipping each bit in $\beta_i$.
  Then let ${\cal O}$ be the ordering \[ \beta_1, \overline \beta_1, \beta_2, \overline \beta_2, \ldots, \beta_{N/2}, \overline \beta_{N/2}.\]
\end{sketch}

\suppress{
\begin{sketch}
  Let $B$ be a minimal LS-backdoor of ${\cal F}_{\cal O}$.  Let $Q =
  \set{q_\alpha}_{\alpha \in \set{0,1}^n}$.  Without loss of
  generality we can assert that $B \subseteq X \cup Q$, since an
  LS-backdoor which queries $a_\alpha$ or $b_\alpha$ variables can be
  replaced with a backdoor querying $q_\alpha$ variables which is no
  larger.  Furthermore, we know that $X \subseteq B$.  To see this,
  observe first that $Q$ is \emph{not} an LS-backdoor of ${\cal
    F}_{\cal O}$, since querying all assignments to the $Q$ variables
  will leave the algorithm in an inconclusive state.  It follows that
  $B$ must contain \emph{some} $X$ variable; to see that it contains
  \emph{all} $X$ variables, it is enough to observe that in order to
  hit a conflict (even after querying all $Q$ variables) we must
  assign a value to every $X$ variable by the structure of ${\cal
    F}_{\cal O}$.  Thus $X \subseteq B \subseteq X \cup Q$ (and $|X|$
  represents the $n$ term in the statement of the lemma). Furthermore,
  observe that we can always assume that if the algorithm queries a
  $q_\alpha$ variable as a decision variable, then it queries the
  variable negatively first.  This is because querying $\neg q_\alpha$
  will cause the CDCL algorithm to hit a conflict and learn the unit
  clause $q_\alpha$, so we may replace such ``positive'' queries
  \emph{in-situ} with negative queries without affecting the
  simulation of the backdoor queries.  In turn, this implies that we
  may assume that all $q_\alpha$ variables occurring in the backdoor
  are queried at the beginning of the algorithm, leaving only queries
  to $X$ variables.  Since all $q_\alpha$ variables in the backdoor
  $B$ are queried at the beginning of the algorithm without loss of
  generality, by the structure of ${\cal F}_{\cal O}$ we can see that
  once we start querying $X$ variables, we will only hit a conflict
  once we have assigned values to \emph{all} of the $X$ variables.
  This implies that the query order for the $X$ variables takes the
  form of a complete depth-$n$ decision tree $T \in {\cal T}_X$, using
  the notation in the statement of the lemma.
	
  With this, we can prove that every clause learned by the algorithm
  is a unit clause of the form $q_\alpha$ for some $\alpha \in
  \set{0,1}^n$.  To see this, consider any time that we have hit a
  conflict in the process of simulating the variable queries of the
  backdoor $B$.  If we have hit a conflict from querying $\neg
  q_\alpha$, as described above, we are done, so suppose otherwise.
  By assumption, the only variables that $B$ contains other than $Q$
  variables are $X$ variables, thus, to hit a conflict we must have
  queried all of the $X$ variables by the structure of ${\cal F}_{\cal
    O}$.  In such a case, since we have not queried $\neg q_\alpha$
  for any $\alpha$, we must have unit-propagated $\neg q_\alpha$ for
  some $\alpha$ by the structure of ${\cal F}_{\cal O}$.  This will
  hit a conflict and learn the unit clause $q_\alpha$, proving our
  claim.
	
  Recalling that $X \leq B \leq X \cup Q$, to prove the lemma it
  suffices to prove that \[|B \cap Q| \geq \min_{T \in {\cal T}_X}
  d({\cal O}, {\cal O}(T)) \] since $|X| = n$.  Since $B$ is a
  backdoor, it must be that at every leaf of the tree $T$ the unit
  propagator will propagate the input to a conflict.  Consider the
  ordering of the assignments ${\cal O}(T)$ induced by this tree $T$.
  At each leaf of this tree, which corresponds to an assignment
  $\alpha$ to the $X$ variables, there are two possibilities: either
  we learn the unit clause $q_\alpha$ or not.  By the structure of
  ${\cal F}_{\cal O}$, we can only learn the unit clause $q_\alpha$ at
  the leaf if we have learned the unit clauses $q_{\alpha'}$ for each
  $\alpha' \leq_{{\cal O}} \alpha$.  Thus, for any index in the
  orderings ${\cal O}(T)$ and ${\cal O}$, if the index has different
  strings in the respective orderings, it follows that we will not be
  able to learn the unit clause $q_\alpha$, and so we will have to
  query at least one extra variable from $Q$ in the backdoor $B$.
  This proves that \[|B \cap Q| \geq \min_{T \in {\cal T}_X} d({\cal
    O}, {\cal O}(T)) \] and therefore the lemma.
\end{sketch}
}

\begin{theorem}
%  There exists an infinite family of formulas $\mathcal{F}$ such that,
%  for each $F\in\mathcal{F}$, the smallest LSR-backdoor of $F$ is
%  exponentially smaller than the smallest LS-backdoor, with respect to
%  a backtracking CDCL solver that uses the 1st-UIP learning scheme.
%For every integer $N > 3$, there is a formula $F_N$ on $N$ variables such that the minimal LSR backdoor has ${\cal O}(\text{log } N)$ variables, while every LS-backdoor has ${\cal O}(N)$ variables.
%For every $n > 3$, there is a formula $F_n$ on $N = 2^n$ variables such that the minimal LSR backdoor has $O(\log N)$ variables, but every LS backdoor has $\Omega(N)$ variables.
For every $n > 3$, there is a formula $F_n$ on $N = O(2^n)$ variables such that the minimal LSR-backdoor has $O(\log N)$ variables, but every LS-backdoor has $\Omega(N)$ variables.
	\label{thm_ls_vs_lsr}
\end{theorem}

%The proof follows directly from the previous three lemmas. Again, complete proofs can be found in  \cite{extended_paper_link}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> tables/paper_extensions.tex <==
\suppress{
	\begin{table}[t]
		\begin{center}
			\begin{tabular}{ |l|l||c|c|c| }
				\hline
				\textbf{Property} & \textbf{Benchmark} & \textbf{Luby} & \textbf{Always Restart} & \textbf{Never Restart} \\ \hline
				\multirow{4}{12em}{P1: Community-based Spatial Locality of Decisions} &
				agile & 0.672 & \textbf{0.701} & 0.693\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P2: Community-based Spatial Locality of Learnt Clauses} &
				agile & 0.725 & \textbf{0.739} & 0.697\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P3: LSR Size} &
				agile & 0.212 & \textbf{0.133} & 0.271\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P4: Avg. LSR of Learnt Clauses} &
				agile & 0.136 & \textbf{0.051} & 0.203\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P5: Avg. Number of Backbone Flips, Normalized for Backbone Size} &
				agile & 578.124 & 3005.809 & \textbf{36.486}\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
				\multirow{4}{12em}{P6: Number of Learnt Clauses Subsumed by Backbones, Normalized for Backbone Size} &
				agile & 14.452 & 164.800 & \textbf{2.106}\\
				& app & nan & nan & nan\\
				& crafted & nan & nan & nan\\
				& random & nan & nan & nan \\ \hline
			\end{tabular}
		\end{center}
	\end{table}
	
\textit{P1: Spatial Locality of Decisions.} Given a community structure, we test whether the branching heuristic tends to disproportionately favor picking from certain communities. Note that this is effectively the same experiment as in \cite{hvc}, however here we are modifying the restart policy rather than the branching heuristic itself.

\textit{P2: Spatial Locality of Learnt Clauses.} Given a community structure, we test whether learnt clauses are disproportionately composed of variables from certain communities.

\textit{P3: LSR Size.} We test the LSR size, as computed by the approach discussed in Section \ref{lsralgsec}. A run of the solver that relies on fewer variables may be more favorable, and demonstrates a different type of locality than in P1 and P2.

\textit{P4: Avg. Learnt Clause LSR Size.} When computing the LSR-backdoor, each learnt clause is annotated with a set of variables $V$, which intuitively is the set of variables a fresh can branch upon and eventually derive the clause (as witnessed by the current run of the solver). We compute the average $V$ value of all learnt clauses. 

\textit{P5: Avg. Number of Backbone Flips.} Ideally, if the solver had \textit{a priori} knowledge of the backbone, it could set all variables to their correct polarity and simplify the formula accordingly. We consider how often the solver ``flips'' the polarity of a backbone literal, i.e., by adding it to the trail with a different polarity than previously. This may, in some sense, indicate that the solver is \textit{unsure} of the correct polarity of the backbone literal. 

\textit{P6: Number of Learnt Clauses Subsumed by the Backbone.} We consider how many learnt clauses are generated that contain a backbone literal with the correct polarity. In some sense, these clauses would be redundant if the solver had \textit{a priori} knowledge of the backbone, since they would be immediately satisfied.

	
We consider whether each of these components affects the size of the minimal backdoor. Further, we will also consider whether incorporating restarts, a pivotal feature of modern CDCL solvers, impacts the size of the backdoor. We note that, in addition to these features, modern solvers also incorporate clause minimization techniques to shrink learnt clauses \cite{Biere}, however we do not consider it in this work.

%\input{bd_comparison_table}

%Table \ref{bd-comparison-table} depicts our results. \todo{If we get a significant chunk of this table filled in, convert to a directed graph}

\begin{tabular}{llllll}
	\toprule
	{} &       simp\_lvr & simp\_all\_decsvr & simp\_lsr\_all\_decs\_unionvr & simp\_lsr\_all\_decs\_intervr & simp\_lsr\_all\_decs\_overlap\_ratio \\
	benchmark &                &                 &                           &                           &                                 \\
	\midrule
	agile     &  0.164 (0.108) &   0.375 (0.159) &             0.398 (0.167) &             0.141 (0.086) &                   0.344 (0.113) \\
	app       &  0.454 (0.335) &   0.564 (0.327) &             0.611 (0.319) &             0.412 (0.347) &                   0.581 (0.289) \\
	crafted   &  0.796 (0.235) &   0.853 (0.221) &             0.905 (0.172) &             0.744 (0.270) &                   0.793 (0.227) \\
	random    &      nan (nan) &       nan (nan) &                 nan (nan) &                 nan (nan) &                       nan (nan) \\
	\bottomrule
\end{tabular}

\section{LSR vs LS Examples}

\subsection{LS-Jumps-Restarts is exponentially smaller than strong \cite{bibid}} 

Assume we have a set $X$ of $k$ variables $x_1 \ldots x_k$. Given $\alpha: x_i \rightarrow {0, 1}$, let $C_\alpha$ be short for $\bigvee_{i=1}^{k} x_i^{1-\alpha_i}$ which is falsified by assigning $X$ according to the natural mapping of $\alpha$, e.g. $C_{001} = x_1 \vee x_2 \vee \neg x_3$. We will show that $X$ is an LSR-backtracking backdoor, but the smallest LS-backtracking backdoor is [TODO: exponentially?] bigger. At each line we learn through 1UIP the unit clause $\neg q_{\alpha}$.

The following is from \cite{Dilkina}, where $\alpha_1$ = $0^k$ and in general $\alpha_i$ is the lexicographic predecessor of $\alpha_{i+1}$.

$$
(C_{\alpha 1} \vee q_{\alpha 1}), 
(\neg q_{\alpha 1} \vee r_{\alpha 1}), 
(\neg q_{\alpha 1} \vee \neg r_{\alpha 1} \vee s_{\alpha 1}),
(\neg q_{\alpha 1} \vee \neg r_{\alpha 1} \vee \neg s_{\alpha 1})
$$
$$
(C_{\alpha 2} \vee q_{\alpha 1} \vee q_{\alpha 2}), 
(\neg q_{\alpha 2} \vee r_{\alpha 2}), 
(\neg q_{\alpha 2} \vee \neg r_{\alpha 2} \vee s_{\alpha 2}),
(\neg q_{\alpha 2} \vee \neg r_{\alpha 2} \vee \neg s_{\alpha 2})
$$
$$ \ldots$$
$$
(C_{\alpha 2^k} \vee q_{\alpha 1} \vee q_{\alpha 2} \vee \ldots \vee q_{\alpha 2^k} ), 
(\neg q_{\alpha 2^k} \vee r_{\alpha 2^k}), 
(\neg q_{\alpha 2^k} \vee \neg r_{\alpha 2^k} \vee s_{\alpha 2^k}),
(\neg q_{\alpha 2^k} \vee \neg r_{\alpha 2^k} \vee \neg s_{\alpha 2^k})
$$

\subsection{LS-Jumps+Restarts is [exponentially(?)] smaller than LS-Jumps-Restarts}
\todo{Not exponential -- view space of $\alpha$'s as a hypercube, and adversary can pick corner}

With the ordering of $\alpha_i$'s above, restarts do not help as a backtracking solver can learn every $\neg q_{\alpha j}$, $j < i$ before learning $\neg q_{\alpha i}$. By changing the sequence of $\alpha_i$'s to not be lexicographic, we can force a non-restarting backtracking solver to branch on variables other than in $X$.

Let $\alpha_1 = 0^k$ as before, and generally let $\alpha_{i+1}$ be the string lexicographically farthest from $\alpha_{i}$, that was not previously defined by any $\alpha_j$, $j < i$. \todo{finish; solver must start branching on non-X vars}

\subsection{Whiteboard Notes}
\begin{itemize}
	\item In order to derive any $q_{\alpha_i}$, must either pick $q_{\alpha_i}$ or derive every $q_{\alpha_j}, j < i$.
	\item If we've already derived some $q_{\alpha_i}$ it would propagate the x's instead, but I don't think this has consequence.
	\item Conjecture -- If we only ever branch on x's and q's, the only clauses we can possibly learn are $\neg q$'s.
	\item Suppose adversary starts with x sequence $x_1, ..., x_k$. Then we must learn every $q$ on the branch of $x_1$ before we can move to $x_1^{-1}$ branch. Need to count the number of assignments on the $x_1$ side that depend on q's of the other side.
\end{itemize}

\begin{conjecture}
	Take the formula from 7.1, with any ordering of the $\alpha$'s. Then, if the solver is only allowed to branch on $x$'s and $q$'s, regardless of the decision sequence, it can only learn unit clauses of the form $\neg q$. \todo{PROBLEM: assign all q's first??}
\end{conjecture}
\begin{proof}
	Suppose $c$ is the first learnt clause. There are three cases which can lead to this conflict. If we assign $q$ (positively), we immediately learn $\not q$. Suppose we falsify some clause with $C_{\alpha_i}$.
\end{proof}

\subsection{Whiteboard Notes 2.0}
Our goal is to show that the smallest LSR+backtracking backdoor for $F$ is exponentially smaller than the smallest LS+backtracking backdoor. We know $F$ is minimally unsatisfiable. First, let us partition $F$ into two sets of clauses. Let $\Delta_1$ be the $2^k$ clauses that contain some $C_{\alpha_i}$ disjunction, and $\Delta_2$ be the remaining clauses that allow us to learn each $\neg q_i$, i.e., the clauses in $L(\neg q_i)$ for all $i$. Let $F_{x=b} = \Delta_1[x=b] \cup \{ L(q_\alpha) \mid q_\alpha \in vars(\Delta_1[x=b]) \}$

\todo{proof sketch -- order the clauses according to number of qs, since each clause has 2 unseen vars, and the formula is min unsat, we must branch upon one of them to use the clause}

\begin{lemma}
For any $x \in X$ and any polarity $b$, $F_{x=b}$ is minimally unsatisfiable.
\end{lemma}
\begin{proof}
	Suppose for some $\alpha$ we remove some clause from $L(\neg q_alpha)$. Then we can assign $q_alpha$ (positively) without conflicting. By assigning $X$ according to $\alpha$, and $\neg q_\beta$, $\beta \ne \alpha$, we can satisfy all other clauses.
	If instead we remove any clause $C \in \Delta_1[x=b]$, then we can satisfy the remaining clauses by setting $\neg q_\alpha$ for every $\alpha$, and $X$ according to $\neg \alpha$.
\end{proof}



\subsection{LS+Jumps+Restarts is [exponentially(?)] smaller than LS+Jumps-Restarts}
\todo{BROKEN, but maybe not for sat case}
$X$ will denote our backdoor set of size $k$, where $k$ is even (\todo{may need one more var}). Different from before, $C_\alpha$ will correspond to a disjunction of the first $k/2$ variables in $X$, and $C_\beta$ is a disjunction of the second $k/2$ variables. Rather than the clauses used to conflict and learn $\neg q_\alpha$ as before, we have the following formula which will be used to derive binary clauses rather than unit clauses:
\todo{Fix 1uip according to williams discussion}
$$
L(l_\alpha \vee l_\beta) ::=
(\neg l_\alpha \vee r_\alpha),
(\neg l_\alpha \vee s_\alpha),
(\neg l_\beta \vee r_\beta),
(\neg l_\beta \vee s_\beta),
(\neg r_\alpha \vee \neg s_\alpha \vee \neg r_\beta \vee \neg s_\beta)
$$

We define a formula $\Omega(n)$ which is any formula over $n$ fresh variables with backdoor size $n$. As an example, the formula with all possible clauses of length $n$ over the $n$ variables will suffice. Finally, let $\Omega[l_1, l_2](n)$, where the literals $l_1, l_2$ are not in $\Omega(n)$, be the same as $\Omega(n)$, but every clause has the additional literals $l_1$ and $l_2$.

Potential example with LSR-backdoor set $X$ + any single $q$ or $r$:

\begin{equation}
\label{lsr_jump_eqn}
\begin{split}
&\bigwedge_{\alpha} 
(C_{\alpha} \vee q_{\alpha}),
\bigwedge_{\beta} 
(C_{\beta} \vee \neg r_{\beta}), \\
&\bigwedge \{ L(q_\alpha \Rightarrow r_\beta) \mid \alpha = \beta\} \\ 
&\bigwedge \{ L(r_\beta \Rightarrow q_\alpha) \mid \alpha = \beta + 1\} \\ 
&\bigwedge \{ \Omega[q_\alpha, \neg r_{\beta}] \mid \alpha \ne \beta \wedge \alpha \ne \beta + 1\}  \\
&(\neg q_{\alpha_0} \Rightarrow  r_{\beta_{2^k}}), 
(q_{\alpha_0} \Rightarrow \neg r_{\beta_{2^k}}), 
(\neg q_{\alpha_0} \Rightarrow \neg r_{\beta_{2^k}}),
\end{split}
\end{equation}

\todo{Might need to hide (4) under last X vals}

\begin{theorem}
	There exists a family of formulas such that the smallest LSR+backjumping backdoor is \todo{exponentially} smaller than the smallest LS+backjumping backdoor.
\end{theorem}
\begin{proof}
We first demonstrate that 
\end{proof}



\suppress{
\section{LSR vs LS old}
$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee p_1^\prime), (\neg x \vee p_2^\prime), (\neg p_1^\prime \vee \neg p_2^\prime \vee \neg q \vee q^\prime), (\neg q^\prime \vee a^\prime), (\neg q^\prime \vee \neg a^\prime \vee b^\prime), (\neg q^\prime \vee \neg a^\prime \vee \neg b^\prime) 
$$
$$
(x \vee q \vee q^\prime \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$


\section{LSR may be arbitrarily smaller than LS}
The following formula from the LS paper has a minimal LS backdoor \{x\}:
$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee q \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$
Essentially, if we set $x=0$, we learn $\neg q$ on the top half, which leads to a conflict on the bottom half when we set $x=1$.

Now consider a new formula which duplicates the first line: 
{\boldmath$$
(x \vee p_1^\prime), (x \vee p_2^\prime), (\neg p_1^\prime \vee \neg p_2^\prime \vee q^\prime), (\neg q^\prime \vee a^\prime), (\neg q^\prime \vee \neg a^\prime \vee b^\prime), (\neg q^\prime \vee \neg a^\prime \vee \neg b^\prime) 
$$
}$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee q \bm{\vee q^\prime} \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$
We can then set $x=0$ to learn $q$ as before, but then restart to learn $q^\prime$ as well. 

We can repeat this any number of times by introducing a new ``prime row'' (and q in the bottom clause).
This breaks my previous conjecture that $LS = LSR + \mathcal{O}(log(numRestarts))$. New conjecture: $LS = LSR + \mathcal{O}(numRestarts))$.


\section{Main Contributions}
\begin{itemize}
	\item LSR backdoor definition + algorithm
	\item Correlation experiments for several metrics over SAT comps + scaling.
	\item Relationship of cmty structure/bridges and backdoors
	\item Solving with a priori knowledge of metrics		
\end{itemize}

\section{Paper Threats}
\begin{itemize}
	\item Need to motivate LSR backdoors
	\begin{itemize}
		\item Small examples where minimum LS-backdoor is larger than LSR
		\item General relationship/bound of LSR to LS sizes.
	\end{itemize}
	\item General Threats to Validity
	\begin{itemize}
		\item We don't have optimal value (e.g. minimum backdoors). Answer: using current best algorithms + long timeouts.
		\item Consider multiple solvers (for now just maplesat times). Have most data for Glucose and Minisat. 
		\item Consider more than linear regression for correlation experiments (ridge regression, which handles multicollinearity better than LR, achieved similar $R^2$ values)
		\item LSR computation based upon solver run (circularity threat?.. cannot remember how we resolved this..)
		\item Solving times should probably be recomputed on StarExec/Azure (sharcnet has some unpredictability).
		\item Need to explain why correlations are lower than 2014 cmty structure paper.
	\end{itemize}
\end{itemize}
}
}

==> tables/regression.tex <==
\begin{center}
\scalebox{0.7}{
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Feature Set} & \textbf{Application} & \textbf{Crafted} & \textbf{Random} & \textbf{Agile}\\ \hline

$V\oplus{}C\oplus{}C/V$ & 0.02 (1093) & 0.04 (706) & 0.08 (126) & 0.85 (4964)\\

$V\oplus{}C\oplus{}Cmtys\oplus{}Q$ & 0.04 (841) & 0.14 (566) & 0.25 (126) & 0.87 (4964)\\

$V\oplus{}C\oplus{}LSR\oplus{}LSR/V$ & 0.16 (345) & 0.40 (281) & N/A & 0.88 (3257)\\

$V\oplus{}C\oplus{}\#Min\_Weak\oplus{}Weak$ & 0.11 (238) & 0.14 (160) & 0.23 (76) & 0.56 (464)\\

$V\oplus{}C\oplus{}Bones\oplus{}Bones/V$ & 0.10 (167) & 0.35 (119) & 0.04 (59) & 0.43 (208)\\

$V\oplus{}C\oplus{}TW\oplus{}TW/V$ & 0.03 (1037) & 0.05 (706) & 0.28 (126) & 0.91 (4964)\\

$V\oplus{}C\oplus{}TW\oplus{}LSR\oplus{}Q\oplus{}Cmtys$ & 0.08 (345) & 0.53 (281) & N/A & 0.95 (3257)\\

$V\oplus{}C\oplus{}TW\oplus{}TW/V$ & 0.03 (1037) & 0.05 (706) & 0.28 (126) & 0.91 (4964)\\

\hline
$C/V\oplus{}Q\oplus{}Q/Cmtys\oplus{}LSR/V\oplus{}TW/V$ & \textbf{0.39 (345)} & 0.62 (281) & N/A & 0.94 (3257)\\

$C\oplus{}C/V\oplus{}Q\oplus{}LSR/V\oplus{}TW/V$ & 0.25 (345) & \textbf{0.65 (281)} & N/A & 0.93 (3257)\\

$V\oplus{}C\oplus{}C/V\oplus{}Cmtys\oplus{}Q$ & 0.10 (345) & 0.34 (281) & \textbf{N/A} & 0.91 (3257)\\

$V\oplus{}C\oplus{}Q\oplus{}LSR/V\oplus{}TW/V$ & 0.17 (345) & 0.58 (281) & N/A & \textbf{0.94 (3257)}\\

\hline
\end{tabular}
}
\end{center}
\caption{Adjusted R$^2$ values for the given features, compared to log of Maplecomsps' solving time. The number in parentheses indicates the number of instances that were considered in each case. The lower section of feature sets consider heterogeneous sets of features from different structural analyses.}
\label{tab-regressions}



==> tables/related_work_table.tex <==
\begin{table}
\begin{center}
	\begin{tabular}{| l | c | c | c |}
		\hline
		Type & Benchmarks & Defined for Unsat? & Tool Available?  \\ \hline
		Strong \cite{Chaharmir2002} & 3SAT  & Yes & Yes (\cite{Li2011, Kilby2005}) \\ \hline
		Weak \cite{Chaharmir2002} & 3SAT, GC & No & Yes (\cite{Li2011, Kilby2005}) \\ \hline
		LS \cite{Dilkina2009a} & LP  & Yes & Yes (implemented) \\ \hline
		Tree \cite{Samer2008} & Auto, 3SAT  & Yes & No \\ \hline
		%Clause Deletion & Not Sure \todo{} & Yes & Not Sure \\  \hline
		LSR  & -- & Yes & Yes (implemented) \\
		\hline \hline
		Weak Keys \cite{Ruan2004} & MGC, LP, QWH & No & Yes (trivial) \\ \hline
		Backbones \cite{Chaharmir2002, Kilby2005} & 3SAT, GC & No & Yes (\cite{Marques-silva2012}) \\ \hline
		LSR Keys & -- & No & Yes (implemented) \\  \hline \hline
		% \footnote{\url{http://sat.inesc-id.pt/~mikolas/#Software}}
		Treewidth \cite{Mateescu2011, Liang2015} & C09, FM & Yes & No (Algorithm in \cite{Mateescu2011}) \\ \hline
		Q \cite{Newsham, Ans??tegui2012} & Most (all?) & Yes & Yes (Louvain, OL) \\ \hline
		Input-restricted \cite{Newsham, Ans??tegui2012} & CS & Yes & Yes (trivial) \\ \hline
	\end{tabular}
\end{center}
\caption{Subset of the proposed backdoors from the literature. Below the first double-line are concepts that are either related to backdoors. We also include treewidth and modularity of the community structure Q, as they have been proposed as an alternative metric for measuring the difficulty of SAT instances.}
\end{table}

==> tables/relatedwork.tex <==
\section{Related Work}
\label{sec-relatedwork}

%\input{tables/benchmark_descriptions_table}
%\input{tables/related_work_table_condensed}

\textbf{Backdoor-related Parameters.} Traditional weak and strong
backdoors for both SAT and CSP were introduced by Williams et al.~
\cite{Williams2003}.  Kilby et al. introduced a local search algorithm
for computing weak backdoors~\cite{Kilby2005}, and showed that random
SAT instances have medium sized backdoors (of roughly 50\% of the
variables), and that the size of weak backdoors did not correlate
strongly with solving time. Li et al. introduced an improved Tabu
local search heuristic for weak backdoors \cite{Li2011}. They
demonstrated that many industrial satisfiable instances from SAT
competitions have very small weak backdoors, often around 1\% of the
variables. The size of backdoors with respect to subsolvers different
from UP was considered in \cite{Dilkina2014,Li2011}. Monasson et
al. introduced backbones to study random 3-SAT instances
\cite{monasson1999determining}. Janota et
al. \cite{janota2015algorithms} introduced and empirically evaluated
several algorithms for computing backbones. Several extensions of
traditional strong and weak backdoors have been
proposed. Learning-sensitive (LS) backdoors also consider the
assignment tree of backdoor variables, but additionally allow clause
learning to occur while traversing the tree, which may yield
exponentially smaller backdoors than strong backdoors
\cite{Dilkina2009,Dilkina2009a}.

\textbf{Graph Abstraction Parameters.}  Mateescu computed lower and
upper bounds on the treewidth of large application formulas
\cite{Mateescu2011}.  Ans\'otegui et al. introduced community
structure abstractions of SAT formulas, and demonstrated that
industrial instances tend to have much better structure than other
classes, such as random \cite{Ansotegui2012}. It has also been shown
that community-based features are useful for classifying industrial
instances into subclasses (which distinguish types of industrial
instances in the SAT competition) \cite{jordi2015classification}.
Community-based parameters have also recently been shown to be one of
the best predictors for SAT solving performance
\cite{newsham2014impact}.

% \todo{cmty,louvain,newjournal} Treewidth of SAT formulas was
%considered in \cite{mateescu}, and although we have investigated
%treewidth by utilizing his work, we do not discuss treewidth in this
%document due to issues with the tool.

\suppress{ \todo{condense if no space} Most of the metrics discussed
  in this paper have associated parameterized complexity results. A
  decision problem and associated parameter $k$ is \textit{fixed
    parameter tractable} (FPT) if for any input $x$, the problem can
  be decided in time $f(k) \cdot |x|^{\mathcal{O}(1)}$, where
  \textit{f} is a computable function dependent only on $k$ (for an
  overview, see \cite{mainfptbook}). In our context, the parameterized
  decision problem is always SAT($\phi$, k), where $\phi$ is the
  Boolean formula and the parameter $k$ may be, for example, a
  backdoor set. Given a formula $\phi$ and weak or strong backdoor
  $k$, the satisfiability of $\phi$ can be determined in time
  $\mathcal{O}(2^k \cdot subsolver(\phi))$ by testing all $2^{|k|}$
  full assignments to the backdoor to determine satisfiability using
  the given subsolver, which by definition runs in polynomial time
  \cite{Williams2003}. Thus the decision problem of SAT with parameter
  weak or strong backdoor is in FPT.  The decision problem of SAT with
  parameter treewidth (of the graph abstraction of the formula) is
  also FPT \cite{szeider2003fixed}. For community structure, the
  notion of h-modularity was introduced, such that a formula with good
  h-modularity can be decomposed into communities that form hitting
  formulas \cite{ganian2015community}. They show that SAT with
  parameter h-modularity is in FPT.  Note importantly that since CDCL
  does not incorporate these FPT algorithms, the FPT upper bounds do
  not necessarily relate to CDCL performance. Our work further
  investigates whether there are empirical relationships between these
  parameters and CDCL runtime.  }


%\begin{figure}
%\input{tables/related_work_table_condensed} 

\begin{table}
	\input{tables/related_work_table_condensed} 
	\input{tables/datasummary}
		\input{tables/satmin_regression}
	\input{tables/satmin_averagemetrics}

\end{table}

%\begin{table}[t]
%	\input{tables/related_work_table_condensed} 
%\end{table}



\suppress{ \textbf{Proof Measures.} J{\"a}rvisalo et al. studied how proof
  measures, such as proof length, width, and space, are related to
  CDCL performance \cite{jarvisalo2012relating}. They showed that
  proof size correlated well with solving time, over a set of crafted
  formulas with fixed width and length.  }

Other work such as SatZilla \cite{xu2008satzilla} focus on large sets
of easy-to-compute parameters that can be used to quickly predict the
runtime of SAT solvers. In this paper, our focus is on parameters
that, if sufficiently favorable, offer provable parameterized
complexity-theoretic guarantees of worst-case runtime
\cite{downey2013fundamentals}. The study of structural parameters of
SAT instances was inspired by the work on clause-variable ratio and
the phase transition phenomenon observed for randomly-generated SAT
instances in the late
1990's~\cite{coarfa2000random,monasson1999determining,selman1996generating}.
 
% This is a dangerous sentence, and it is not really what is said in Moshe's talk.
%Subsequent
%work showed that a similar sharp phase transition is not observed for
%industrial instances \cite{}.


% I don't know of a well cited work for this missing citation. I
% recall Moshe Vardi asserting that there is no phase transition
% observed for industrial instances in his Banff 2014 talk. You can
% see that from his talk. We should probably do some googling of
% ``phase transition industrial SAT instances''.

Table \ref{tab-relatedwork} lists previous results on empirically
computing several parameters and correlating them with SAT solving
time.  While weak backdoors, backbones, and treewidth have been
evaluated on some industrial instances from the SAT competitions, only
modularity has been evaluated across a wide range of instances. Some
benchmarks, such as the random 3-SAT and graph coloring instances
considered in \cite{Kilby2005}, are too small/easy for modern day CDCL
solvers to perform meaningful analysis. Additionally, the benchmarks
used in previous works to evaluate each parameter are mostly disjoint,
making comparisons across the data difficult.


==> tables/satanalysis.tex <==
\section{Analysis of Structural SAT Parameters}
\label{sec_sat_analysis} 

Our first set of experiments investigate the relationship between
structural parameters and CDCL performance. While we would like to
evaluate all parameters considered in Section \ref{sec-relatedwork},
we focus on weak backdoors, backbones, community structure, treewidth,
and LSR-backdoors. We note that obtaining any non-trivial upper bound
on the size of the strong backdoor seems infeasible at this time.

\suppress{
\begin{table}[t]
	\centering
	\begin{tabular}{|l|rrrrrr|}
		\hline
		{} &  \#Instances &   LSR &  Weak &  Cmty  & Backbones &  maplecomsps \\ \hline
		agile    &       5000 &  1829 &   377 &  5000 &  &      2543   \\
		application &       1048 &   482 &   257 &   888 & &         1045  \\
		crafted  &        783 &   300 &     0 &   726 &  &           783 \\
		random   &        126 &   106 &     0 &   126 & &          126 \\ 
		Total    &       6957 &  2717 &   634 &  6740 &  &        4497 \\ \hline
	\end{tabular}
	\caption{\todo{column for sat}Depicts the number of instances
          in each benchmark, as well as the number of instances we
          were able to successfully compute each metric/time. ``Cmty''
          refers community metrics.}
	\label{tab-datasummary}
\end{table}
}
%\input{tables/datasummary}



\suppress{
\begin{table}
	\centering
	\begin{tabular}{|l|ccccc|}
		\hline
		{} &   LSR &  Weak+keys &  Cmty  & Backbones & maplecomsps \\ \hline
		agile    &  (6GB, 300s) &   (6GB, 1h) &  (6GB, 1h) & (6GB, 24h) & (6GB, 60s)   \\
		app/crafted/random &  (6GB, 3h) &   (6GB, 24h) &  (6GB, 2h) & (6GB, 24h) & (6GB, 5000s)   \\ \hline
	\end{tabular}
	\caption{\todo{fold into text not worth the space}Allocated resources for each experiment.}
	\label{tab-resources}
\end{table}
}

\textbf{Experimental Setup, Tools, and Benchmarks.}  We use off the
shelf tools to compute weak backdoors \cite{Li2011}, community
structure and modularity \cite{newsham2014impact}, backbones
\cite{janota2015algorithms}, and treewidth \cite{Mateescu2011}. Their
approaches are briefly described in Table \ref{tab-relatedwork}. Due
to the difficulty of exactly computing these parameters, with the
exception of backbones, the algorithms used in previous work (and our
experiments) do not find optimal solutions, e.g., the output may be an
upper-bound on the size of the minimum backdoor. We compute
LSR-backdoors using a tool we developed called \textit{LaSeR}, which
computes an upper-bound on the size of the minimal LSR-backdoor. The
tool is built on top of the MapleSat SAT solver
\cite{liang2016learning},  an extension of MiniSat
\cite{een2003extensible}.  We describe the \textit{LaSeR} algorithm in
Section \ref{sec_lsr_algorithms}. We use \textit{MapleCOMSPS}, the
2016 SAT competition main track winner as our reference solver for
solver runtime.

Table \ref{tab_data_summary} shows the data sources for our
experiments. We include all instances from the Application and Crafted
tracks of the SAT competitions from 2009 to 2014, as well as the 2016
Agile track. We additionally included a small set of random instances
as a baseline. As the random instances from recent SAT competitions
are too difficult for CDCL solvers, we include a set of instances from
older competitions. We pre-selected all random instances from the 2007
and 2009 SAT competitions that could be solved in under 5 minutes by
MapleCOMSPS. All instances were simplified using MapleCOMSPS'
preprocessor before computing the parameters. The preprocessing time
was not included in solving time.
 
Experiments were run on an Azure cluster, where each node contained
two 3.1 GHz processors and 14 GB of RAM. Each experiment was limited
to 6 GB. For the Application, Crafted, and Random instances, we
allotted 5000 seconds for MapleCOMSPS solving (the same as used in the
SAT competition), 24 hours for backbone and weak backdoor computation,
2 hours for community structure computation, and 3 hours for LSR
computation. For the Agile instances, we allowed 60 seconds for
MapleCOMSPS solving and 300 seconds for LSR computation; the remaining
Agile parameter computations had the same cutoff as Application. Due
to the difficulty of computing these parameters, we do not obtain
values for all instances due to time or memory limits being
exceeded.  Several longer running experiments were run on the SHARCNET
Orca cluster \cite{sharcnet}. Nodes contain cores between 2.2GHz and
2.7GHz.

\textbf{Structural Parameters and Solver Runtime Correlation:} The
first research question we posed is the following: \textit{Do
  parameter values correlate with solving time? In particular, can we
  build significantly stronger regression models by incorporating
  combinations of these features?} To address this, we
construct ridge regression models from subsets of features related to
these parameters. We used ridge regression, as opposed to linear
regression, in order to penalize multi-collinear features in the
data. We consider the following ``base'' features: number of variables
(V), number of clauses (C), number of communities (Cmtys), modularity
(Q), weak backdoor size (Weak), the number of minimal weak backdoors
computed (\#Min\_Weak), LSR-backdoor size (LSR), treewidth upper-bound
(TW), and backbone size (Bones). For each $P \in \{$\textit{C, Cmtys,
  Weak, LSR, TW, Bones}$\}$ we include its ratio with respect to $V$
as $P/V$. We also include the ratio feature $Q/Cmtys$, as used in
\cite{newsham2014impact}. All features are normalized to have mean 0
and standard deviation 1. For a given subset of these features under
consideration, we use the ``$\oplus$'' symbol to indicate that our
regression model contains these base features, as well as all
higher-order combinations of them (combined by multiplication). For
example, $V \oplus C$ contains four features: $V$, $C$, and $V \cdot
C$, plus one ``intercept'' feature. Our dependent variable is the log
of runtime of the MapleCOMSPS solver.

In Table \ref{tab-regressions}, we first consider sets of
\textit{homogeneous} features with respect to a given parameter, e.g.,
only weak backdoor features, or only community structure based
features, along with $V$ and $C$ as baseline features. Each cell
reports the adjusted $R^2$ value of the regression, as well as the
number of instances considered in each case (which corresponds to the
number of instances for which we have data for each feature in the
regression). It is important to note that since different subsets of SAT
formulas are used for each regression (since our dataset is
incomplete), we should not directly compare the cells in the top
section of the table. Nonetheless, the results do give some indication
if each parameter relates to solving time.

In order to show that combinations of these features can produce
stronger regression models, in the bottom half of Table
\ref{tab-regressions}, we consider all instances for which we have
LSR, treewidth, and community structure data. We exclude backbones and
weak backdoors in this case, as it limits our study to SAT instances
and greatly reduces the number of datapoints.  We considered all
subsets of base features of size 5 (e.g. $V \oplus LSR/V \oplus LSR
\oplus Q \oplus TW$), and report the best model for each benchmark,
according to adjusted $R^2$ (i.e. the bolded data along the
diagonal). This results in notably stronger correlations than with any
of the homogeneous features sets. Although we report our results with
five base features (whereas most homogeneous models only used four),
similar results appear if we only use four base features.  We also
note that $R^2$ values results to be higher for the Agile instances,
as compared to application and crafted instances. This is somewhat
expected, as the set of instances are all derived from the SAGE
whitebox fuzzer~\cite{godefroid2008automated}, as compared to our other benchmarks
which come from a heterogeneous set of sources.

For each row corresponding to the heterogeneous feature sets, the base
features are ordered according to the \textit{confidence level}
(corresponding to p-values), that the feature is significant to the
regression (highest first), with respect to the model used to produce
the bold data along the diagonal (i.e. the best model for each
benchmark). Confidence values are measured as a percentage; for
brevity, we consider values over 99\% as very significant, values
between 99\% and 95\% are significant, and values below 95\% are
insignificant. For application instances, \textit{Q}, \textit{C/V},
and \textit{LSR/V} are all very significant, \textit{Q/Cmtys} was
significant, and $C$ was not significant.  For crafted instances,
\textit{TW/V} and \textit{Q} were very significant, but the other base
features were insignficant.  No features are significant for the
random track, indicating that the $R^2$ value is likely spurious,
partly due to the small size of the benchmark. For the Agile
benchmark, all five features are very significant. In each model,
several higher-order features are also reported as significant,
including several where the base feature is not considered
significant.

We also remark that previous work showed notably higher $R^2$ values
for community-based features \cite{newsham2014impact}. There are
several significant differences between our experiments. First, our
instances are pre-simplified before computing community
structure. Their experiments grouped all Application, Crafted, and
Random into a single benchmark, whereas ours are split.

%% A potential issue is that the majority of random instances will
%% have both very poor community structure (i.e. low $Q$ values) and
%% timeouts for the dependent variable, allowing the regression model
%% to easily fit this subset of data points.

%Further, they allowed six base features, as opposed to our four,
%which improves the model. What about the fact that you are using
%ridge as opposed to linear regression. Does that impact the results
%vis-a-vis Zack's work?

\suppress{
\begin{table}[t]
	\centering
	\begin{tabular}{|l|rrr|}
		\hline
		benchmark &       lvr &      wvr &         Q \\ \hline
		agile     &  0.224 (0.135) &  0.004 (0.002) &  0.870 (0.054) \\
		app       &  0.320 (0.319) &  0.015 (0.024) &  0.789 (0.183) \\
		crafted   &  0.573 (0.268) &      N/A &  0.630 (0.250)\\
		random    &  0.476 (0.152) &      N/A &  0.147 (0.104)\\
		\hline
	\end{tabular}
	\caption{Mean (std. dev.) values for each parameter.}
	\label{tab-meanstd}
\end{table}
}
%\input{tables/averagemetrics}

\textbf{Structural Parameters for Industrial vs. Crafted Instances:}
The research question we posed here is the following: \textit{Do
  real-world SAT instances have significantly more favorable parameter
  values (e.g. smaller backdoors or higher modularity), when compared
  to crafted or random instances?}  A positive result, such that
instances from application domains (including Agile) have better
structural values, would support the hypothesis that such structure
may relate to the efficiency of CDCL solvers. Table \ref{tab-meanstd}
summarizes our results.  We note that while application and Agile
instances indeed appear more structured with respect to these
parameters, the application benchmark has high standard deviation
values. This could be due to the application instances
coming from a wide variety of sources.

\subsection{Using Structural Parameters to Compare Solving Heuristics}
When comparing different solvers or heuristics, the most common
approach is to run them on a benchmark to compare solving times, or in
some cases the number of conflicts during solving. However, such an
approach does not lend much insight as to \textit{why} one heuristic
is better than another, nor does it suggest any ways in which a less
performant heuristic may be improved. By contrast, in their recent
works Liang et al.~\cite{liang2016learning,liang2015understanding},
drew comparisons between various branching heuristics by comparing
their locality with respect to the community structure or the
``learning rate'' of the solver. This eventually led them to build
much better branching heuristics. We hope to do the same by using
LSR-backdoors as a lens to compare restart policies.

Starting from the baseline MapleSAT solver, we consider three restart
heuristics: 1) the default heuristic based on the Luby sequence
\cite{luby1993optimal}; 2) restarting after every conflict (always restart); and 3)
never restarting.  We test the following properties of these
heuristics, which may relate to their effect on solving performance.
First, we consider the LSR-backdoor size, as computed by the approach discussed
in Section \ref{sec_lsr_algorithms}. A run of the solver that focuses
on fewer variables can be seen as being more ``local,'' which may be
favorable in terms of runtime. When computing LSR-backdoor sizes, each learnt
clause $C$ is annotated with a set of \textit{dependency variables}
(denoted $D_C^*$ in Section \ref{sec_lsr_algorithms}), which
intuitively is a sufficient set of variables such that a fresh solver,
branching only on variables in this set, can learn $C$. Our second
measure looks at the average dependency set size for each learnt
clause.

\begin{table}[t]
\input{tables/structure_logging}
\end{table}

Due to space limitations, we only consider the Agile instances as this
gives us a large benchmark where all instances are from the same
domain.  The data in Table \ref{tab_lens} corresponds to the average
and standard deviation values across the benchmark. We only consider
instances where we can compute all data for each heuristic, in total
2145 instances. The always restart policies emits smaller LSR sizes,
both overall and on average per clause, and, somewhat surprisingly,
always restarting outperforms the more standard Luby policy in this
context.  Note that we do not expect this result to hold across all
benchmarks, as it has been shown that different restart
policies are favorable for different types of instances
\cite{biere2015evaluating}.  However, given the success of always
restarting here, results such as ours may promote techniques to
improve rapidly restarting solvers such as in~\cite{ramos2011between}.

%% \suppress{	
%% \textbf{RQ 3:} \textit{Do backdoor variables relate to important
%%   aspects of the community structure, such as bridge variables?}
%% Bridge variables correspond to vertices in the VIG that share an edge
%% with a neighboring community (as opposed to vertices that are only
%% directly connected to vertices in its own community). In
%% \cite{liang2015understanding}, it was shown that VSIDS
%% disproportionately picks bridge variables. Since these variables are
%% somehow important to branching heuristics, a strong relationships
%% between bridge variables and backdoor sets may indicate that backdoors
%% are somehow important during CDCL SAT solving. More particularly, we
%% test the following hypothesis: \textit{the set of bridge variables in
%%   a given formula highly overlap with the set of backdoor
%%   variables}. If being a bridge variable is a good indicator of being
%% a backdoor variable, then this would give us a cheap way to
%% approximate a backdoor set.

%% \begin{table}[t]
%% 	\centering
%% 	\begin{tabular}{|l|rr|}
%% 		\hline
%% 		Benchmark   &   Sensitivity &   Specificity \\
%% 		\hline
%% 		application &      0.600062 &      0.349982 \\
%% 		agile       &      0.383205 &      0.220569 \\
%% 		crafted     &      0.717464 &      0.647817 \\
%% 		random      &      0.997432 &      0.907196 \\
%% 		\hline
%% 	\end{tabular}
%% 	\caption{Sensitivity and specificity averages for each
%%           benchmark. Random is unusually high due to the poor
%%           community structure typically causing all variables to be in
%%           their own community, and thus always be bridge
%%           variables. These instances also tend to have very large
%%           backdoors.}
%% 	\label{tab-sensitivity}
%% \end{table}

%% Unfortunately, we show that there is not a strong relationship between
%% backdoors and bridge variables. We report the sensitivity (true
%% positive rate) -- \#backdoor bridge variables / \#bridges, and
%% specificity (true negative rate) -- \#non-bridge non-backdoor
%% variables / \#non-backdoor variables. Table \ref{tab-sensitivity}
%% depicts the average sensitivity and specificity on a per case study
%% basis. Ideally, both values would be close to 1.  }
%Further with a sufficiently strong relationship, bridge variables could be able to 
	
%% \suppress{
%% \subsection{Ongoing Work}
%% \label{sec-ongoing}
%% Due to the computational difficulty in computing such metrics, we are
%% still waiting for data on other metrics, namely backbones
%% \cite{monasson1999determining}, backdoor keys \cite{Ruan2004}, and
%% treewidth \cite{Mateescu2011}.
%% %However, preliminary results are so far similar, in the sense that
%% %there is not a strong relationship between solving time and the value
%% %of these features.
%% We further intend to explore regression models more sophisticated than
%% linear regression.

%% We additionally will investigate the following questions. How do the
%% variables chosen by the branching heuristic of a SAT solver relate to
%% these structural characteristics? This would essentially be an
%% extension of previous work \cite{liang2015understanding} (as well as
%% the bridge variable experiment above), in which we studied the
%% variable choices of the VSIDS branching heuristic with respect to the
%% community structure of the formula. Second, do "scaling" crafted
%% instances (such as a set formulas that encode multiplier circuits of
%% increasing bit-width), have scaling structural metric values? Since
%% these instances become increasingly difficult for SAT solvers as their
%% size increases, a metric that is a good indicator of hardness should
%% change proportionally. Finally, even though computing these metrics is
%% computationally difficult, it is worth exploring whether a priori
%% knowledge of these metrics can improve solving performance (e.g. by
%% giving the solver knowledge of a backdoor in advance of
%% solving). Positive results would motivate the exploration of
%% approximation algorithms for these metrics, which may be of more
%% practical value to solvers. Further, utilizing structural properties
%% may have similar value in the context of problems beyond SAT, such as
%% MaxSAT or incremental SAT solving.  }
%These algorithms are mostly fixed-parameter tractable \cite{thebook}:


==> tables/satmin_lsr_all_decs_comparison.tex <==
\centering
\begin{tabular}{llll}
\hline
Benchmark &        Laser & All Decisions & Overlap Ratio \\
\hline
Agile       &  0.18 (0.13) &   0.36 (0.17) &   0.43 (0.14) \\
Application &  0.34 (0.33) &   0.57 (0.35) &   0.70 (0.26) \\
Crafted     &  0.58 (0.35) &   0.89 (0.19) &   0.89 (0.17) \\
Random      &  0.64 (0.32) &    0.91 (nan) &    0.92 (nan) \\
\hline
\end{tabular}

\caption{Mean (std. dev.) of Laser produced backdoor sizes versus all decision variables. Overlap Ratio is the size of the set $(Laser \cap All Decisions) / (Laser \cup All Decisions)$.}
\label{lsr_vs_all_decs_table}



==> tables/scrap.tex <==
\suppress{
We consider whether each of these components affects the size of the minimal backdoor. Further, we will also consider whether incorporating restarts, a pivotal feature of modern CDCL solvers, impacts the size of the backdoor. We note that, in addition to these features, modern solvers also incorporate clause minimization techniques to shrink learnt clauses \cite{Biere}, however we do not consider it in this work.

%\input{bd_comparison_table}

%Table \ref{bd-comparison-table} depicts our results. \todo{If we get a significant chunk of this table filled in, convert to a directed graph}



\section{LSR vs LS Examples}

\subsection{LS-Jumps-Restarts is exponentially smaller than strong \cite{bibid}} 

Assume we have a set $X$ of $k$ variables $x_1 \ldots x_k$. Given $\alpha: x_i \rightarrow {0, 1}$, let $C_\alpha$ be short for $\bigvee_{i=1}^{k} x_i^{1-\alpha_i}$ which is falsified by assigning $X$ according to the natural mapping of $\alpha$, e.g. $C_{001} = x_1 \vee x_2 \vee \neg x_3$. We will show that $X$ is an LSR-backtracking backdoor, but the smallest LS-backtracking backdoor is [TODO: exponentially?] bigger. At each line we learn through 1UIP the unit clause $\neg q_{\alpha}$.

The following is from \cite{Dilkina}, where $\alpha_1$ = $0^k$ and in general $\alpha_i$ is the lexicographic predecessor of $\alpha_{i+1}$.

$$
(C_{\alpha 1} \vee q_{\alpha 1}), 
(\neg q_{\alpha 1} \vee r_{\alpha 1}), 
(\neg q_{\alpha 1} \vee \neg r_{\alpha 1} \vee s_{\alpha 1}),
(\neg q_{\alpha 1} \vee \neg r_{\alpha 1} \vee \neg s_{\alpha 1})
$$
$$
(C_{\alpha 2} \vee q_{\alpha 1} \vee q_{\alpha 2}), 
(\neg q_{\alpha 2} \vee r_{\alpha 2}), 
(\neg q_{\alpha 2} \vee \neg r_{\alpha 2} \vee s_{\alpha 2}),
(\neg q_{\alpha 2} \vee \neg r_{\alpha 2} \vee \neg s_{\alpha 2})
$$
$$ \ldots$$
$$
(C_{\alpha 2^k} \vee q_{\alpha 1} \vee q_{\alpha 2} \vee \ldots \vee q_{\alpha 2^k} ), 
(\neg q_{\alpha 2^k} \vee r_{\alpha 2^k}), 
(\neg q_{\alpha 2^k} \vee \neg r_{\alpha 2^k} \vee s_{\alpha 2^k}),
(\neg q_{\alpha 2^k} \vee \neg r_{\alpha 2^k} \vee \neg s_{\alpha 2^k})
$$

\subsection{LS-Jumps+Restarts is [exponentially(?)] smaller than LS-Jumps-Restarts}
\todo{Not exponential -- view space of $\alpha$'s as a hypercube, and adversary can pick corner}

With the ordering of $\alpha_i$'s above, restarts do not help as a backtracking solver can learn every $\neg q_{\alpha j}$, $j < i$ before learning $\neg q_{\alpha i}$. By changing the sequence of $\alpha_i$'s to not be lexicographic, we can force a non-restarting backtracking solver to branch on variables other than in $X$.

Let $\alpha_1 = 0^k$ as before, and generally let $\alpha_{i+1}$ be the string lexicographically farthest from $\alpha_{i}$, that was not previously defined by any $\alpha_j$, $j < i$. \todo{finish; solver must start branching on non-X vars}

\subsection{Whiteboard Notes}
\begin{itemize}
	\item In order to derive any $q_{\alpha_i}$, must either pick $q_{\alpha_i}$ or derive every $q_{\alpha_j}, j < i$.
	\item If we've already derived some $q_{\alpha_i}$ it would propagate the x's instead, but I don't think this has consequence.
	\item Conjecture -- If we only ever branch on x's and q's, the only clauses we can possibly learn are $\neg q$'s.
	\item Suppose adversary starts with x sequence $x_1, ..., x_k$. Then we must learn every $q$ on the branch of $x_1$ before we can move to $x_1^{-1}$ branch. Need to count the number of assignments on the $x_1$ side that depend on q's of the other side.
\end{itemize}

\begin{conjecture}
	Take the formula from 7.1, with any ordering of the $\alpha$'s. Then, if the solver is only allowed to branch on $x$'s and $q$'s, regardless of the decision sequence, it can only learn unit clauses of the form $\neg q$. \todo{PROBLEM: assign all q's first??}
\end{conjecture}
\begin{proof}
	Suppose $c$ is the first learnt clause. There are three cases which can lead to this conflict. If we assign $q$ (positively), we immediately learn $\not q$. Suppose we falsify some clause with $C_{\alpha_i}$.
\end{proof}

\subsection{Whiteboard Notes 2.0}
Our goal is to show that the smallest LSR+backtracking backdoor for $F$ is exponentially smaller than the smallest LS+backtracking backdoor. We know $F$ is minimally unsatisfiable. First, let us partition $F$ into two sets of clauses. Let $\Delta_1$ be the $2^k$ clauses that contain some $C_{\alpha_i}$ disjunction, and $\Delta_2$ be the remaining clauses that allow us to learn each $\neg q_i$, i.e., the clauses in $L(\neg q_i)$ for all $i$. Let $F_{x=b} = \Delta_1[x=b] \cup \{ L(q_\alpha) \mid q_\alpha \in vars(\Delta_1[x=b]) \}$

\todo{proof sketch -- order the clauses according to number of qs, since each clause has 2 unseen vars, and the formula is min unsat, we must branch upon one of them to use the clause}

\begin{lemma}
For any $x \in X$ and any polarity $b$, $F_{x=b}$ is minimally unsatisfiable.
\end{lemma}
\begin{proof}
	Suppose for some $\alpha$ we remove some clause from $L(\neg q_alpha)$. Then we can assign $q_alpha$ (positively) without conflicting. By assigning $X$ according to $\alpha$, and $\neg q_\beta$, $\beta \ne \alpha$, we can satisfy all other clauses.
	If instead we remove any clause $C \in \Delta_1[x=b]$, then we can satisfy the remaining clauses by setting $\neg q_\alpha$ for every $\alpha$, and $X$ according to $\neg \alpha$.
\end{proof}



\subsection{LS+Jumps+Restarts is [exponentially(?)] smaller than LS+Jumps-Restarts}
\todo{BROKEN, but maybe not for sat case}
$X$ will denote our backdoor set of size $k$, where $k$ is even (\todo{may need one more var}). Different from before, $C_\alpha$ will correspond to a disjunction of the first $k/2$ variables in $X$, and $C_\beta$ is a disjunction of the second $k/2$ variables. Rather than the clauses used to conflict and learn $\neg q_\alpha$ as before, we have the following formula which will be used to derive binary clauses rather than unit clauses:
\todo{Fix 1uip according to williams discussion}
$$
L(l_\alpha \vee l_\beta) ::=
(\neg l_\alpha \vee r_\alpha),
(\neg l_\alpha \vee s_\alpha),
(\neg l_\beta \vee r_\beta),
(\neg l_\beta \vee s_\beta),
(\neg r_\alpha \vee \neg s_\alpha \vee \neg r_\beta \vee \neg s_\beta)
$$

We define a formula $\Omega(n)$ which is any formula over $n$ fresh variables with backdoor size $n$. As an example, the formula with all possible clauses of length $n$ over the $n$ variables will suffice. Finally, let $\Omega[l_1, l_2](n)$, where the literals $l_1, l_2$ are not in $\Omega(n)$, be the same as $\Omega(n)$, but every clause has the additional literals $l_1$ and $l_2$.

Potential example with LSR-backdoor set $X$ + any single $q$ or $r$:

\begin{equation}
\label{lsr_jump_eqn}
\begin{split}
&\bigwedge_{\alpha} 
(C_{\alpha} \vee q_{\alpha}),
\bigwedge_{\beta} 
(C_{\beta} \vee \neg r_{\beta}), \\
&\bigwedge \{ L(q_\alpha \Rightarrow r_\beta) \mid \alpha = \beta\} \\ 
&\bigwedge \{ L(r_\beta \Rightarrow q_\alpha) \mid \alpha = \beta + 1\} \\ 
&\bigwedge \{ \Omega[q_\alpha, \neg r_{\beta}] \mid \alpha \ne \beta \wedge \alpha \ne \beta + 1\}  \\
&(\neg q_{\alpha_0} \Rightarrow  r_{\beta_{2^k}}), 
(q_{\alpha_0} \Rightarrow \neg r_{\beta_{2^k}}), 
(\neg q_{\alpha_0} \Rightarrow \neg r_{\beta_{2^k}}),
\end{split}
\end{equation}

\todo{Might need to hide (4) under last X vals}

\begin{theorem}
	There exists a family of formulas such that the smallest LSR+backjumping backdoor is \todo{exponentially} smaller than the smallest LS+backjumping backdoor.
\end{theorem}
\begin{proof}
We first demonstrate that 
\end{proof}



\suppress{
\section{LSR vs LS old}
$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee p_1^\prime), (\neg x \vee p_2^\prime), (\neg p_1^\prime \vee \neg p_2^\prime \vee \neg q \vee q^\prime), (\neg q^\prime \vee a^\prime), (\neg q^\prime \vee \neg a^\prime \vee b^\prime), (\neg q^\prime \vee \neg a^\prime \vee \neg b^\prime) 
$$
$$
(x \vee q \vee q^\prime \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$


\section{LSR may be arbitrarily smaller than LS}
The following formula from the LS paper has a minimal LS backdoor \{x\}:
$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee q \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$
Essentially, if we set $x=0$, we learn $\neg q$ on the top half, which leads to a conflict on the bottom half when we set $x=1$.

Now consider a new formula which duplicates the first line: 
{\boldmath$$
(x \vee p_1^\prime), (x \vee p_2^\prime), (\neg p_1^\prime \vee \neg p_2^\prime \vee q^\prime), (\neg q^\prime \vee a^\prime), (\neg q^\prime \vee \neg a^\prime \vee b^\prime), (\neg q^\prime \vee \neg a^\prime \vee \neg b^\prime) 
$$
}$$
(x \vee p_1), (x \vee p_2), (\neg p_1 \vee \neg p_2 \vee q), (\neg q \vee a), (\neg q \vee \neg a \vee b), (\neg q \vee \neg a \vee \neg b) 
$$
$$
(\neg x \vee q \bm{\vee q^\prime} \vee r), (\neg r \vee a), (\neg r \vee \neg a \vee b), (\neg r \vee \neg a \vee \neg b)
$$
We can then set $x=0$ to learn $q$ as before, but then restart to learn $q^\prime$ as well. 

We can repeat this any number of times by introducing a new ``prime row'' (and q in the bottom clause).
This breaks my previous conjecture that $LS = LSR + \mathcal{O}(log(numRestarts))$. New conjecture: $LS = LSR + \mathcal{O}(numRestarts))$.


\section{Main Contributions}
\begin{itemize}
	\item LSR backdoor definition + algorithm
	\item Correlation experiments for several metrics over SAT comps + scaling.
	\item Relationship of cmty structure/bridges and backdoors
	\item Solving with a priori knowledge of metrics		
\end{itemize}

\section{Paper Threats}
\begin{itemize}
	\item Need to motivate LSR backdoors
	\begin{itemize}
		\item Small examples where minimum LS-backdoor is larger than LSR
		\item General relationship/bound of LSR to LS sizes.
	\end{itemize}
	\item General Threats to Validity
	\begin{itemize}
		\item We don't have optimal value (e.g. minimum backdoors). Answer: using current best algorithms + long timeouts.
		\item Consider multiple solvers (for now just maplesat times). Have most data for Glucose and Minisat. 
		\item Consider more than linear regression for correlation experiments (ridge regression, which handles multicollinearity better than LR, achieved similar $R^2$ values)
		\item LSR computation based upon solver run (circularity threat?.. cannot remember how we resolved this..)
		\item Solving times should probably be recomputed on StarExec/Azure (sharcnet has some unpredictability).
		\item Need to explain why correlations are lower than 2014 cmty structure paper.
	\end{itemize}
\end{itemize}
}
}

==> tables/structure_logging_table.tex <==
\begin{table}[t]
	\begin{center}
		\begin{tabular}{ |l|l||c|c|c| }
			\hline
			\textbf{Property} & \textbf{Benchmark} & \textbf{Luby} & \textbf{Always Restart} & \textbf{Never Restart} \\ \hline
			\multirow{4}{12em}{P1: LSR Size} &
			agile & nan & nan & nan\\
			& app & nan & nan & nan\\
			& crafted & nan & nan & nan\\
			& random & nan & nan & nan \\ \hline
			\multirow{4}{12em}{Solving Time} &
			agile & nan & nan & nan\\
			& app & nan & nan & nan\\
			& crafted & nan & nan & nan\\
			& random & nan & nan & nan \\ \hline
		\end{tabular}
		\caption{\todo{fill in}}
	\end{center}
\end{table}

==> tables/summary.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrrrrr}
\toprule
{} &  Instances &   SAT &  LSR &  Weak &  Cmty &  Bones &    TW \\
\midrule
Agile       &       4968 &   315 &    0 &   464 &  4968 &    208 &  4968 \\
Application &       1144 &   438 &    0 &   281 &   891 &    193 &  1088 \\
Crafted     &        753 &   236 &    0 &   195 &   613 &    154 &   753 \\
Random      &        126 &    76 &    0 &    76 &   126 &     59 &   126 \\
Total       &       6991 &  1065 &    0 &  1016 &  6598 &    614 &  6935 \\
\bottomrule
\end{tabular}

\caption{The number of instances in each benchmark, as well as the number of instances we were able to successfully compute each parameter/time (timeouts included). ``Cmty'' refers to the community parameters; ``TW'' denotes the treewidth upper bound; ``Bones'' denotes backbone size. Note that the number of satisfiable instances upper bounds the number of instances for which we can obtain weak backdoors and backbones.}
\end{table}



==> tables/threats.tex <==
\section{Threats to Validity}
\todo{circularity argument against correlations with solving time, especially for lsr/weak, which were computed using a run of the solver.}


Due to the difficulty of computing the exact/best values for the parameters considered in the paper, we must rely upon heuristic algorithms. We attempt to mitigate this threat by using the best off-the-shelf algorithms for each parameters and by allowing long runtimes when necessary. 
Our results are also dependent upon the instances that we studied. We attempt to make our results more generally applicable, by studying a large set of instances from multiple categories of the SAT competitions. We also expect that solving time correlation results would be higher if we used more heterogeneous sets of instances. We mitigate this by separating the results with respect to the SAT competition categories, however a finer-grained analysis might be fruitful. We also only used a small set of random instances which may affect results, however given the intrinsically unstructured nature of random instances, we expect that adding more instances would only make correlations worse.
Correlations were also computed with ridge regression in order to better deal with multi-collinearities in the data, as compared to standard linear regression. Our results are also dependent on the solvers MapleSAT and MapleCOMSPS. We expect similar results for other MiniSAT-based solvers, but more solvers should be considered.

In regard to LSR computation, in order to improve confidence that our backdoor sets are indeed backdoors, we built a verifier and ensured that the solver could correctly determine satisfiability by only branching on backdoor variables.



==> tables/tsebg.tex <==
\section{Background}
\label{sec:background}
This section provides the necessary background on FMs
and the use of SAT solvers in analyzing them. We also describe the structural metrics that will be analyzed in Section \ref{sec:structural}.

\subsection{Feature Models (FM)}

\begin{figure}
	\begin{centering}
		\includegraphics[width=\linewidth]{fm.pdf}
		\caption{A feature model depicting a family of mobile phone products.}
		\label{fig:fm}
	\end{centering}
\end{figure}

Figure \ref{fig:fm} depicts an example FM of family of mobile phones.
Structurally, a FM looks like a tree where each node
represents a distinct feature. The terms node and feature will be
used interchangeably. Child nodes have two flavours: \emph{mandatory}
(the child feature is present if and only if the parent feature is
present) such as \texttt{OS} and \texttt{Calls}, and \emph{optional} (if the parent feature is present then
the child feature is optional, otherwise it is absent) such as \texttt{Android} and \texttt{Bluetooth}. Parent nodes
can also restrict its children with feature groups: \emph{or} (if the
parent feature is present, then at least one of its child features is
present) such as \texttt{Connectivity}, and \emph{alternative} (if the parent feature is present,
then exactly one of its child features is present) as in \texttt{OS}. These are the
structural constraints between the child and the
parent.
%Figure~\ref{fig:wikifm} is an example of a FM
%represented diagrammatically.

Structural constraints are often not enough to enforce the integrity
of the model, in which case cross-tree constraints are
necessary. Cross-tree constraints (e.g. \texttt{Video requires Camera}) have no restrictions like structural
constraints do, and can apply to any feature regardless of their
position in the tree-part of the model. For this paper, cross-tree
constraints are formulas in propositional logic where features are the
variables in the formulas. Two examples of common cross-tree
constraints are $A \rightarrow B$ (A requires B) and $A \rightarrow \neg B$
(A excludes B). An example phone product for the FM in Figure \ref{fig:fm} is an Android phone with voice calling, but no connectivity.

\begin{table*}
\scriptsize
        \begin{centering}
\begin{tabular}{lrrrrrr}
\hline
Model & Variables & Clauses & Horn (\%) & Anti-Horn (\%) & Binary (\%) & Other (\%) \\\hline
2.6.28.6-icse11 & 6888 & 343944 & 7.54 & 50.80 & 6.19 & 47.29 \\
2.6.32-2var & 60072 & 268223 & 61.81 & 70.66 & 27.02 & 5.01 \\
2.6.33.3-2var & 62482 & 273799 & 63.24 & 70.05 & 27.74 & 5.08 \\
axTLS & 684 & 2155 & 71.04 & 52.99 & 25.85 & 7.19 \\
buildroot & 14910 & 45603 & 76.78 & 61.81 & 40.24 & 2.68 \\
busybox-1.18.0 & 6796 & 17836 & 79.79 & 56.91 & 37.25 & 1.94 \\
coreboot & 12268 & 47091 & 82.67 & 68.53 & 45.73 & 0.59 \\
ecos-icse11 & 1244 & 3146 & 92.59 & 73.36 & 73.27 & 6.64 \\
embtoolkit & 23516 & 180511 & 29.06 & 87.65 & 17.81 & 0.34 \\
fiasco & 1638 & 5228 & 84.87 & 52.85 & 38.49 & 1.42 \\
freebsd-icse11 & 1396 & 62183 & 8.25 & 84.79 & 2.63 & 9.52 \\
freetz & 31012 & 102705 & 76.56 & 52.35 & 34.60 & 3.04 \\
toybox & 544 & 1020 & 90.49 & 67.75 & 46.76 & 0.00 \\
uClinux-config & 11254 & 31637 & 69.23 & 63.42 & 30.73 & 0.96 \\
uClinux & 1850 & 2468 & 100.00 & 75.04 & 50.00 & 0.00 \\ \hline 

\end{tabular}
                \caption{Clause and variable counts of real-world
                  FMs. The last four columns count the percentage of
                  clauses with the specified property (as discussed in Section \ref{sec:restricted}). ``Other" are
                  clauses that are neither Horn, anti-Horn, nor
                  binary. The percentages do not sum to 100\% because
                  Horn, anti-Horn, and binary are not
                  disjoint.}
                \label{tab:stats}
        \end{centering}
\end{table*}

\begin{table*}
	\scriptsize
	\begin{centering}
		\begin{tabular}{lrrrrrr}
			\hline
			Model & Variables & Clauses & Horn (\%) & Anti-Horn (\%) & Binary (\%) & Other (\%) \\\hline
			Large RW\hspace{14pt} & 15770 & 92503 & 66.26 & 65.93 & 48.96 & 6.11 \\
			CDL & 1246 & 7067 & 84.77 & 62.83 & 63.00 & 14.53 \\
			KConfig & 34824 & 677612 & 68.06 & 56.40 & 43.25 & 3.86 \\
			SPLOT & 86 & 158 & 90.53 & 89.47 & 90.42 & 0.01 \\
			Random & 2750 & 5012 & 90.96 & 77.30 & 88.95 & 0.00 \\
			
		\end{tabular}
		\caption{Clause data average-of-averages for each case study considered. Large RW refers to the same dataset as listed in Table \ref{tab:stats}.}
		\label{tab:summarystats}
	\end{centering}
\end{table*}


\subsection{SAT-based Analysis of Feature Models}
The goal of SAT-based analysis of FMs is to find an assignment to the
features such that the structural and cross-tree constraints are
satisfied. It turns out that there is a natural reduction from feature
models to SAT~\cite{BatorySPLC}. Each feature is mapped to a Boolean
variable, the variable is true/false if the feature is
selected/deselected. The structural and cross-tree constraints are
encoded as propositional logic formulas. The SAT solver can answer
questions like whether the feature model encodes no products.
The solver can also be adapted to handle product
configuration: given a set of features that must be present and
another set of features that must be absent, the solver will find a
product that satisfies the request or answer that no such product
exists. Optimization is also possible such as finding the product with
the highest performance, although for this we need optimization
solvers, multiple calls to a SAT solver, and/or bit-blasting the feature model attributes
into a Boolean formula. Dead features, features that cannot exist in any valid
products, can also be detected using solvers. More generally, SAT
solvers provide a variety of possibilities for automated analysis of
FMs, where manual analysis may be infeasible. Many
specialized solvers~\cite{FMAlloy,SATConfigurator,FMReasoning} for FM
analysis have been built that use SAT solvers as a backend. It is
natural to ask why SAT-based analysis tools scale so well and are so
effective in diverse kinds of analysis of large real-world FMs. This
question has been studied with randomly generated FMs based
on realistic parameters~\cite{MendoncaEasySat,BETTY,Pohl2013} where
all the instances were easily solved by a modern SAT solver. In this
paper, we are studying large real-world FMs to explain why they are
easy for SAT solvers.

\subsection{Structural Metrics}
\subsubsection{Backdoors-related Concepts}
For the purposes of this section we only introduce informal and partial definitions of backdoor-related concepts; formal definitions can be found in the corresponding literature below.
A set of variables \textit{B} is a \textit{weak backdoor} to a formula \textit{F}  if there exists some assignment $a_B : B \rightarrow$ $\{t, f\}$ such that \textit{F}$[a_B]$, that is, \textit{F} simplified by the assignment $a_B$, can be solved using only BCP  \cite{williams2003backdoors}. Intuitively, if the weak backdoor \textit{B} is very small, then we can perform a systematic search over assignments to \textit{B} to solve the problem. The \textit{backbone} of a SAT instance is the set of variables such that all models of the instance contain the same polarity of the variable \cite{monasson1999determining}. Note that weak backdoors and backbones are implicitly only defined over satisfiable instances. Further, while the backbone of an instance is unique, many weak backdoors may exist; we typically try to find the smallest weak backdoors possible.

\subsubsection{Graph Abstractions}
All graphs discussed in this paper are undirected.
The \textit{variable incidence graph (VIG)} of a CNF formula $F$ is defined as follows: vertices of the
graph are the variables in the formula.  For every clause $c \in F$ we
have an edge between each pair of variables in $c$.  In other words,
each clause corresponds to a clique between its variables.  The weight
of an edge is $\frac{1}{|c|-1}$ where $|c|$ is the length of the
clause.  VIG does not distinguish between positive and negative
occurrences of variables.  We combine all edges between each pair of
vertices into one weighted edge by summing the weights. More precisely,
the VIG of a CNF formula $F$ is a weighted graph defined as follows:
set of vertices $V = Var$, set of edges $E =\{xy \mid x,y\in
c\in F\}$, and the weight function $w(xy) = \sum_{x,y\in c                                                                                                                                                          
	\in F} \frac{1}{|c|-1}$.

For the \textit{incidence graph} of a CNF formula, we introduce one vertex for every variable, and one vertex for every clause. An edge exists between a ``variable vertex'' and a ``clause vertex'' exactly when the corresponding variable occurs in the corresponding clause. No edges exists from between two variable vertices, nor between two clause vertices. The sets of variable vertices and clause vertices therefore form a bipartition of the incidence graph. 

\subsubsection{Graph Metrics}
Given a graph abstraction, the \textit{treewidth} of the graph intuitively measures how much a graph resembles a tree. Actual trees have treewidth 1. Further details can be found in \cite{robertson1984graph}.

The community structure of a graph is a partition of the vertices into communities, such that there are more intracommunity edges within a community than intercommunity edges. The \textit{modularity} or \textit{Q} value denotes how easily separable are the communities of the graph. The \textit{Q} value ranges from $[0, 1]$, where $1$ means the communities are highly separable and the graph intuitively has a \textit{better} community structure.


==> threats.tex <==
\section{Threats to Validity}
\todo{circularity argument against correlations with solving time, especially for lsr/weak, which were computed using a run of the solver.}


Due to the difficulty of computing the exact/best values for the parameters considered in the paper, we must rely upon heuristic algorithms. We attempt to mitigate this threat by using the best off-the-shelf algorithms for each parameters and by allowing long runtimes when necessary. 
Our results are also dependent upon the instances that we studied. We attempt to make our results more generally applicable, by studying a large set of instances from multiple categories of the SAT competitions. We also expect that solving time correlation results would be higher if we used more heterogeneous sets of instances. We mitigate this by separating the results with respect to the SAT competition categories, however a finer-grained analysis might be fruitful. We also only used a small set of random instances which may affect results, however given the intrinsically unstructured nature of random instances, we expect that adding more instances would only make correlations worse.
Correlations were also computed with ridge regression in order to better deal with multi-collinearities in the data, as compared to standard linear regression. Our results are also dependent on the solvers MapleSAT and MapleCOMSPS. We expect similar results for other MiniSAT-based solvers, but more solvers should be considered.

In regard to LSR computation, in order to improve confidence that our backdoor sets are indeed backdoors, we built a verifier and ensured that the solver could correctly determine satisfiability by only branching on backdoor variables.



==> tsebg.tex <==
\section{Background}
\label{sec:background}
This section provides the necessary background on FMs
and the use of SAT solvers in analyzing them. We also describe the structural metrics that will be analyzed in Section \ref{sec:structural}.

\subsection{Feature Models (FM)}

\begin{figure}
	\begin{centering}
		\includegraphics[width=\linewidth]{fm.pdf}
		\caption{A feature model depicting a family of mobile phone products.}
		\label{fig:fm}
	\end{centering}
\end{figure}

Figure \ref{fig:fm} depicts an example FM of family of mobile phones.
Structurally, a FM looks like a tree where each node
represents a distinct feature. The terms node and feature will be
used interchangeably. Child nodes have two flavours: \emph{mandatory}
(the child feature is present if and only if the parent feature is
present) such as \texttt{OS} and \texttt{Calls}, and \emph{optional} (if the parent feature is present then
the child feature is optional, otherwise it is absent) such as \texttt{Android} and \texttt{Bluetooth}. Parent nodes
can also restrict its children with feature groups: \emph{or} (if the
parent feature is present, then at least one of its child features is
present) such as \texttt{Connectivity}, and \emph{alternative} (if the parent feature is present,
then exactly one of its child features is present) as in \texttt{OS}. These are the
structural constraints between the child and the
parent.
%Figure~\ref{fig:wikifm} is an example of a FM
%represented diagrammatically.

Structural constraints are often not enough to enforce the integrity
of the model, in which case cross-tree constraints are
necessary. Cross-tree constraints (e.g. \texttt{Video requires Camera}) have no restrictions like structural
constraints do, and can apply to any feature regardless of their
position in the tree-part of the model. For this paper, cross-tree
constraints are formulas in propositional logic where features are the
variables in the formulas. Two examples of common cross-tree
constraints are $A \rightarrow B$ (A requires B) and $A \rightarrow \neg B$
(A excludes B). An example phone product for the FM in Figure \ref{fig:fm} is an Android phone with voice calling, but no connectivity.

\begin{table*}
\scriptsize
        \begin{centering}
\begin{tabular}{lrrrrrr}
\hline
Model & Variables & Clauses & Horn (\%) & Anti-Horn (\%) & Binary (\%) & Other (\%) \\\hline
2.6.28.6-icse11 & 6888 & 343944 & 7.54 & 50.80 & 6.19 & 47.29 \\
2.6.32-2var & 60072 & 268223 & 61.81 & 70.66 & 27.02 & 5.01 \\
2.6.33.3-2var & 62482 & 273799 & 63.24 & 70.05 & 27.74 & 5.08 \\
axTLS & 684 & 2155 & 71.04 & 52.99 & 25.85 & 7.19 \\
buildroot & 14910 & 45603 & 76.78 & 61.81 & 40.24 & 2.68 \\
busybox-1.18.0 & 6796 & 17836 & 79.79 & 56.91 & 37.25 & 1.94 \\
coreboot & 12268 & 47091 & 82.67 & 68.53 & 45.73 & 0.59 \\
ecos-icse11 & 1244 & 3146 & 92.59 & 73.36 & 73.27 & 6.64 \\
embtoolkit & 23516 & 180511 & 29.06 & 87.65 & 17.81 & 0.34 \\
fiasco & 1638 & 5228 & 84.87 & 52.85 & 38.49 & 1.42 \\
freebsd-icse11 & 1396 & 62183 & 8.25 & 84.79 & 2.63 & 9.52 \\
freetz & 31012 & 102705 & 76.56 & 52.35 & 34.60 & 3.04 \\
toybox & 544 & 1020 & 90.49 & 67.75 & 46.76 & 0.00 \\
uClinux-config & 11254 & 31637 & 69.23 & 63.42 & 30.73 & 0.96 \\
uClinux & 1850 & 2468 & 100.00 & 75.04 & 50.00 & 0.00 \\ \hline 

\end{tabular}
                \caption{Clause and variable counts of real-world
                  FMs. The last four columns count the percentage of
                  clauses with the specified property (as discussed in Section \ref{sec:restricted}). ``Other" are
                  clauses that are neither Horn, anti-Horn, nor
                  binary. The percentages do not sum to 100\% because
                  Horn, anti-Horn, and binary are not
                  disjoint.}
                \label{tab:stats}
        \end{centering}
\end{table*}

\begin{table*}
	\scriptsize
	\begin{centering}
		\begin{tabular}{lrrrrrr}
			\hline
			Model & Variables & Clauses & Horn (\%) & Anti-Horn (\%) & Binary (\%) & Other (\%) \\\hline
			Large RW\hspace{14pt} & 15770 & 92503 & 66.26 & 65.93 & 48.96 & 6.11 \\
			CDL & 1246 & 7067 & 84.77 & 62.83 & 63.00 & 14.53 \\
			KConfig & 34824 & 677612 & 68.06 & 56.40 & 43.25 & 3.86 \\
			SPLOT & 86 & 158 & 90.53 & 89.47 & 90.42 & 0.01 \\
			Random & 2750 & 5012 & 90.96 & 77.30 & 88.95 & 0.00 \\
			
		\end{tabular}
		\caption{Clause data average-of-averages for each case study considered. Large RW refers to the same dataset as listed in Table \ref{tab:stats}.}
		\label{tab:summarystats}
	\end{centering}
\end{table*}


\subsection{SAT-based Analysis of Feature Models}
The goal of SAT-based analysis of FMs is to find an assignment to the
features such that the structural and cross-tree constraints are
satisfied. It turns out that there is a natural reduction from feature
models to SAT~\cite{BatorySPLC}. Each feature is mapped to a Boolean
variable, the variable is true/false if the feature is
selected/deselected. The structural and cross-tree constraints are
encoded as propositional logic formulas. The SAT solver can answer
questions like whether the feature model encodes no products.
The solver can also be adapted to handle product
configuration: given a set of features that must be present and
another set of features that must be absent, the solver will find a
product that satisfies the request or answer that no such product
exists. Optimization is also possible such as finding the product with
the highest performance, although for this we need optimization
solvers, multiple calls to a SAT solver, and/or bit-blasting the feature model attributes
into a Boolean formula. Dead features, features that cannot exist in any valid
products, can also be detected using solvers. More generally, SAT
solvers provide a variety of possibilities for automated analysis of
FMs, where manual analysis may be infeasible. Many
specialized solvers~\cite{FMAlloy,SATConfigurator,FMReasoning} for FM
analysis have been built that use SAT solvers as a backend. It is
natural to ask why SAT-based analysis tools scale so well and are so
effective in diverse kinds of analysis of large real-world FMs. This
question has been studied with randomly generated FMs based
on realistic parameters~\cite{MendoncaEasySat,BETTY,Pohl2013} where
all the instances were easily solved by a modern SAT solver. In this
paper, we are studying large real-world FMs to explain why they are
easy for SAT solvers.

\subsection{Structural Metrics}
\subsubsection{Backdoors-related Concepts}
For the purposes of this section we only introduce informal and partial definitions of backdoor-related concepts; formal definitions can be found in the corresponding literature below.
A set of variables \textit{B} is a \textit{weak backdoor} to a formula \textit{F}  if there exists some assignment $a_B : B \rightarrow$ $\{t, f\}$ such that \textit{F}$[a_B]$, that is, \textit{F} simplified by the assignment $a_B$, can be solved using only BCP  \cite{williams2003backdoors}. Intuitively, if the weak backdoor \textit{B} is very small, then we can perform a systematic search over assignments to \textit{B} to solve the problem. The \textit{backbone} of a SAT instance is the set of variables such that all models of the instance contain the same polarity of the variable \cite{monasson1999determining}. Note that weak backdoors and backbones are implicitly only defined over satisfiable instances. Further, while the backbone of an instance is unique, many weak backdoors may exist; we typically try to find the smallest weak backdoors possible.

\subsubsection{Graph Abstractions}
All graphs discussed in this paper are undirected.
The \textit{variable incidence graph (VIG)} of a CNF formula $F$ is defined as follows: vertices of the
graph are the variables in the formula.  For every clause $c \in F$ we
have an edge between each pair of variables in $c$.  In other words,
each clause corresponds to a clique between its variables.  The weight
of an edge is $\frac{1}{|c|-1}$ where $|c|$ is the length of the
clause.  VIG does not distinguish between positive and negative
occurrences of variables.  We combine all edges between each pair of
vertices into one weighted edge by summing the weights. More precisely,
the VIG of a CNF formula $F$ is a weighted graph defined as follows:
set of vertices $V = Var$, set of edges $E =\{xy \mid x,y\in
c\in F\}$, and the weight function $w(xy) = \sum_{x,y\in c                                                                                                                                                          
	\in F} \frac{1}{|c|-1}$.

For the \textit{incidence graph} of a CNF formula, we introduce one vertex for every variable, and one vertex for every clause. An edge exists between a ``variable vertex'' and a ``clause vertex'' exactly when the corresponding variable occurs in the corresponding clause. No edges exists from between two variable vertices, nor between two clause vertices. The sets of variable vertices and clause vertices therefore form a bipartition of the incidence graph. 

\subsubsection{Graph Metrics}
Given a graph abstraction, the \textit{treewidth} of the graph intuitively measures how much a graph resembles a tree. Actual trees have treewidth 1. Further details can be found in \cite{robertson1984graph}.

The community structure of a graph is a partition of the vertices into communities, such that there are more intracommunity edges within a community than intercommunity edges. The \textit{modularity} or \textit{Q} value denotes how easily separable are the communities of the graph. The \textit{Q} value ranges from $[0, 1]$, where $1$ means the communities are highly separable and the graph intuitively has a \textit{better} community structure.

